Optimal Pricing of Information

A decision maker is choosing between an active action (e.g., purchase a house, invest certain stock) and a passive action. The payoff of the active action depends on the buyer's private type and also an unknown state of nature. An information seller can design experiments to reveal information about the realized state to the decision maker, and would like to maximize profit from selling such information. We characterize, in closed-form, the revenue-optimal information selling mechanism for the seller. After eliciting the buyer's type, the optimal mechanism charges the buyer an upfront payment and then simply reveals whether the realized state exceeds a certain threshold or not. The optimal mechanism features both price discrimination and information discrimination. The special buyer type who is a-priori indifferent between the active and passive action benefits the most from participating in the mechanism.

==> case2.tex <==
%\begin{lemma}\label{lem:optimal-case2} 
%    \item If $v(t_2) \geq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx $ (or equivalently, $v(t_1) \geq -  \int_{t_1}^{t_2} \int_{q: \rho(q) \leq \bar{\theta}_x} \\ g(q) v_1(q) dq  dx $) and $\bar{\phi}(t)$ is monotone non-decreasing, the optimal information selling mechanism is a threshold mechanism on $\rho(q)$ with threshold $\bar{\theta}(t) =  -\bar{\phi}(t) $ for each type $t$. The payment is determined by the following identity and is monotone non-increasing in $t$:
%    $$p(t) = \int_{q\in Q} [g(q) \pi(q,t)v(q,t)] dq - v(t_2) + \int_{t}^{t_2} P(x)  dx.$$   
%\end{lemma}

\section{Optimal Mechanism for Case 2 ($v(t_2)\ge V_H$)}
\label{sec:case2}
In this section, we will discuss the second case of our main result, where $v(t_2)\ge V_H$. In this case, if we still use $t_1$ as the reference point and follow the same analysis of Section \ref{sec:case1}, we will end up having a mechanism with $u(t_2)<v(t_2)$, hence infeasible. To solve this problem, we write the revenue expression $REV(\pi,p)$ using $t_2$ as the reference point. Although the resulting mechanism looks different, the approach for deriving it is quite similar to that in Section \ref{sec:case1}.
\begin{lemma}
    \label{lem:optimal-case2} 
    If $v(t_2) \geq V_H $, the optimal information selling mechanism is the threshold mechanism $\pi^*$ with threshold ${\theta}^*(t) =  -\bar{\phi}^+(t) $ for each type $t$. The payment is determined by the following equation and is monotone non-increasing in $t$:
    \begin{gather*}
        p^*(t) = \int_{q\in Q} g(q) \pi^*(q,t)v(q,t)\,\dd q  + \int_{t}^{t_2} P_{\pi^*}(x)\,\dd x- v(t_2).
    \end{gather*}
\end{lemma}
%\begin{remark}
%    The proof of Lemma \ref{lem:optimal-case2} is very similar to that of Lemma \ref{lem:optimal-case1}. The major difference is that now we use a different reference point $u(t_2)$. The discussion before Lemma \ref{lem:optimal-case2} is why we have to derive another utility representation by using the equality  $u(t) = u(t_2) -\int_{t }^{t_2} P_{\pi}(x)\,\dd x$ to expand $u(t)$ with $t_2$ as the reference point. This gives us a slightly different representation of the same $REV (\pi, p)$. 
%\end{remark}
\begin{proof}%[Proof of Lemma \ref{lem:optimal-case2}]
    Similar to the proof of Lemma \ref{lem:optimal-case1}, this proof also contains 3 steps:
    
    {\bfseries Step 1.} In the first step, we derive the revenue of information selling in a slightly different way than in the proof of Lemma \ref{lem:optimal-case1}, i.e., using $t_2$ as the reference point instead of $t_1$.
    \begin{align}
        REV (\pi, p)
        =&\int_{t_1}^{t_2} f(t)\left[\int_{q \in Q} g(q) \pi^*(q,t)v(q,t) \,\dd q -u(t) \right]\,\dd t \nonumber\\
        =&\int_{t_1}^{t_2} f(t)\left[\int_{q \in Q} g(q)\pi^*(q,t)v(q,t) \,\dd q  -u(t_2) + \int_{t}^{t_2} P_{\pi^*}(x)\,\dd x \right]\,\dd t \nonumber\\
        =&\int_{t_1}^{t_2} f(t)\left[\int_{q \in Q} g(q) \pi^*(q,t)v(q,t)  \,\dd q \right]\,\dd t + \int_{t_1}^{t_2} \int_{t}^{t_2}f(t) P_{\pi^*}(x)\,\dd x\dd t -u(t_2) \nonumber\\
        =&\int_{t_1}^{t_2} f(t)\left[\int_{q \in Q} g(q) \pi^*(q,t)v(q,t)  \,\dd q \right]\,\mathrm{d}t + \int_{t_1}^{t_2} \int_{t_1}^{x}f(t) P_{\pi^*}(x)\,\dd t\dd x -u(t_2) \nonumber\\
        =&\int_{q \in Q} g(q)\left[\int_{t_1}^{t_2} f(t) \pi^*(q,t)v(q,t) \,\dd q \right]\,\dd t + \int_{t_1}^{t_2} F(t)\int_{q \in Q} g(q)\left[ \pi^* (q,t)v_1(q) \right]\,\dd q\dd t-u(t_2) \nonumber\\
        =&\int_{q \in Q} g(q)\left[ \int_{t_1}^{t_2} f(t)\pi^*(q,t)v_1(q) \left[ \bar{\phi}(t) + \rho(q)\right]\,\dd t \right]\,\dd q -u(t_2) \label{eq:revenue-2}
    \end{align}
%    \begin{align} 
%        &REV (\pi, p)=\int_{t_1}^{t_2} f(t)p(t)\,\mathrm{d}t \nonumber\\
%        &=\int_{t_1}^{t_2} f(t)\left(\int_{q \in Q} g(q) \left[ \pi(q,t)v(q,t)\right]  dq -u(t) \right)\,\mathrm{d}t \nonumber \\
%        &=\int_{t_1}^{t_2} f(t)\left(\int_{q \in Q} g(q)\pi(q,t)v(q,t) dq  -u(t_2) + \int_{t}^{t_2} P(x) \mathrm{d}x \right)\,\mathrm{d}t \nonumber\\
%        &=\int_{t_1}^{t_2} f(t)\left(\int_{q \in Q} g(q) \pi(q,t)v(q,t)  dq \right)\,\mathrm{d}t + \int_{t_1}^{t_2} \int_{t}^{t_2}f(t) P(x)\,\mathrm{d}x\,\mathrm{d}t -u(t_2) \nonumber\\
%        &=\int_{t_1}^{t_2} f(t)\left(\int_{q \in Q} g(q) \pi(q,t)v(q,t)  dq \right)\,\mathrm{d}t + \int_{t_1}^{t_2} \int_{t_1}^{x}f(t) P(x)\,\mathrm{d}t\,\mathrm{d}x -u(t_2) \nonumber\\
%        &=\int_{t_1}^{t_2} f(t)\left(\int_{q \in Q} g(q)  \pi(q,t)v(q,t) dq \right)\,\mathrm{d}t + \int_{t_1}^{t_2} F(x)P(x)\,\mathrm{d}x-u(t_2) \nonumber\\
%        &=\int_{q \in Q} g(q)\left[\int_{t_1}^{t_2} f(t) \pi(q,t)v(q,t) dq \right]\,\mathrm{d}t + \int_{t_1}^{t_2} F(t)\int_{q \in Q} g(q)\left[ \pi (q,t)v_1(q) \right] \mathrm{d}q\,\mathrm{d}t-u(t_2) \nonumber\\
%        &=\int_{q \in Q} g(q)\left[ \int_{t_1}^{t_2} f(t)\pi(q,t) \left(v(q,t)+ v_1(q)\frac{F(t)}{f(t)}\right)\,\mathrm{d}t \right] \mathrm{d}q -u(t_2) \nonumber\\
%        &=\int_{q \in Q} g(q)\left[ \int_{t_1}^{t_2} f(t)\pi(q,t)v_1(q) [ \bar{\phi}(t) + \rho(q)]\,\mathrm{d}t \right] \mathrm{d}q -u(t_2) \label{eq:revenue-2}
%    \end{align}
%    where $\bar{\phi}(t) = t + \frac{F(t)}{f(t)} $ is the upper virtual value function described in Definition XXX \todo{define it before stating main theorem. }.  
    
    {\bfseries Step 2.} Now we show that the given mechanism $(\pi^*,p)$ achieves the maximum revenue. The threshold ${\theta}^*(t) =  -\bar{\phi}(t)$ is picked such that $\pi^*(q,t) =1$ whenever $  \bar{\phi}(t) + \rho(q) \ge 0$ and $\pi^*(q,t) =0$ whenever $ \bar{\phi}(t) + \rho(q) < 0$. That is, the revenue function \eqref{eq:revenue-2}, expressed with $t_2$ as the reference point, is entry-wise maximized. This clearly achieves the maximum possible value in the first term of Equation \eqref{eq:revenue-2}.
    
    The second term is maximized by choosing the minimum possible $u(t_2)$ value, i.e., $u(t_2) = v(t_2)$. With the defined payment function, we indeed choose 
    \begin{gather*}
        u(t_2)  = \int_{q\in Q} g(q) \pi^*(q,t_2)v(q,t_2) \,\dd q - p^*(t_2) =    v(t_2) - \int_{t_2}^{t_2} P_{\pi^*}(x)  \,\dd x = v(t_2).
    \end{gather*}
    
    {\bfseries Step 3.} In the final step, we argue that this choice also leads to a feasible mechanism, satisfying the characterization of Lemma \eqref{lem:feasible-M}. Since the upper virtual value function $\bar{\phi}$ is monotone non-decreasing, we know that the threshold ${\theta}^*(t) = -\bar{\phi}(t)$   is monotone non-increasing in $t$. This implies that 
    \begin{equation*}
        P_{\pi^*}(t) = \int_{q \in Q} \pi^*(q, t) g(q)v_1(q) \,\dd q =   \int_{q: \rho(q) \geq {\theta}^*(t)}   g(q)v_1(q) \,\dd q 
    \end{equation*}
    is monotone non-decreasing in $t$ since a larger $t$ leads to a smaller $\bar{\theta}(t)$ and thus larger integral domain for $q$. So constraint \eqref{eq:signal-monotonicity} is satisfied.
    
    We now prove that $(\pi^*, p^*)$ satisfies constraint \eqref{eq:buyer-utility-identify2}. Plugging the payment function $\pi^*(t)$ into the definition of $u(t)$, we get
    \begin{gather*}
        u(t)  = \int_{q\in Q} g(q) \pi^*(q,t)v(q,t) \,\dd q - p^*(t) =    v(t_2) - \int_{t}^{t_2} P_{\pi^*}(x) \,\dd x.
    \end{gather*}
    It is easy to see that $u(t_2) =  v(t_2)$, which can be plugged back to the above equality to obtain constraint \eqref{eq:buyer-utility-identify2}.
    
    For constraint \eqref{eq:ir-t2}, we already have $u(t_2) =  v(t_2)$. And
    \begin{align*}
        u(t_1) = v(t_2) - \int_{t_1}^{t_2} P_{\pi^*}(x)\,\dd x \geq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} P_{\pi^*}(x)\,\dd x - \int_{t_1}^{t_2} P_{\pi^*}(x) \,\dd x \geq 0.
    \end{align*}
    % For the other side, we know $v(t_1) \geq  - \int_{t_1}^{t_2} \int_{q: \rho(q) \leq \bar{\theta}_x}  g(q) v_1(q) dq  dx$
    
    % If $v(t_1) \geq 0$, 
    % from \eqref{lem:surplus-concave}, we know $s(t)$ is monotone non-increasing for $t \in [\bar{t}, t_2]$, where $v(\bar{t}) = 0 $. Since $v(t_1) \geq 0 \; \Rightarrow \forall t \; v(t) \geq 0$, we have 
    % \begin{align*}
    % s(t_1) &\geq s(t_2) = 0 \\
    % u(t_1) &= v(t_1) + s(t_1) \geq 0 + 0 = 0
    % \end{align*}
    
    % If $\int_{t_1}^{t_2} \int_{q: \rho(q) \leq \bar{\theta}_x}  g(q) v_1(q) dq  dx \geq v(t_1) \geq 0$,
    
    Finally, we show that the payment $p^*(t)$ is non-negative i.e., $p^*(t)$ satisfies constraint \eqref{eq:non-negativity}. We first prove that the $p^*(t)$ is non-increasing in $t$.  
    %
    % due to our choice of $t$ with $F(t)>0$, we have $\bar{\theta}(t) < -t$. Note that the types with $F(t) = 0$ does not need to be taken care as their total probability measure is $0$. 
    %
    % Next, we show $q2 \geq q_t^*$. Since $ v(t) = \int_{q \in Q} g(q)  v(q,t)\, \mathrm{d}q \geq 0$ and $g(q)\geq 0$, we know some of $v(q,t)$ in this integral must be greater than 0. And $q_t^*$ makes $v(q_t^*,t) = v_1(q_t^*)t + v_0(q_t^*) = 0$, so $q_2 \geq q_t^*$. Thus, $q_2 \geq q_t^* \geq \bar{\theta}(t)$.
    %
    %We observe that there exists a small interval $(t-\epsilon, t)$ such that   $\bar{\theta}(t) \leq \bar{\theta}(t') < -t$. Such an $\epsilon$ must exist because $\bar{\theta}(t) = - t - \frac{F(t)}{f(t)}$ is a non-increasing continuous function. Consequently, for any $t'$ in our carefully chosen interval $(t - \epsilon, t)$ we have
    For any $t>t_1$ and $t'\in (t, \bar{\phi}(t))$, we have
    \begin{align}
        p^*(t') -p^*(t) =& \int_{q\in Q} g(q) \pi^*(q,t')v(q,t') \,\dd q - \int_{q\in Q} g(q) \pi^*(q,t)v(q,t) \,\dd q - \int_{t}^{t'} P_{\pi^*}(x)  dx \nonumber\\ 
        =& \int_{q: \rho(q) \geq {\theta}^*(t')}  g(q) v(q,t') \,\dd q - \int_{q: \rho(q) \geq {\theta}^*(t)}  g(q) v(q,t) \,\dd q - \int_{t}^{t'} P_{\pi^*}(x)\,\dd x. \label{eq:payment_decreasing}
    \end{align}
    Observe that ${\theta}^*(t) =-\bar{\phi}(t)\geq -\bar{\phi}(t')= {\theta}^*(t')$.
    So the first term in the right-hand side can be written as:
    \begin{gather*}
        \int_{q: \rho(q) \geq {\theta}^*(t')}  g(q) v(q,t') \,\dd q=\int_{q: \rho(q) \geq {\theta}^*(t)}  g(q) v(q,t') \,\dd q+\int_{q: {\theta}^*(t)\le \rho(q) \leq {\theta}^*(t')}  g(q) v(q,t') \,\dd q.
    \end{gather*}
    When ${\theta}^*(t')\le \rho(q) \leq {\theta}^*(t)$, we have $v(q, t')=v_1(q)[t'+\rho(q)]\le v_1(q)[\bar{\phi}(t)+{\theta}^*(t)]= 0$, where the inequality is due to the choice of $t'$. Therefore, the second term in the right-hand side of the above equation is negative. As a result,
    \begin{gather*}
        \int_{q: \rho(q) \geq {\theta}^*(t')}  g(q) v(q,t') \,\dd q\le \int_{q: \rho(q) \geq {\theta}(t)}  g(q) v(q,t') \,\dd q.
    \end{gather*}
    Combined with Equation \eqref{eq:payment_decreasing}, we get
    \begin{align*}
        p^*(t') -p^*(t) \le & \int_{q: \rho(q) \geq {\theta}^*(t)}  g(q) v(q,t') \,\dd q - \int_{q: \rho(q) \geq {\theta}(t)}  g(q) v(q,t) \,\dd q - \int_{t}^{t'} P_{\pi^*}(x)\,\dd x\\
        =&\int_{q: \rho(q) \geq {\theta}^*(t)}g(q)v_1(q)(t'-t)\,\dd q- \int_{t}^{t'} P_{\pi^*}(x)\,\dd x\\
        =&(t'-t)P_{\pi^*}(t)-\int_{t}^{t'} P_{\pi^*}(x)\,\dd x\\
        \le&0.
    \end{align*}
%    
%  We know that the threshold $\bar{\theta} _t$ satisfies $ \bar{\phi}(t) +  {\theta}^*(t) = 0$. Since $\bar{\phi}(t) = t +\frac{F(t)}{f(t)} \ge t$, we have ${\theta}^*(t) \le -t$.
%    Observe that ${\theta}^*(t)\le {\theta}^*(t')=-\bar{\phi}(t')\le -t'$. Thus when $\rho(q)\ge {\theta}^*(t)$, $v(q,t)=v_1(q)[t+\rho(q)]$.
%    \begin{align*}
%        p(t) -p(t')\leq& \int_{q: \rho(q) \geq {\theta}^*(t')}  g(q) v(q,t)\,\dd q - \int_{q: \rho(q) \geq \bar{\theta}(t')}  g(q) v(q,t')\,\dd q - \int_{t'}^{t} P_{\pi^*}(x)\,\dd x \\ 
%        = & \int_{q: \rho(q) \geq \bar{\theta}(t')} g(q) (v(q,t)-v(q,t'))  dq - \int_{t'}^{t} P(x)  dx \\  
%        =& (t-t') \int_{ q: \rho(q) \geq \bar{\theta}(t') } g(q) v_1(q)  dq - \int_{t'}^{t} P(x)  dx \\ 
%        =& (t-t') \int_{ q \in Q} g(q) v_1(q) \pi^*(q,t')  dq - \int_{t'}^{t} P(x)  dx \\ 
%        =& (t-t') P(t') - \int_{t'}^{t} P(x)  dx \\ 
%        \leq & 0
%    \end{align*}
%    The first inequality is due to  $\bar{\theta}(t) \leq \bar{\theta}(t') < -t$  and thus  $\int_{q: \rho(q) \geq \bar{\theta}(t')}  g(q) v(q,t)  dq$ integrates over less negative terms  compared with $\int_{\bar{\theta}(t)}^{q_2} g(q) v(q,t)  dq$. The last inequality is due to monotonicity of $P(x)$ and our choice of $t>t'$.  Therefore, to prove the non-negativity of the payment, we only need to prove $p(t_2) \geq 0$, as follows:  

\sz{Another direct way is

Since
\begin{align*}
    p(t)=&  \int_{q\in Q} g(q) \pi^*(q,t)v(q,t)\,\dd q  + \int_{t}^{t_2} P_{\pi^*}(x)\,\dd x- v(t_2)\\
    =& \int_{q\in Q} g(q) \pi^*(q,t)v(q,t)\,\dd q  + u(t_2) - \int_{t_1}^{t} P_{\pi^*}(x)\,\dd x- v(t_2)\\
    =&\int_{q:\rho(q)\ge -\bar{\phi}^+(t)}g(q)v(q, t)\,\mathrm{d}q-\int_{t_1}^t \int_{q \in Q} g(q) \pi(q,x) v_1(q)\,\mathrm{d}q\mathrm{d}x + u(t_2) - v(t_2)\\
    =&\int_{q:\rho(q)\ge -\bar{\phi}^+(t)}g(q)v(q, t)\,\mathrm{d}q-\int_{t_1}^t \int_{q:\rho(q)\ge -\bar{\phi}^+(x)} g(q) v_1(q)\,\mathrm{d}q\mathrm{d}x + u(t_2) - v(t_2)
\end{align*}

the differential of $p(t)$ is
\begin{align*}
    \mathrm{d}p(t)=&\left[\int_{q:\rho(q)\ge -\bar{\phi}^+(t)}g(q)\frac{\partial v(q,t)}{\partial t}\,\mathrm{d}q\right]\mathrm{d}t+\left[\frac{\mathrm{d}}{\mathrm{d}\bar{\phi}^+(t)}\int_{q:\rho(q)\ge -\bar{\phi}^+(t)}g(q)v(q, t)\,\mathrm{d}q\right]\mathrm{d}\bar{\phi}^+(t)\\
    &-\left[\int_{q:\rho(q)\ge -\bar{\phi}^+(t)} g(q) v_1(q)\,\mathrm{d}q\right]\mathrm{d}t\\
    =&\left[\frac{\mathrm{d}}{\mathrm{d}\bar{\phi}^+(t)}\int_{q:\rho(q)\ge -\bar{\phi}^+(t)}g(q)v(q, t)\,\mathrm{d}q\right]\mathrm{d}\bar{\phi}^+(t)\\
    =&\left[\sum_{q:\rho(q)=-\bar{\phi}^+(t)}g(q)v(q,t)\right]\mathrm{d}\bar{\phi}^+(t)\\
    =&\left[\sum_{q:\rho(q)=-\bar{\phi}^+(t)}g(q) v_1(q)[t - \bar{\phi}^+(t)] \right]\mathrm{d}\bar{\phi}^+(t) 
\end{align*}
Because we have proved $\bar{\phi}^+(t) \geq t$, we have  $[t - \bar{\phi}^+(t)] \leq 0$ . Since $d\bar{\phi}^+(t)$, $g(q)$, $v_1(q)$ are positive, we get $\forall t \: dp(t)\leq 0 $.

}

    This shows that $p^*(t)$ is monotone non-increasing in the interval $(t,\bar{\phi}(t))$ for any $t>t_1$. Since set of intervals $\{(t,\bar{\phi}(t))\mid t\in T\}$ covers interval $(t_1,t_2]$ and $p(t)$ is clearly continuous, we can conclude that $p^*(t)$ is monotone non-increasing in the entire interval $T$\footnote{Similar techniques are also used to proved existence of solutions for differential equations.}. Thus, to show that the payment is always non-negative, we only need to prove that $p^*(t_2)\ge 0$:
    \begin{align*}
        p^*(t_2) &= \int_{q \in Q} g(q) \pi^*(q,t_2)v(q,t_2)\,\dd q - v(t_2) + \int_{t_2}^{t_2} P_{\pi^*}(x)\,\dd x   \\
        &= \int_{q \in Q} \pi^*(q,t_2) g(q)  v(q,t_2)\, \dd q - \int_{q \in Q} g(q)  v(q,t_2)\, \dd q\\ 
        & \geq 0.
    \end{align*}
    The last inequality comes from the fact that $\pi^*(q,t_2) = 1$ for all $q$ such that $v(q,t_2)\geq 0$. 
\end{proof}
\begin{remark}
    \label{remark:case_2_condition_eq}
    The condition $v(t_2)\ge V_H$ in Lemma \ref{lem:optimal-case2} is equivalent to:
    \begin{gather}
        v(t_1) \geq -  \int_{t_1}^{t_2} \int_{q: \rho(q) \leq {\theta}^*(x)}  g(q) v_1(q)\,\dd q \dd x.\label{eq:case2_condition}
    \end{gather}
    To show the equivalence, note that
    \begin{gather*}
        v(t_2)=v(t_1) + (t_2 - t_1) \int_{q \in Q} v_1(q) g(q) \,\dd q.
    \end{gather*}
    Combining with $v(t_2)\ge V_H$ yields
    \begin{gather*}
        v(t_1) -\max \{v(t_1), 0 \}  \geq    \int_{t_1}^{t_2} \int_{q: \rho(q) \geq {\theta}(x)} g(q) v_1(q)\,\dd q \dd x - (t_2 - t_1) \int_{q \in Q} v_1(q) g(q)\,\dd q.
    \end{gather*}
    Therefore,
    \begin{gather*}
        \min \{v(t_1), 0 \}  \geq  -   \int_{t_1}^{t_2} \int_{q: \rho(q) \leq {\theta}^*(x)}  g(q) v_1(q) \,\dd q \dd x,
    \end{gather*}
    which is equivalent to inequality \eqref{eq:case2_condition} since the right-hand side is negative.
\end{remark}
%
%First, prove the equivalence
%
%\begin{align}
%    &   v(t_2) \geq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx  \nonumber \\ 
%    \Longleftrightarrow \quad  &   v(t_1) + (t_2 - t_1) \int_{q \in Q} v_1(q) g(q) dq  \geq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx \nonumber \\ 
%    \Longleftrightarrow \quad  &   v(t_1) -\max \{v(t_1), 0 \}  \geq    \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx - (t_2 - t_1) \int_{q \in Q} v_1(q) g(q) dq   \nonumber \\ 
%    \Longleftrightarrow \quad  &   v(t_1) -\max \{v(t_1), 0 \}  \geq  -   \int_{t_1}^{t_2} \int_{q: \rho(q) \leq \bar{\theta}_x}  g(q) v_1(q) dq  dx    \nonumber \\
%    \Longleftrightarrow \quad  &   v(t_1)   \geq  -   \int_{t_1}^{t_2} \int_{q: \rho(q) \leq \bar{\theta}_x}  g(q) v_1(q) dq  dx    \label{remark:case_1_condition_eq}
%\end{align}



For the instances in between this two cases, such that
$\int_{t_1}^{t_2} \int_{\underline{\theta_x}}^{q_2} g(q) v_1(q) dq  dx \leq v(t_2) \leq \int_{t_1}^{t_2} \int_{\bar{\theta_x}}^{q_2} g(q) \\ v_1(q) dq  dx $. They are rare but existing, because $\forall t \; \underline{\phi}(t) \leq \bar{\phi}(t) $. Thus, $\forall t \; \underline{\theta_x} \geq \bar{\theta_x} $. Since $g(q)v_1(q)$ is positive, the left-hand-side integral will be smaller than the right-hand-side.
Now, let's define them as cases 3.

Neither of this payment function and allocation rule will solve case 3. Because if we use the threshold and payment function for case 1, $s(t_1) = 0$,  $s(t_2) = u(t_2) - v(t_2) = \int_{t_1}^{t_2} \int_{\underline{\theta_x}}^{q_2} g(q) v_1(q) dq  dx - v(t_2) <= 0$. This will not guarantee the IR constraint. Ditto for case 2.

Thus, the prove of case 3 will need to find a balance and take care of both sides' surplus $s(t_1)$ and $s(t_2)$. The high-level idea in proof of case 3 is to combine the two virtual value $\bar{\phi}(t)$ and  $\underline{\phi}(t)$ tactfully to maximize the revenue function while satisfying IR constraint.

\begin{corollary} \label{same-payment}
If recommendation policies are the same for any two types, then the payment is the same for these two types. Formally, $ \forall t \, \forall t'$, where \, $ \forall q , \pi(q,t) = \pi(q,t')$, then $p(t) = p(t') $.
\end{corollary}

\begin{proof}
We can assume without generality $t \leq t'$. Because $ \forall q, \pi(q,t) = \pi(q,t')$ and monotonicity of $\theta(t)$, we have  $ \forall t \leq t^* \leq t'\, \forall q, \pi(q,t) = \pi(q,t^*) =\pi(q,t')$.




\begin{align*}
p(t) &= \int_{q \in Q} g(q) \pi(q,t)v(q,t) dq -  \int_{t_1}^{t} P(x)  dx. \\
&= \int_{q \in Q} g(q) \pi(q,t')v(q,t) dq -  \int_{t_1}^{t} P(x)  dx. \\
&= \int_{q \in Q} g(q) \pi(q,t')v(q,t') dq -  (t' - t)\int_{q \in Q} g(q) \pi(q,t')v_1(q) dq - \int_{t_1}^{t} P(x)  dx. \\
&= \int_{q \in Q} g(q) \pi(q,t')v(q,t') dq -  \int_{t}^{t'} \int_{q \in Q} g(q) \pi(q,x)v_1(q) dq  dx  -  \int_{t_1}^{t} P(x)  dx. \\
&= \int_{q \in Q} g(q) \pi(q,t')v(q,t') dq -  \int_{t}^{t'} P(x)  dx  -  \int_{t_1}^{t} P(x)  dx. \\
&= \int_{q \in Q} g(q) \pi(q,t')v(q,t') dq -   \int_{t_1}^{t'} P(x)  dx. \\
&= p(t')
\end{align*}

For case 2, we can think the tail terms as $- v(t_2) + \int_{t}^{t_2} P(x)  dx = - u(t_2) + \int_{t}^{t_2} P(x)  dx = - u(t_1) - \int_{t_1}^{t} P(x)  dx$. Since $u(t_1)$ is a constant, this proof still ho.


\end{proof}

==> case3.tex <==
\section{Optimal Mechanism for Case 3 ($V_L< v(t_2)< V_H$)}
In this section, we consider the case where $V_L< v(t_2)< V_H$. The techniques used to handle previous two cases do not apply to this case, as we cannot use either $t_1$ or $t_2$ as the reference point. Instead, we use both $t_1$ and $t_2$ as reference points. We will first derive a different revenue function that features a new virtual value function. The new virtual value function is a convex combination of both the lower and the upper virtual value functions with a carefully chosen coefficient. Then we prove that the threshold mechanism defined according to the new virtual value function could achieve the maximum possible revenue.
\begin{lemma}
    \label{lem:case_3}
    If $V_L < v(t_2) < V_H$, define $\widetilde{\phi}(t) = c \underline{\phi}(t) + (1-c) \bar{\phi}(t) $ to be the combined virtual value function, where $c \in (0,1) $ is a constant that satisfies
    \begin{gather*}
        \int_{t_1}^{t_2}\int_{q:\rho(q)\ge-\widetilde{\phi}(t)} g(q)  v_1(q)\,\dd q \dd t = v(t_2).
    \end{gather*}
    Let $\widetilde{\phi}^+(t)$ be the ironed version of $\widetilde{\phi}(t)$.
    The optimal mechanism is the threshold mechanism $\pi^*$ with threshold $\theta^*(t) =-\widetilde{\phi}^+(t)$ for each type $t$.
    The payment is determined by the following equation and is monotone non-decreasing in $t$ when $F(t)\leq c$ and monotone non-increasing when $F(t)>c$:
    \begin{gather*}
        {p}^*(t) = \int_{q \in Q} g(q) {\pi}^*(q,t)v(q,t) \,\dd q -  \int_{t_1}^{t} P_{{\pi}^*}(x)\,\dd x.
    \end{gather*}     
\end{lemma}
The proof of Lemma \ref{lem:case_3} consists of two cases, which depends on whether the function $\widetilde{\phi}(t)$ is regular or not. 
%When $\widetilde{\phi}(t)$ is regular (i.e., $\widetilde{\phi}(t)$ is monotone non-decreasing), we still use similar techniques for handling the other two cases. But we will need to use both $t_1$ and $t_2$ as reference points. When $\widetilde{\phi}(t)$ is irregular, we also apply the ironing trick and show that the threshold mechanism corresponding  $\widetilde{\phi}^+(t)$ is optimal.
But before proving the optimality of our mechanism, we will first argue that the constant $c$ described in Lemma \ref{lem:case_3} actually exists. Then we will show that the proposed threshold mechanism is feasible.

\begin{lemma}
    \label{lem:existence_of_C}
    If $V_L < v(t_2) < V_H$, there exists a constant $C\in (0,1)$, such that
    \begin{gather*}
        \int_{t_1}^{t_2}\int_{q:\rho(q)\ge-\widetilde{\phi}(t)} g(q)  v_1(q)\,\dd q \dd t = v(t_2).
    \end{gather*}
\end{lemma}
\begin{proof}
    Remark \ref{remark:case_2_condition_eq} implies that $v(t_2)<V_H$ is equivalent to the following:
    \begin{gather}
        v(t_1) < -  \int_{t_1}^{t_2} \int_{q: \rho(q) \leq \bar{\theta}_x}  g(q) v_1(q) \,\dd q  \dd x.
    \end{gather}
    The right-hand side of the above inequality is clearly non-positive. Thus $\max \{v(t_1), 0 \}=0$, and the condition $V_L < v(t_2) < V_H$ can be written as:
    \begin{gather*}
        \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) \,\dd q\dd x < v(t_2) <  \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) \,\dd q\dd x.
    \end{gather*}
    When $C = 0$, we have $\underline{\theta}_x=-\underline{\phi}(t)=-\widetilde{\phi}(t)$ and
    \begin{gather*}
        \int_{t_1}^{t_2}\int_{q:\rho(q)\ge-\widetilde{\phi}(t)} g(q)  v_1(q)\,\dd q \dd t = \int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\underline{\phi}(t)} g(q) v_1(q) \,\dd q\dd t < v(t_2).
    \end{gather*}
    When $C = 1$, we have $\bar{\theta}_x=-\bar{\phi}(t)=-\widetilde{\phi}(t)$ and
    \begin{gather*}
        \int_{t_1}^{t_2} \int_{\rho(q) \geq - C \underline{\phi}(t) - (1-C) \bar{\phi}(t)  } g(q) v_1(q) dq dt = \int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\bar{\phi}(t)} g(q) v_1(q) \,\dd q\dd t > v(t_2).
    \end{gather*}    
    \sz{
        We can write 
        \begin{align*}
            \int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\widetilde{\phi}(t)} g(q) v_1(q) \,\dd q\dd t &= \int_{t_1}^{t_2} \int_{\rho(q) \geq - C \underline{\phi}(t) - (1-C) \bar{\phi}(t)  } g(q) v_1(q) dq dt \\
            &= \int_{t_1}^{t_2} \int_{\rho(q) \geq - (t+\frac{F(t)}{f(t)}+\frac{C}{f(t)}) } g(q) v_1(q) dq dt \\
            &= Y(C)
        \end{align*}    
        Now, we are going to show this function is continuous on $C \in (0,1)$, because supposing $\epsilon$ is positive,
        \begin{align*}  
            Y(C+\epsilon) - Y(C)  &= \int_{t_1}^{t_2} \int_{\rho(q) \geq - (t+\frac{F(t)}{f(t)}+\frac{C+\epsilon}{f(t)}) } g(q) v_1(q) dq dt - \int_{t_1}^{t_2} \int_{\rho(q) \geq - (t+\frac{F(t)}{f(t)}+\frac{C}{f(t)}) } g(q) v_1(q) dq dt\\
            &= \int_{t_1}^{t_2} \int_{\rho(q) \geq - (t+\frac{F(t)}{f(t)}+\frac{C+\epsilon}{f(t)}) }^{\rho(q) < - (t+\frac{F(t)}{f(t)}+\frac{C}{f(t)}) } g(q) v_1(q) dq dt
        \end{align*}   
        \begin{align*}  
            Y(C) - Y(C-\epsilon)  &= \int_{t_1}^{t_2} \int_{\rho(q) \geq - (t+\frac{F(t)}{f(t)}+\frac{C}{f(t)}) } g(q) v_1(q) dq dt - \int_{t_1}^{t_2} \int_{\rho(q) \geq - (t+\frac{F(t)}{f(t)}+\frac{C -\epsilon}{f(t)}) } g(q) v_1(q) dq dt\\
            &= \int_{t_1}^{t_2} \int_{\rho(q) \geq - (t+\frac{F(t)}{f(t)}+\frac{C}{f(t)}) }^{\rho(q) < - (t+\frac{F(t)}{f(t)}+\frac{C-\epsilon}{f(t)}) } g(q) v_1(q) dq dt
        \end{align*}    
        
        If $t+\frac{F(t)}{f(t)}$ is a constant, it is fine, since $\frac{C}{f(t)}$ is not a constant.
        
        For example, if $\rho(q)$ is a constant, the concern is that $\lim_{\varepsilon \to 0} Y(C+\epsilon) - Y(C) = 0$ may not be 0. There are three cases.
        1. Given any $\rho(q)$ not in the range of $q$ at all. $Y(C)$ will just be a constant over its domain, which is continuous.
        
        2. If $\rho(q)$ is in the range of $q$, suppose $\rho(q) = - (t+\frac{F(t)}{f(t)}+\frac{C}{f(t)})$. It is true that $Y(C)$ will suddenly increase at $\rho(q) = - (t+\frac{F(t)}{f(t)}+\frac{C}{f(t)}) $. But its right limits $\lim_{\varepsilon \to 0} Y(C+\epsilon) - Y(C) = 0$ is still 0. 
        
        However, the left limits $\lim_{\varepsilon \to 0} Y(C) - Y(C- \epsilon) > 0$. 
        
        So, this function is not continuous and it is actually common existed even when $\rho(q)$ is not a constant. 
        Thus, we need partial recommendations on the boundary cases.
        Define $C$ as,
        
        $$  \argmax_{C}Y(C) =\{ C \mid \int_{t_1}^{t_2} \int_{\rho(q) \geq -(t+\frac{F(t)}{f(t)}+\frac{C}{f(t)})  } g(q) v_1(q)\, \dd q \dd t \leq v(t_2) \}$$
        And define $D$ as the following,
        $$D =  \frac{v(t_2) - \int_{t_1}^{t_2} \int_{\rho(q) \geq - (t+\frac{F(t)}{f(t)}+\frac{C}{f(t)})  } g(q) v_1(q)\, \dd q \dd t }{\int_{\rho(q) = - (t+\frac{F(t)}{f(t)}+\frac{C}{f(t)}) \bar{\phi}(t)  } g(q) v_1(q)\, \dd q \dd t }$$
        
        $D$ is a constant where $D \in (0,1)$. $D > 0$ because we have both the numerator and denominator positive in above equation. Since $C$ is from argmax, this means the numerator is greater than denominator. Otherwise, $C$ can be larger to include the denominator and still be less than $v(t_2)$
        
        
        Our recommendation mechanism will be
        \begin{gather*}
            \pi(q,t)=
            \begin{cases}
                1 & \text{ if } \rho(q) > -\widetilde{\phi}^+(t)\\
                D & \text{ if } \rho(q) = -\widetilde{\phi}^+(t)\\
                0 & \text{ otherwise}
            \end{cases}.
        \end{gather*}
        
        %     \begin{align*}  C(t-\frac{1-F(t)}{f(t)}) + (1-C)(t+\frac{F(t)}{f(t)}) &= Ct -C\frac{1-F(t)}{f(t)} + (1-C)(t)+(1-C)\frac{F(t)}{f(t)}) \\
        %   &=  Ct -C\frac{1}{f(t)} +C\frac{F(t)}{f(t)} +  (1-C)(t)+(1-C)\frac{F(t)}{f(t)})
        %   = t + \frac{F(t)}{f(t)} - \frac{1}{f(t)}
        %     \end{align*} 
        
        
    }
    
    Since $\int_{t_1}^{t_2} \int_{\rho(q) \geq - \widetilde{\phi}(t)} g(q) v_1(q) \,\dd q\dd t$ is continuous in $C$ \swr{Reealy?}, we must have $C\in(0,1)$ such that $$    \int_{t_1}^{t_2} \int_{\rho(q) \geq - C \underline{\phi}(t) - (1-C) \bar{\phi}(t)  } g(q) v_1(q)\, \dd q \dd t = v(t_2) $$.
\end{proof}

Lemma \ref{lem:existence_of_C} implies that the mechanism proposed in Lemma \ref{lem:case_3} exists. Now we show that it is also feasible.
\begin{lemma}
    \label{lem:case_3_feasible}
    The mechanism $(\widetilde{\pi}, \widetilde{p})$ is feasible.
\end{lemma}
\begin{proof}
    To prove Lemma \ref{lem:case_3_feasible}, it suffices to show that mechanism $(\widetilde{\pi}, \widetilde{p})$ satisfies constraints \eqref{eq:signal-monotonicity}, \eqref{eq:buyer-utility-identify2}, \eqref{eq:ir-t2}, and \eqref{eq:non-negativity}. By definition,
    \begin{gather*}
        P_{\widetilde{\pi}}(t) = \int_{q:\rho(q)\ge \widetilde{\theta}_t} g(q) v_1(q) \,\dd q.
    \end{gather*}
    Since $\widetilde{\phi}^+(t)$ is non-decreasing, $\widetilde{\theta}_t=-\widetilde{\phi}^+(t)$ is non-increasing in $t$. Thus the integral domain of $P_{\widetilde{\pi}}(t)$ gets larger as $t$ increases, So $P_{\widetilde{\pi}}(t)$ is non-decreasing, satisfying constraint \eqref{eq:signal-monotonicity}.
    
    To show that $\widetilde{\phi}^+(t)$ satisfies constraint \eqref{eq:buyer-utility-identify2}, note that
    \begin{gather*}
        u(t)=\int_{q \in Q}   g(q) \pi(q,t)v(q,t_1) \,\dd q -p(t)=\int_{t_1}^{t} P_{\widetilde{\pi}}(x)\,\dd x.
    \end{gather*}
    Thus $u(t_1)=0$ and 
    \begin{gather*}
        u(t)=u(t_1)+\int_{t_1}^{t} P_{\widetilde{\pi}}(x)\,\dd x.
    \end{gather*}
    As for constraint \eqref{eq:ir-t2}, we already have $u(t_1)=0$. And
    \begin{gather*}
        u(t_2) = \int_{t_1}^{t_2} P_{\widetilde{\pi}}(x)\,\dd x = \int_{t_1}^{t_2} \int_{\widetilde{\phi}_q(t)\ge C } g(q) v_1(q) \,\dd q \dd t = v(t_2),
    \end{gather*}
    where the last equation is the definition of the constant $C$.
    
    Finally, we show that the payment is non-negative, i.e., mechanism $(\widetilde{\pi}, \widetilde{p})$ satisfies constraint \eqref{eq:non-negativity}. We claim that $p(t)$ is monotone non-decreasing when $F(t)\le C$, and monotone non-increasing when $F(t)\ge C$.
    
    Note that
    \begin{gather*}
        \widetilde{\phi}(t)=C \underline{\phi}(t) + (1-C) \bar{\phi}(t)=t-\frac{C-F(t)}{f(t)}.
    \end{gather*}
    Let $t_C$ be such that $F(t_C)=C$. So for any $t$ with $t<t_C$, we have $\widetilde{\phi}(t)<t$, and for any $t$ with $t>t_C$, we have $\widetilde{\phi}(t)>t$. We will show that this is also true for the ironed function $\widetilde{\phi}^+(t)$. 
    
    In fact, $t_C$ must lie in a non-ironed interval. Otherwise, if $t_C$ is in an ironed interval $(a,b)$, then at least one of the points $(a, \widetilde{H}(a))$ and $(b, \widetilde{H}(b))$ lies strictly below the tangent line of function $\widetilde{\phi}(t)$ at point $(z_C, \widetilde{H}(z_C))$, where $z_C=F(t_C)$ and $\widehat{H}(\cdot)$ is the corresponding function when ironing $\widetilde{\phi}(t)$. Assume, without loss of generality, that the point is $(a, \widetilde{H}(a))$. Then there exists $s\in (a, z_C)$ such that $\widetilde{H}'(s)=\frac{\widetilde{H}(z_C)-\widetilde{H}(a)}{z_C-a}$. This means $\widetilde{H}'(s)> \widetilde{H}'(z_C)$ since $(a, \widetilde{H}(a))$ is strictly below the tangent line at $(z_C, \widetilde{H}(z_C))$. This contradicts the fact that $\widetilde{\phi}(t)<t, \forall t<t_C$, implying that $t_C$ is in a non-ironed interval. Also, we have $\widetilde{\phi}^+(t_C)=t_C$.
    
    For any $t<t_C$, if $t$ is in a non-ironed interval, then $\widetilde{\phi}^+(t)=\widetilde{\phi}(t)<t$. If $t$ is in an ironed interval $I=(a,b)$, then we know that $t_C\not\in I$ as $t_C$ is in a non-ironed interval. Since $\widetilde{H}(\cdot)$ is linear in $I$, we have $\widetilde{\phi}^+(t)=\widetilde{\phi}^+(a)=\widetilde{\phi}(a)<a<t$. The case where $t>t_C$ follows from similar arguments.
    
    For any $t<t_C$, let $t'$ be any number in the interval $[\widetilde{\phi}^+(t), t]$. Thus $\widetilde{\phi}^+(t)\ge \widetilde{\phi}^+(t')$. And
    \begin{align*}
        \widetilde{p}(t)-\widetilde{p}(t')=&\int_{q\in Q} g(q) \widetilde{\pi}(q,t)v(q,t)\,\dd q -\int_{q\in Q} g(q) \widetilde{\pi}(q,t')v(q,t')\,\dd q -  \int_{t'}^{t} P_{\widetilde{\pi}}(x)  \,\dd x\\
        =&\int_{q:\rho(q)\ge \widetilde{\theta}_t}g(q)v(q,t)\,\dd q-\int_{q:\rho(q)\ge \widetilde{\theta}_{t'}}g(q)v(q,t')\,\dd q-  \int_{t'}^{t} P_{\widetilde{\pi}}(x)  \,\dd x.
    \end{align*}
    When $\rho(q)\ge \widetilde{\theta}_{t}=-\widetilde{\phi}^+(t)$, we have $v(q,t')=v_1(q)[t'+\rho(q)]\ge v_1(q)[t'-\widetilde{\phi}^+(t)]\ge 0$, where the last inequality is because of the choice of $t'$. So the second term in the above equation satisfies:
    \begin{align*}
        \int_{q:\rho(q)\ge \widetilde{\theta}_{t'}}g(q)v(q,t')\,\dd q=&\int_{q:\rho(q)\ge \widetilde{\theta}_{t}}g(q)v(q,t')\,\dd q-\int_{q:\widetilde{\theta}_{t}\le\rho(q)\le \widetilde{\theta}_{t'}}g(q)v(q,t')\,\dd q\\
        \ge&\int_{q:\rho(q)\ge \widetilde{\theta}_{t}}g(q)v(q,t')\,\dd q.
    \end{align*}
    Thus,
    \begin{align*}
        \widetilde{p}(t)-\widetilde{p}(t')\ge&\int_{q:\rho(q)\ge \widetilde{\theta}_t}g(q)v(q,t)\,\dd q-\int_{q:\rho(q)\ge \widetilde{\theta}_{t}}g(q)v(q,t')\,\dd q-  \int_{t'}^{t} P_{\widetilde{\pi}}(x)  \,\dd x\\
        =&\int_{q:\rho(q)\ge \widetilde{\theta}_t}g(q)v_1(q)(t-t')\,\dd q-\int_{t'}^{t} P_{\widetilde{\pi}}(x)  \,\dd x\\
        =&(t-t')P_{\widetilde{\pi}}(t)-\int_{t'}^{t} P_{\widetilde{\pi}}(x)  \,\dd x\\
        \ge &0,
    \end{align*}
    where the last inequality is due to the monotonicity of $P_{\widetilde{\pi}}(t)$.
    
    Therefore, the payment function $p(t)$ is monotone non-decreasing in the interval $[\underline{\phi}(t),t]$. Since the set of intervals $\{[\underline{\phi}(t),t]\mid t\in T\}$ covers $[t_1,t_C]$, we conclude that $p(t)$ is monotone non-decreasing in $[t_1,t_C]$.
    
    Using similar analyses, we can show that $p(t)$ is monotone non-increasing in the interval $[t_C,t_2]$. Therefore, to prove that $p(t)\ge 0$ for all $t\in T$, it suffices to show that $p(t_1)\ge0$ and $p(t_2)\ge 0$. Indeed, we have
    \begin{align*}
        \widetilde{p}(t_1) = \int_{q \in Q} \widetilde{\pi}(q,t_1) g(q)  v(q,t_1)\, \dd q - u(t_1) = \int_{q:\rho(q)\geq\widetilde{\theta}_{t_1}}  g(q)  v(q,t_1)\, \dd q \geq 0.
    \end{align*}
    The inequality holds because when $\rho(q)\ge\widetilde{\theta}_{t_1}=-\widetilde{\phi}^+(t_1)\ge -t_1$, we have $v(q,t_1)=v_1(q)[t_1+\rho(q)]\ge 0$. And
    \begin{align*}
        \widetilde{p}(t_2) =& \int_{q \in Q} \widetilde{\pi}(q,t_2) g(q)  v(q,t_2)\, \dd q - u(t_2)\\
        =&\int_{\rho(q) \geq \widetilde{\theta}_{t_2} } g(q) v_1(q)[t_2+\rho(q)]\, \dd q -\int_{q \in Q} g(q) v_1(q)[t_2 + \rho(q)]\,\dd q\\
        =&-\int_{\rho(q) < \widetilde{\theta}_{t_2} } g(q) v_1(q)[t_2+\rho(q)]\, \dd q\\
        \ge& 0,
    \end{align*}
    where the inequality is because $\rho(q) < \widetilde{\theta}_{t_2}=-\widetilde{\phi}^+(t_2)\le -t_2$, 
\end{proof}

Now we are ready to prove the regular case of Lemma \ref{lem:case_3}.
\begin{proof}[Proof of Lemma \ref{lem:case_3} (regular case)]
    Different from the proofs of Lemma \ref{lem:optimal-case1} and \ref{lem:optimal-case2}, in this proof, we will derive a different revenue function by using both $t_1$ and $t_2$ as reference points. Let $\beta\in[0,1]$ be a real number, and write the revenue as a convex combination of Equation \eqref{eq:revenue-1} and \eqref{eq:revenue-2}:
    \begin{align*}
        REV(\pi, p)=&\beta \left[\int_{q \in Q} g(q)\int_{t_1}^{t_2} f(t)\pi(q,t) v_1(q) \left[\underline{\phi}(t) + \rho(q)\right]\,\dd t \, \dd q -u(t_1) \right] \\
        &+ (1-\beta)  \left[\int_{q \in Q} g(q) \int_{t_1}^{t_2} f(t)\pi(q,t)v_1(q) \left[ \bar{\phi}(t) + \rho(q)\right]\,\mathrm{d}t  \mathrm{d}q -u(t_2) \right] \\
        = & \int_{t_1}^{t_2}\int_{q\in Q} \left[\beta \underline{\phi}(t) + (1-\beta)\bar{\phi}(t) - \rho(q)\right] \pi(q,t) f(t) g(q) v_1(q)\,\dd q\dd t - \beta u(t_1) - (1-\beta)u(t_2).
    \end{align*}
    Since Equation \eqref{eq:revenue-1} and \eqref{eq:revenue-2} are just different representations of the revenue of any mechanism $(\pi,p)$, the above equation holds for any $\beta$. Choose $\beta$ to be the constant $C$ described in Lemma \ref{lem:case_3}, and we have:
    \begin{gather}
        \label{eq:revenue-3}
        REV(\pi, p)=\int_{t_1}^{t_2}\int_{q\in Q} \left[\widetilde{\phi}(t) + \rho(q)\right] \pi(q,t) f(t) g(q) v_1(q)\,\dd q\dd t - C u(t_1) - (1-C)u(t_2).
    \end{gather}
    
    Now consider the mechanism $(\widetilde{\pi}, \widetilde{p})$. According to Lemma \ref{lem:case_3_feasible}, this mechanism is feasible. Since the function $\widetilde{\phi}(t)$ is regular, we have $\widetilde{\phi}^+(t)=\widetilde{\phi}(t),\forall t\in T$. Mechanism $(\widetilde{\pi}, \widetilde{p})$ clearly maximizes the first term of Equation \eqref{eq:revenue-3} as $\widetilde{\pi}(q, t)=1$ whenever $\rho(q)\ge \widetilde{\theta}_t= -\widetilde{\phi}^+(t)=-\widetilde{\phi}(t)$ and $0$ whenever $\rho(q)< \widetilde{\theta}_t$. Furthermore, according to the proof of Lemma \ref{lem:case_3_feasible}, we have $u(t_1)=0$ and $u(t_2)=v(t_2)$. These also maximize the last two terms of Equation \eqref{eq:revenue-3} as the feasibility constraint \eqref{eq:ir-t2} requires $u(t_1)\ge0$ and $u(t_2)\ge v(t_2)$. Therefore, we can conclude that mechanism $(\widetilde{\pi}, \widetilde{p})$ maximizes Equation \eqref{eq:revenue-3}, hence optimal.
\end{proof}

To prove for the irregular case, we still use the ironing trick, and show that the mechanism $(\widetilde{\pi}, \widetilde{p})$ (defined according to $\widetilde{\phi}^+(t)$) achieves the same revenue as the entry-wise maximization mechanism (though infeasible) defined according to non-ironed $\widetilde{\phi}(t)$.

\begin{proof}[Proof of Lemma \ref{lem:case_3} (irregular case)]
    Let $(\pi, p)$ be the feasible mechanism.Let $\widetilde{H}(\cdot),\widetilde{L}(\cdot),\widetilde{h}(\cdot),\widetilde{l}(\cdot)$ be the corresponding functions when ironing the function $\widetilde{\phi}(t)$. Applying Equation \eqref{eq:revenue-3} to mechanism $(\pi^*, p^*)$, we have
    \begin{gather*}
        REV(\pi, p)=\int_{t_1}^{t_2}\int_{q\in Q} \left[\widetilde{\phi}(t) + \rho(q)\right] \pi(q,t) f(t) g(q) v_1(q)\,\dd q\dd t - C u(t_1) - (1-C)u(t_2).
    \end{gather*}
    
    By definition, we have $\widetilde{h}(F(t))=\widetilde{\phi}(t)$ and $\widetilde{l}(F(t))=\widetilde{\phi}^+(t)$. So the first term in the above equation can be written as
    \begin{align*}
        &\int_{t_1}^{t_2}\int_{q\in Q} \left[\widetilde{\phi}(t) + \rho(q)\right] \pi(q,t) f(t) g(q) v_1(q)\,\dd q\dd t\\
        =&\int_{t_1}^{t_2}\int_{q\in Q} \left[\widetilde{\phi}^+(t) + \rho(q)\right] \pi(q,t) f(t) g(q) v_1(q)\,\dd q\dd t \\
        &+\int_{t_1}^{t_2}\int_{q\in Q} \left[\widetilde{h}(F(t)) - \widetilde{l}(F(t))\right] \pi(q,t) f(t) g(q) v_1(q)\,\dd q\dd t.
    \end{align*}
    Using integration by parts, we can simplify the second term as follows:
    \begin{align*}
        & \int_{t_1}^{t_2}\int_{q\in Q} \left[\widetilde{h}(F(t)) - \widetilde{l}(F(t))\right] \pi(q,t) f(t) g(q) v_1(q)\,\dd q\dd t \\
        =& \int_{t_1}^{t_2} \left[\widetilde{h}(F(t))- \widetilde{l}(F(t))\right] P_{\pi}(t) \,\dd F(t) \\
        =& \left.\left[\widetilde{H}(F(t))- \widetilde{L}(F(t))\right] P_{\pi}(t) \right|_{t_1}^{t_2}  - \int_{t_1}^{t_2} \left[\widetilde{H}(F(t))- \widetilde{L}(F(t))\right] \,\dd P_{\pi}(t) \\
    \end{align*}
    Because $\widetilde{L}$ is the ``convex hull'' of $\widetilde{H}$, so $\widetilde{L}(0) = \widetilde{H}(0)$ and $\widetilde{L}(1) = \widetilde{H}(1)$. Thus the first term above is simply $0$, and we have 
    \begin{align}
        REV(\pi, p)=&\int_{t_1}^{t_2}\int_{q\in Q} \left[\widetilde{\phi}(t) + \rho(q)\right] \pi(q,t) f(t) g(q) v_1(q)\,\dd q\dd t- C u(t_1) - (1-C)u(t_2)\nonumber\\
        = &\int_{t_1}^{t_2}\int_{q\in Q} \left[\widetilde{\phi}^+(t) + \rho(q)\right] \pi(q,t) f(t) g(q) v_1(q)\,\dd q\dd t \nonumber\\ 
        & - \int_{t_1}^{t_2} \left[\widetilde{H}(F(t))- \widetilde{L}(F(t))\right] \,\dd P_{\pi}(t)- C u(t_1) - (1-C)u(t_2)\label{eq:new-rev-3}
    \end{align}
    
    Now consider mechanism $(\widetilde{\pi}, \widetilde{p})$, which is feasible according to Lemma \ref{lem:case_3_feasible}. This mechanism clearly maximizes the first term in Equation \eqref{eq:new-rev-3} as $\widetilde{\pi}(q, t)=1$ if and only if $\widetilde{\phi}(t) + \rho(q)\ge 0$. We also have $u(t_1)=0$ and $u(t_2)=v(t_2)$ as shown in the proof of Lemma \ref{lem:case_3_feasible}, which also optimizes the last two terms as constraint \eqref{eq:ir-t2} requires $u(t_1)\ge 0$ and $u(t_2)\ge v(t_2)$. As for the second term, note that $\widetilde{H}(F(t))- \widetilde{L}(F(t))\ge 0$ by definition, and $\dd P_{\pi}(t)\ge0$ for any feasible mechanism. Thus the second term is always non-negative. However, we claim that with mechanism $(\widetilde{\pi}, \widetilde{p})$, this term is actually 0. The only interesting case is when $\widetilde{H}(F(t))- \widetilde{L}(F(t))\ne 0$. In this case, $t$ must lie in an ironed interval $I$. Thus $\widetilde{L}(z)$ is linear in the interval $I$, where $z=F(t)$. This implies that $\widetilde{\phi}^+(t)=\widetilde{l}(z)=\widetilde{L}'(z)$ is constant. So
    \begin{gather*}
        P_{\widetilde{\pi}}(t)=\int_{ q \in Q}\widetilde{\pi}(q,t)g(q)v_1(q)\,\dd q=\int_{ q :\rho(q)\ge -\widetilde{\phi}^+(t)}g(q)v_1(q)\,\dd q
    \end{gather*}
    is also constant in the interval $I$, which leads to $\dd P_{\widetilde{\pi}}(t)$ being 0.
    
    Therefore, the mechanism $(\widetilde{\pi}, \widetilde{p})$ optimizes all the 4 terms in Equation \eqref{eq:new-rev-3} simultaneously, thus is the optimal feasible mechanism.    
\end{proof}

==> discrete.tex <==
\section{The Discrete Case}





\begin{definition}[Upper/Lower-Boundary Virtual Value Function]
We call $\underline{\varphi}(t_k) = t_k - (t_{k+1}-t_{k})\frac{1-F(t_k)}{f(t_k)}$  the \emph{lower-boundary} virtual value function and call  $\bar{\varphi}(t_k) = t_k + (t_k - t_{k-1})\frac{F(t_{k-1})}{f(t_k)} $   the \emph{upper-boundary} virtual value function.  We say a virtual value function, upper-boundary or lower-boundary, is regular if it is monotone non-decreasing in $t$. 
\end{definition}

\begin{theorem}\label{dis-theorem}

\begin{enumerate}
\item If  $v(t_N) < \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \underline{\theta}(t_{i-1}) }g(q)v_1(q)$ and $\underline{\varphi}(t_k)$ is monotone non-decreasing, the optimal information selling mechanism is a threshold mechanism on $\rho(q)$ with threshold $\underline{\theta}(t_k) =  -\underline{\varphi}(t_k) $ for each type $t$.  The payment is determined by the following identity and is monotone non-decreasing in $t$: $$p(t_k) = \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k)  - \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1})$$ 
\item If $v(t_N) \geq \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q)$ and $\bar{\varphi}(t_k)$ is monotone non-decreasing, the optimal information selling mechanism is a threshold mechanism  on $\rho(q)$ with threshold $\theta(t_k) =  -\bar{\varphi}(t_k) $ for each type $t$. The payment is determined by the following identity and is monotone non-increasing in $t$:
$$p(t_k) = \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k) -v(t_N) + \sum_{i=k+1}^N(t_i - t_{i-1})P(t_{i})$$   
\item    For $v(t_N)$ not in the above 2 cases where $ \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \underline{\theta}(t_{i-1})} \\ g(q)v_1(q) \leq v(t_N) < \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q)$ (or equivalently,  $ -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \underline{\theta}(t_{i-1}) }g(q)v_1(q)  \leq  v(t_1) < -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \bar{\theta}(t_{i}) }g(q)v_1(q)$)and $\widetilde{\varphi}_q(t_i) = f(t_i)  \frac{[\underline{\varphi}(t_i) + \rho(q)]}{(t_{i+1}-t_{i}) }$ is non-decreasing in t for any q, the optimal mechanism is a threshold mechanism on $\rho(q)$ with threshold $\theta(t_i) = t_i+ (t_{i+1}-t_{i})\frac{C-F(t_i)}{f(t_i)} $, where $C \in (0,1]$ is a constant and satisfies  $\sum_t\sum_{q:}_{ \widetilde{\varphi}_q(t) + 1 >= C } g(q)  v_1(q) (t_{i+1}-t_{i})   = v(t_N)$. 
 

The payment function is,
\begin{gather*}
p(t_k) =
\begin{cases}
\sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k)  - \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1}) & \text{for } F(t_k) \leq C\\
\sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k) -v(t_N) + \sum_{i=k+1}^N(t_i - t_{i-1})P(t_{i}) & \text{for } F(t_k) > C
\end{cases}
\end{gather*}

$P(t_k)$ is monotone non-decreasing in t when $F(t) \leq C $ and monotone non-increasing when $F(t) > C$.
  
 
 
 


\end{enumerate}
\end{theorem}
 
 
 
 \todo{add a few examples and derive their optimal scheme and see what it is like. $v(q,t) = t*q - 1$ where }
 
 \todo{add a proof sketch here...}  
 
 \sz{I find a proof sketch will be very hard to explain, because the mechanism formula itself is hard to explain. This example can only give a procedure impression to readers, instead of not any intuitive sense why this $\pi(q,t)$ and $p(t)$ is optimal. 
 
 I think pointing out some interesting points like recommending buying things with $v(q,t) < 0$ and same policy will induce same payment may be better to attract readers.}
 
 \hf{why still discrete? We will need a closed-form mechanism for CONTINUOUS cases. We are looking for closed form characterization, some statement like "the threshold for type $t$ is $2t^2 - 5t$", while not a table for different $t$. These tables are not insightful as they can be computed from an LP, so why it is useful to list them here. Please see what Myerson wrote at page 10 here of his Optimal Auction Design paper. That is what we are looking for.}
 
 In the table, we define an example to show how this algorithm works.  Define $v_1(q) = q, \; v_0(q) = -6$, we have $v(q,t) = q*t - 6$.  And both $t$ and $q$ are uniformly distributed. Recall, $\rho(q) = \frac{v_0(q)}{v_1(q)}$ We have this value table. 
 
 

\begin{table}[!htb]
    % \caption{Global caption}
    \begin{minipage}{.5\linewidth}
      \caption{Value table}
      \centering
        \begin{tabular}{|c| c| c| c|} 
        \hline
        & $t_1 = 3$ & $t_2 = 4 $ & $t_3 = 5$ \\ [0.5ex] 
        \hline
        $q_1 = 1, \; \rho(q_1) = -6$ & -3 & -2 & -1 \\ 
        \hline
        $q_2 = 2, \; \rho(q_2) = -3$ & 0 & 2 & 4 \\
        \hline
        $q_3 = 3, \; \rho(q_3) = -2$ & 3 & 6 & 9 \\
        \hline
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        \caption{Threshold table}
            \begin{tabular}{|c| c| c| c|} 
            \hline
            & $t_1 = 3$ & $t_2 = 4 $ & $t_3 = 5$ \\ [0.5ex] 
            \hline
            $\bar{\theta}(t_k)$& -3 & -5 & -7 \\ [0.5ex] 
            \hline
            \end{tabular}
    \end{minipage} 
\end{table}

This is a instance of theorem \ref{dis-theorem} case 2. Based on $\bar{\theta}(t_k) = - \bar{\varphi}(t_k) = -( t_k + (t_k - t_{k-1})\frac{F(t_{k-1})}{f(t_k)} )$, we can get the threshold table.

In this threshold policy, if $\rho(q)$ passes the threshold, the recommendation policy will recommend $purchase$ with probability 1, otherwise, with probability 0. Base on payment function $p(t_k) = \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k) -v(t_N) + \sum_{i=k+1}^N(t_i - t_{i-1})\sum_{q\in Q} g(q) \pi(q,t_i)v_1(q)  $. The optimal recommendation policy and the payment are the following.


\begin{table}[!htb]
    % \caption{Global caption}
    \begin{minipage}{.5\linewidth}
      \caption{Recommendation Policy}
      \centering
        \begin{tabular}{|c| c| c| c|} 
        \hline
        & $t_1 = 3$ & $t_2 = 4 $ & $t_3 = 5$ \\ [0.5ex] 
        \hline
        $q_1 = 1, \; \rho(q_1) = -6$ & 0 & 0 & 1 \\ 
        \hline
        $q_2 = 2, \; \rho(q_2) = -3$ & 1 & 1 & 1 \\
        \hline
        $q_3 = 3, \; \rho(q_3) = -2$ & 1 & 1 & 1 \\
        \hline
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        \caption{Payment}
            \begin{tabular}{|c| c| c| c|} 
            \hline
            & $t_1 = 3$ & $t_2 = 4 $ & $t_3 = 5$ \\ [0.5ex] 
            \hline
            $p(t)$& $\frac{2}{3}$ & $\frac{2}{3}$ & 0 \\ [0.5ex] 
            \hline
            \end{tabular}
    \end{minipage} 
\end{table}

We can see although $v(q_1,t_3) = -1$, the optimal way is to recommend $purchase$ it without charging $t_3$ anything since the $\rho(q_1)$ passes the threshold defined on virtual value $\bar{\varphi}(t_3)$. Also, for $t_1$ and $t_2$, because they are recommending the same policy, the $p(t)$ is the same, which will also be proved later.



%%%%%%-------------Theorem and Examples-------------%%%%%%%%%%%%%%%%


Now, we are going to extend our theorem to discrete cases \cite{soton263443}, where things will get different. For example, the $P(t)$ will no longer be the derivative of utility function $u(t)$ because t are not continuous anymore. 

We first introduce the notations. We still model the value function $v(q,t) = v_1(q)t+v_0(q)$ and is an increasing function in $q$ and $t$.

The value $q$ is drawn from a finite set $Q = \{ q_i | i = 1,...,M \}$ according to a distribution $g_i$. We assume that $q_1 < q_2 < ... < q_M$. The distribution $g$ has the probabilities $g(q)$ for each $q_i \in Q$ s.t. $\Pr[q = q_i ] = g(q)$.

The value $t$ is drawn from a finite set $T = \{ t_i | i = 1,...,N \}$ according to a distribution $f$. We assume that $t_1 < t_2 < ... < t_N$. The distribution $f$ has the probabilities $f(t_i)$ for each $t_i \in T$ s.t. $\Pr[t = t_i ] = f(t)$.

Now, define the new goal and the constraints, they are the same except we use summation here instead of integral.

\begin{equation}\label{dis-cons:obj}
\text{ Seller's Objective: } \quad \max_{\pi, p} \sum_{t\in T} f(t) p(t)   
\end{equation}

\begin{equation}\label{dis-cons:obedience}
\text{Obedience: } \quad  \sum_{q \in Q} \pi(q, t) \cdot g(q) v(q,t)  \geq   \max \{ 0, v(t) \}, \, \, \, \forall t \in [T]
\end{equation}

\begin{equation}\label{dis-cons:IC}
\text{IC: } \quad \sum_{q \in Q} \pi(q, t) \cdot g(q) v(q,t)  - p(t) \geq \sum_{q \in Q} \pi(q, t') \cdot g(q) v(q,t)   - p(t'), \, \, \, \forall, t, t' \in [T] 
\end{equation}

\begin{equation}\label{dis-cons:IR}
    \text{IR Constraint: } \quad \sum_{q \in Q} \pi(q, t) \cdot g(q) v(q,t)  - p(t) \geq  \max \{ 0, v(t) \}, \, \, \, \forall, t  \in [T]  
\end{equation} 

Lemma \ref{lem:positive-pay} still holds in here, so we can omit the obedience constraint \eqref{dis-cons:obedience}.

Define the utility function:

\begin{equation}
\text{Utility of Buyer Type }t: \quad u(t)= \sum_{q \in Q} \left[ g(q) \pi(q,t)v(q,t) \right]  -p(t)
\end{equation}

From \eqref{dis-cons:IC}, we have 
\begin{gather}
\sum_{q \in Q} [\pi(q, t) - \pi(q, t')] \cdot g(q) v(q,t)  \geq  p(t)  - p(t'), \label{dis-eq:ic1}\\
\sum_{q \in Q} [\pi(q, t') - \pi(q, t)] \cdot g(q) v(q,t')  \geq  p(t')  - p(t).\label{dis-eq:ic2}
\end{gather}

Combining Inequality \eqref{dis-eq:ic1} and \eqref{dis-eq:ic2}, we obtain the following constraint for any pair of types $t, t'$:
\begin{gather*}
\sum_{q \in Q} [\pi(q, t') - \pi(q, t)] \cdot g(q) v(q,t)  \leq p(t')  - p(t) \leq \sum_{q \in Q} [\pi(q, t') - \pi(q, t)] \cdot g(q) v(q,t')  . 
\end{gather*} 

\begin{eqnarray*}\label{eq:IC-outcome1}
0 &\leq&  \sum_{q \in Q} [\pi(q, t') - \pi(q, t)] \cdot g(q) [v(q,t') - v(q, t)]\\ 
& = & [ t' - t] \sum_{q \in Q} [\pi(q, t') - \pi(q, t)] \cdot g(q) v_1(q) 
\end{eqnarray*}
Define $$   P(t) = \sum_{q \in Q}  \pi(q, t) \cdot g(q) v_1(q) $$
We have,$(t' - t) ( P(t')-P(t )) \geq 0 $ implies $P(t)$ is non-decreasing in $t$.

\begin{eqnarray*}
 u(t) &=& \sum_{q \in Q} \left[ g(q) \pi(q,t)v(q,t) \right] -p(t) \\
 &\geq& \sum_{q \in Q} \left[ g(q) \pi(q,t')v(q,t) \right]  -p(t')  & \mbox{by Ineq. \eqref{dis-eq:ic1}} \\
 &=& \sum_{q \in Q} \left[ g(q) \pi(q,t')v(q,t) \right] + u(t') - \sum_{q \in Q} \left[ g(q) \pi(q,t')v(q,t') \right] & \mbox{Def of $u(t')$}\\ 
 &=& \sum_{q \in Q} \left[ g(q) \pi(q,t')[ v(q,t) - v(q, t')]  \right] + u(t')  & \mbox{Algebraic Manipulation}\\ 
 &=& (t-t') P(t') + u(t')  & \mbox{Def. of $P(t)$ and $v(q,t)$}\\   
\end{eqnarray*}

As a consequence, Inequality \eqref{dis-eq:ic1} implies  $u(t) -u(t') \geq (t-t')P(t') $. Together with a similar derivation from Inequality \eqref{dis-eq:ic2}, we  have the following inequality 
\begin{equation}
(t-t') P(t')  \le u(t)-u(t')\le (t-t') P(t).
\end{equation}
\begin{equation}
(t_i-t_{i-1}) P(t_{i-1})  \le u(t_i)-u(t_{i-1})\le (t_i-t_{i-1}) P(t_i).
\end{equation}

Since we have $t_{i-1} < t_{i}$, we know $P(t_i)$ is monotone non-decreasing in $t$.

So, for any IC mechanims there exist $P^\sim(t_i) \in [P(t_{i-1}),P(t_i)]$ such that
$$
u(t_k) = u(t_1) + \sum_{i=2}^k(t_i-t_{i-1}) P^\sim(t_i)
$$

Since $P(t)$ is monotone non-decreasing in $t$, we can denote $P^\sim(t_i)$ as $P(t^\sim_i)$ and $t^\sim_i \in [t_{i-1},t_i]$.

As $ u(t) = \sum_{q \in Q} \left[ g(q) \pi(q,t)v(q,t) \right] -p(t) $, we have

\begin{eqnarray*}
p(t_i) &=& \sum_{q \in Q} \left[ g(q) \pi(q,t_i)v(q,t_i) \right] -u(t_i) \\ 
&=& -u(t_1) + \sum_{q \in Q} \left[ g(q) \pi(q,t_i)v(q,t_i) \right] - \sum_{k=2}^i(t_k-t_{k-1}) P^\sim(t_k)
\end{eqnarray*}

Lemma \ref{lem:positive-pay} also works for discrete case. So, $p(t)\geq 0, \; \forall t \in T$ .

\begin{lemma}\label{dis-lem:feasible-M}[Characterization of Feasible Mechanisms]
A mechanism $(\pi, p)$ with non-negative payments is feasible if and only if it satisfies the following constraints:
\begin{eqnarray}\label{dis-eq:signal-monotonicity}
&& P(t) \text{ is monotone non-decreasing in } t \\\label{dis-eq:buyer-utility-identify2}
&& u(t_k) = u(t_1) + \sum_{i=2}^k(t_i-t_{i-1}) P^\sim(t_i), \, \, \, \forall t \in [T] \\\label{dis-eq:ir-t2}
& & u(t_N) \geq v(t_N), \, \, \, u(t_1) \geq 0 \\ \label{dis-eq:non-negativity}
& & p(t) \geq 0,  \, \, \forall t \in [T]. 
 \end{eqnarray}
\end{lemma}



\begin{proof}
 
The necessity of these constraints come from the above derivation and the IR constraint for type $t_N$ and $t_1$.  We now prove that they are sufficient.  That is, Constraint \eqref{eq:signal-monotonicity}-\eqref{eq:non-negativity} implies Obedience, IC and IR constraints \eqref{dis-cons:obedience}, \eqref{dis-cons:IC} and \eqref{dis-cons:IR}. 

IC constraint \eqref{dis-cons:IC} is equivalent to 
\begin{equation*}
     u(t) \geq u(t') + \sum_{q \in Q} \pi(q, t') \cdot g(q) [v(q,t) - v(q,t')] = u(t') + (t-t') P(t'). 
\end{equation*}
Therefore Constraint \eqref{dis-eq:signal-monotonicity} and \eqref{dis-eq:buyer-utility-identify2} implies IC constraint \eqref{dis-cons:IC} because for any of $t_x,t_y$ where $x <= y$ we have 
\begin{equation*}
     u(t_y) - u(t_x) = \sum_{i=x+1}^{y} (t_i-t_{i-1})P^\sim(t_i)   \geq \sum_{i=x+1}^{y} (t_i-t_{i-1})P^\sim(t_{x+1})  = (t_y-t_x)P^\sim(t_{x+1}) \geq (t_y-t_x)P(t_x) 
\end{equation*}
Similarly, when $x > y$,
$$
u(t_y) - u(t_x) = - \sum_{i=y+1}^{x} (t_i-t_{i-1})P^\sim(t_i)   \geq -\sum_{i=y+1}^{x} (t_i-t_{i-1})P^\sim(t_{x})  = (t_y-t_x)P^\sim(t_{x}) \geq (t_y-t_x)P(t_x) 
$$

The IR constraint \eqref{dis-cons:IR} is equivalent to $u(t) \geq 0$ and $u(t) \geq v(t)$. Since $P(t)\geq 0, \; \forall t \in T$, Constraint \eqref{dis-eq:buyer-utility-identify2}, together with $u(t_1) \geq 0$, implies $u(t) \geq 0, \; \forall t \in T$. We now leverage $u(t_N) \geq v(t_N)$ to prove    $u(t) \geq v(t), \; \forall t \in T$, as follows:
\begin{eqnarray*}
u(t_k) &=&  u(t_1) + \sum_{i=2}^k(t_i-t_{i-1}) P^\sim(t_i)  \\
& = &  u(t_N) - \sum_{i=k+1}^N(t_i-t_{i-1}) P^\sim(t_i)  \\
& \geq  &   v(t_N) - \sum_{i=k+1}^N(t_i-t_{i-1}) P^\sim(t_i)  \\
& \geq  &   v(t_N) - \sum_{i=k+1}^N(t_i-t_{i-1}) P(t_i)  \\
& =   &   \sum_{q \in Q} g(q) v_1(q)[t_N + \rho(q)]  - \sum_{i=k+1}^N(t_i-t_{i-1})   \sum_{q \in Q}  \pi(q, t_i) \cdot g(q) v_1(q)    \\
& \geq  &   \sum_{q \in Q} g(q) v_1(q)[t_N + \rho(q)]   - \sum_{i=k+1}^N(t_i-t_{i-1})   \sum_{q \in Q}   g(q) v_1(q)    \\
& =  &   \sum_{q \in Q} g(q) v_1(q)[t_k + \rho(q)]   = v(t_k) \\
\end{eqnarray*}

Finally, the Obedience constraint \eqref{dis-cons:obedience} follows from IR constraint \eqref{dis-cons:IR} and $p(t) \geq 0, \; \forall t \in T$. 

\end{proof}

Next we characterize the buyer's surplus from participating the information selling mechanism,  defined as follows:
\begin{equation}\label{eq:buyer-surplus}
\text{Buyer Surplus: } \quad s(t) = u(t) - \max \{ 0, v(t) \} 
\end{equation}
That is, the buyer surplus is the difference between his utility from the information selling mechanism and his utility from directly picking the better action among $0,1$ without purchasing any information. Note that the IR constraint \eqref{dis-cons:IR} is (naturally)  equivalent to $s(t) \geq 0$.   
Recall that the buyer of type $t$ has expected utility $v(t) = \sum_{q \in Q} v(q, t) g(q)  $ for action 1 without purchasing any information. Since $v(q, t)$ is monotone non-decreasing in $t$, we know that $v(t)$ is also monotone non-decreasing. Let $\bar{t}$ be the buyer type at which $v(t)$ crosses $0$   The following lemma characterize how the buyer's surplus changes as a function of his type. 

\begin{lemma}\label{lem:surplus-concave}
Let $\bar{t}$ be the buyer type such that $v(\bar{t}) = \sum_{q \in Q} v(q, \bar{t}) g(q)  = 0 $. In any feasible mechanism $(\pi, p)$ with non-negative payments, the buyer's surplus $s(t) $ is non-negative,  monotone non-decreasing for $t \in [t_1, \bar{t}]$, and monotone non-increasing for $t \in [\bar{t}, t_2]$. 
\end{lemma}
\begin{proof}
When $t_k \leq \bar{t}$, we have $v(t_k) \leq 0$, therefore $s(t_k) = u(t_k) = u(t_1) + \sum_{i=2}^k(t_i-t_{i-1}) P^\sim(t_i)  dx$ by Equation \eqref{eq:ir-t2}. Since $u(t_1) \geq 0$ and  $\forall i\geq 2, \; (t_i - t_{i-1}) \geq 0$ and $P(t_i) \geq 0$, it is easy to see that $s(t)$ is non-negative and monotone non-decreasing. 

When $t_k \geq \bar{t}$, we have $v(t_k) \geq 0$, therefore 
\begin{eqnarray*}
s(t_k) &=&  u(t_k) - v(t_k) \\
&=&  \bigg[ u(t_1) + \sum_{i=2}^k(t_i-t_{i-1}) P^\sim(t_i)  \bigg] - \bigg[ \sum_{q \in Q}  v_1(q) [t + \rho(q)] g(q)  \bigg]  \\
&=&  \bigg[ u(t_1) + \sum_{i=2}^k(t_i-t_{i-1}) P^\sim(t_i)  \bigg] - \bigg[ \sum_{i=2}^k(t_i-t_{i-1})\sum_{q \in Q}  v_1(q)g(q)  + v(t_1)\bigg]  \\
&=&  \bigg[ u(t_1) + \sum_{i=2}^k(t_i-t_{i-1}) \sum_{q \in Q}\pi(q,t_i^\sim) v_1(q)g(q)  \bigg] - \bigg[ \sum_{i=2}^k(t_i-t_{i-1})\sum_{q \in Q}  v_1(q)g(q)  + v(t_1)\bigg]  \\
&=&  u(t_1) - v(t_1) + \bigg[  \sum_{i=2}^k(t_i-t_{i-1}) \sum_{q \in Q}(\pi(q,t_i^\sim)-1) v_1(q)g(q)  \bigg].     \\  
\end{eqnarray*} 
Since $[\pi(q,t^\sim_i) - 1] \leq 0 $ and $v_1(q)    g(q) \geq 0$, we thus have $s(t)$ is monotone non-increasing in $t$. Consequently, $ s(t) \geq s(t_N) = u(t_N) - v(t_N) \geq 0$ by Inequality \eqref{eq:ir-t2}. 
\end{proof}
 
 

\subsection{Characterization of the Optimal Mechanism}
We are now ready to characterize the optimal mechanism using Lemma \ref{dis-lem:feasible-M}. We first derive the seller's revenue as a function of the mechanism $(\pi, p)$ that is assumed to satisfy Lemma \ref{dis-lem:feasible-M}. 
Define $t_0 = t_1$
We have 

\begin{align*}
REV (\pi, p)&=\sum_{k=1}^{N} f(t_k)p(t_k)\\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right]  -u(t_k) \right)\\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] - \sum_{i=2}^k(t_i-t_{i-1}) P^\sim(t_i)  -u(t_1) \right)\\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] \right)- \sum_{k=1}^{N} \sum_{i=2}^k f(t_k)(t_i-t_{i-1}) P^\sim(t_i)  -u(t_1) \\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] \right)- \sum_{i=2}^{N} \sum_{k=i}^N f(t_k)(t_i-t_{i-1}) P^\sim(t_i)  -u(t_1) \\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] \right)- \sum_{i=2}^{N} (1-F(t_{i-1}))(t_i-t_{i-1}) P^\sim(t_i)  -u(t_1) \\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] \right)- \sum_{i=1}^{N-1} (1-F(t_{i}))(t_{i+1}-t_{i}) P^\sim(t_{i+1})  -u(t_1) \\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] \right)- \sum_{i=1}^{N} (1-F(t_{i}))(t_{i+1}-t_{i}) P^\sim(t_{i+1})  -u(t_1) \\
&=\sum_{q\in Q} g(q)\left( \sum_{k=1}^{N} f(t_k)\left[ \pi(q,t_k)v(q,t_k)\right] \right)- \sum_{k=1}^{N} (1-F(t_{k}))(t_{k+1}-t_{k}) P^\sim(t_{k+1})  -u(t_1) \\
\end{align*}

Since $P(t)$ is monotone non-decreasing in $t$ and $P^\sim(t_i) \in [P(t_{i-1}),P(t_i)]$, to achieve maximized revenue, we should always set  $P^\sim(t_i) =P(t_{i-1})$.

\begin{align*}
REV (\pi, p) &=\sum_{q\in Q} g(q)\left( \sum_{k=1}^{N} f(t_k)\left[ \pi(q,t_k)v(q,t_k)\right] \right)- \sum_{k=1}^{N} (1-F(t_{k}))(t_{k+1}-t_{k}) P(t_{k})  -u(t_1) \\
&=\sum_{q\in Q} g(q)\left( \sum_{k=1}^{N} f(t_k)\left[ \pi(q,t_k)v(q,t_k)\right] \right)- \sum_{k=1}^{N} (1-F(t_{k}))(t_{k+1}-t_{k}) \sum_{q\in Q} \pi(q,t_{k})g(q)v_1(q)  -u(t_1) \\
&=\sum_{q\in Q} g(q)\left[ \sum_{k=1}^{N} f(t_k)\pi(q,t_k)\left( v(q,t_k) -(t_{k+1}-t_{k})v_1(q)\frac{1-F(t_k)}{f(t_k)}\right) \right]  -u(t_1) \\
&=\sum_{q\in Q} g(q)\left[ \sum_{k=1}^{N} f(t_k)\pi(q,t_k) v_1(q) [\underline{\varphi}(t_k) + \rho(q)] \right] -u(t_1) 
\end{align*}
where $\underline{\varphi}(t_k) = t_k - (t_{k+1}-t_{k})\frac{1-F(t_k)}{f(t_k)}$ is the standard virtual value function format used in the classic mechanism design literature. 

Note that the above derivation used the equality $u(t_k) = u(t_1) + \sum_{i=2}^k(t_i-t_{i-1}) P^\sim(t_i)$ to expand $u(t)$ with $u(t_1)$ as the reference point. This is also the original Myerson's approach. This approach works in Myerons's optimal auction design because there the buyer's surplus equals the buyer's utility from participating the mechanism since the only outside option is to not purchase resulting in utility $0$. Therefore, in Myerons's optimal auction design,  $u(t_1) \geq 0$   guarantees IR constraint, i.e., $u(t) \geq 0$, for any feasible mechanism. This however, ceases to be true in our setup because $s(t_1) \geq 0$ does not guarantee $s(t_2) \geq 0$. In fact, Lemma \ref{lem:surplus-concave} shows that $s(t)$ is a concave function with $s(\bar{t})$ as the maximum surplus where $\bar{t}$ is a zero of $v(t)$ function. Nevertheless, we know that the optimal mechanism must satisfy either $s(t_1) = 0$ or $s(t_2) = 0 $ since otherwise, we can shift the entire $s(t)$ curve down by a constant --- achieved by asking each buyer type to pay the same additional amount --- until one of them reach $0$. 

The above discussion is why we have to derive another utility representation by using the equality   
\begin{align*}
u(t_k) & =  u(t_1) + \sum_{i=2}^k(t_i-t_{i-1})P^\sim(t_i) \\
u(t_N) & = u(t_1) + \sum_{i=2}^N(t_i-t_{i-1})P^\sim(t_i)  \\
u(t_1) &= u(t_k) - \sum_{i=2}^k(t_i-t_{i-1})P^\sim(t_i)\\
u(t_N) & = u(t_k) - \sum_{i=2}^k(t_i-t_{i-1})P^\sim(t_i)+ \sum_{i=2}^N(t_i-t_{i-1})P^\sim(t_i)  \\
u(t_k) & = u(t_N) + \sum_{i=2}^k(t_i-t_{i-1})P^\sim(t_i) - \sum_{i=2}^N(t_i-t_{i-1})P^\sim(t_i)  \\
u(t_k) & = u(t_N)  - \sum_{i=k+1}^N(t_i-t_{i-1})P^\sim(t_i)  \\
\end{align*}
to expand $u(t)$ with $u(t_N)$ as the reference point. This gives us a slightly different representation of the same $REV (\pi, p)$. 

Set $t_0 = t_1$.
Revenue derivation with $t_N$ as the reference point can be expressed as follows: 

\begin{align*}
REV (\pi, p)&=\sum_{k=1}^{N} f(t_k)p(t_k)\\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right]  -u(t_k) \right)\\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] - u(t_N)  + \sum_{i=k+1}^N(t_i-t_{i-1})P^\sim(t_i) \right)\\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] \right)+ \sum_{k=1}^{N} \sum_{i=k+1}^N f(t_k)(t_i-t_{i-1}) P^\sim(t_i)  -u(t_N) \\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] \right)+ \sum_{k=1}^{N-1} \sum_{i=k+1}^N f(t_k)(t_i-t_{i-1}) P^\sim(t_i)  -u(t_N) \\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] \right)+ \sum_{i=2}^{N} \sum_{k=1}^{i-1} f(t_k)(t_i-t_{i-1}) P^\sim(t_i)  -u(t_N) \\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] \right)+ \sum_{i=2}^{N} F(t_{i-1})(t_i-t_{i-1}) P^\sim(t_i)  -u(t_N) \\
&=\sum_{k=1}^{N} f(t_k)\left(\sum_{q\in Q} g(q) \left[ \pi(q,t_k)v(q,t_k)\right] \right)+ \sum_{i=1}^{N} F(t_{i-1})(t_i-t_{i-1}) P^\sim(t_i)  -u(t_N) \\
&=\sum_{q\in Q} g(q)\left( \sum_{k=1}^{N} f(t_k)\left[ \pi(q,t_k)v(q,t_k)\right] \right)+ \sum_{k=1}^{N} F(t_{k-1})(t_{k}-t_{k-1}) P^\sim(t_{k})  -u(t_N) \\
\end{align*}

Since $P(t)$ is monotone non-decreasing in $t$ and $P^\sim(t_i) \in [P(t_{i-1}),P(t_i)]$, to achieve maximized revenue, we should always set  $P^\sim(t_i) =P(t_{i})$.

\begin{align*}
REV (\pi, p) &=\sum_{q\in Q} g(q)\left( \sum_{k=1}^{N} f(t_k)\left[ \pi(q,t_k)v(q,t_k)\right] \right)+ \sum_{k=1}^{N} F(t_{k-1})(t_{k}-t_{k-1}) P(t_{k})  -u(t_N) \\
&=\sum_{q\in Q} g(q)\left( \sum_{k=1}^{N} f(t_k)\left[ \pi(q,t_k)v(q,t_k)\right] \right) + \sum_{k=1}^{N} F(t_{k-1})(t_{k}-t_{k-1}) \sum_{q\in Q} \pi(q,t_{k})g(q)v_1(q)  -u(t_N) \\
&=\sum_{q\in Q} g(q)\left[ \sum_{k=1}^{N} f(t_k)\pi(q,t_k)\left( v(q,t_k) +(t_{k}-t_{k-1})v_1(q)\frac{F(t_{k-1})}{f(t_k)}\right) \right]  -u(t_N) \\
&=\sum_{q\in Q} g(q)\left[ \sum_{k=1}^{N} f(t_k)\pi(q,t_k) v_1(q) [\underline{\varphi}(t_k) + \rho(q)] \right] -u(t_N) 
\end{align*}

where $\bar{\varphi}(t_k) = t_k + (t_k - t_{k-1})\frac{F(t_{k-1})}{f(t_k)} $ is a transformed type function, which differs from the virtual value function in classic auction design. 
From the revenue function using $t_2$ as the reference point, we have the following optimization problem.

\begin{align*} 
\max_{\pi} & \sum_{q\in Q} g(q)\left[ \sum_{k=1}^{N} f(t_k)\pi(q,t_k) v_1(q) [\underline{\varphi}(t_k) + \rho(q)] \right] \\
\text{subject to} & \\
& P(t) \text{ is monotone non-decreasing in } t  \\
& u(t_k) = u(t_1) + \sum_{i=2}^k(t_i-t_{i-1}) P^\sim(t_i), \, \, \, \forall t \in [T] \\
& u(t_N) \geq v(t_N), \, \, \, u(t_1) \geq 0 \\ 
& p(t) \geq 0,  \, \, \forall t \in [T]. \\
\end{align*}




\begin{definition}[Upper/Lower-Boundary Virtual Value Function]
We call $\underline{\varphi}(t_k) = t_k - (t_{k+1}-t_{k})\frac{1-F(t_k)}{f(t_k)}$  the \emph{lower-boundary} virtual value function and call  $\bar{\varphi}(t_k) = t_k + (t_k - t_{k-1})\frac{F(t_{k-1})}{f(t_k)} $   the \emph{upper-boundary} virtual value function.  We say a virtual value function, upper-boundary or lower-boundary, is regular if it is monotone non-decreasing in $t$. 
\end{definition}

\begin{lemma}\label{dis-lem:two-simple-cases}

\begin{enumerate}
\item If  $v(t_N) < \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})P(t_{i-1}) = \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \underline{\theta}(t_{i-1}) }g(q)v_1(q)$ (or equivalently,  $v(t_1)   <  -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \underline{\theta}(t_{i-1}) }g(q)v_1(q)  $) and $\underline{\varphi}(t_k)$ is monotone non-decreasing, the optimal information selling mechanism is a threshold mechanism on $\rho(q)$ with threshold $\underline{\theta}(t_k) =  -\underline{\varphi}(t_k) $ for each type $t$.  The payment is determined by the following identity and is monotone non-decreasing in $t$: $$p(t_k) = \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k)  - \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1})$$ 
\item If $v(t_N) \geq \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})P(t_{i}) =\max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q)$ (or equivalently, $v(t_1)   \geq  -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \bar{\theta}(t_{i}) }g(q)v_1(q)    $)and $\bar{\varphi}(t_k)$ is monotone non-decreasing, the optimal information selling mechanism is a threshold mechanism  on $\rho(q)$ with threshold $\theta(t_k) =  -\bar{\varphi}(t_k) $ for each type $t$. The payment is determined by the following identity and is monotone non-increasing in $t$:
$$p(t_k) = \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k) -v(t_N) + \sum_{i=k+1}^N(t_i - t_{i-1})P(t_{i})$$   
\end{enumerate}
\end{lemma}
\begin{proof}
\textbf{Case 1:}

\textbf{Optimality:}



First, prove the equivalence
\begin{align*}
& v(t_N) < \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \underline{\theta}(t_{i-1}) }g(q)v_1(q)\\
\Longleftrightarrow \quad  &   v(t_1) + (t_N - t_1) \sum_{q \in Q} v_1(q) g(q)  < \max \{ 0,v(t_1) \} +\sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \underline{\theta}(t_{i-1}) }g(q)v_1(q)\\
\Longleftrightarrow \quad  &   v(t_1) -\max \{0,v(t_1) \}  <    \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \underline{\theta}(t_{i-1}) }g(q)v_1(q) - (t_N - t_1) \sum_{q \in Q} v_1(q) g(q)  \\ 
\Longleftrightarrow \quad  &   v(t_1) -\max \{0,v(t_1) \}  <   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \underline{\theta}(t_{i-1}) }g(q)v_1(q) - \sum_{i=2}^N(t_i - t_{i-1}) \sum_{q \in Q} v_1(q) g(q)  \\ 
 \Longleftrightarrow \quad  &   v(t_1) -\max \{0 , v(t_1)\} <  -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \underline{\theta}(t_{i-1}) }g(q)v_1(q)   \\
  \Longleftrightarrow \quad  &   v(t_1)   <  -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \underline{\theta}(t_{i-1}) }g(q)v_1(q)    \\ 
\end{align*}

The last equivalence is because supposing $v(t_1) \geq 0$, we will have $0<-   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \underline{\theta}(t_{i-1}) }\\g(q)v_1(q)$. Since $\forall q, 
\; g(q)$ and $v_1(q)$ are non-negative, this equation doesn't hold. So, $v(t_1) < 0$. Then, we get the last equivalence.

The threshold $\underline{\theta}(t) = -\underline{\varphi}(t)$ is picked such that $\pi(q,t) =1$ whenever $ \underline{\varphi}(t) + \rho(q)  > 0$ and $\pi(q,t) =0$ whenever $ \underline{\varphi}(t) + \rho(q) < 0$. That is,  the revenue function, expressed with $t_1$ as reference point, is entry-wise maximized. This clearly achieves the maximum possible value in the first term of  the revenue $REV(\pi, p)$ expression. 

The second term is maximized by choosing the minimum possible $u(t_1)$ value, i.e., $u(t_1) = 0$. With the defined payment function, we indeed choose $u(t_1)  = \sum_{q\in Q} [g(q) \pi(q,t_1)v(q,t_1)]  - p(t_1) = \sum_{i=2}^1(t_i - t_{i-1})P(t_{i-1})   = 0 $.

Thus, this mechanism is optimal.

\textbf{Feasibility:}

Next, we argue that this choice also leads to a feasible mechanism, satisfying the characterization of Lemma \eqref{lem:feasible-M}. Since the lower-boundary virtual value function $\underline{\varphi}(t)$ is monotone non-decreasing in $t$, we know that the threshold $\underline{\theta}(t) =  -\underline{\varphi}(t)$   is monotone non-increasing in $t$. This implies that 
\begin{equation*}
    P(t_k) = \sum_{q \in Q} \pi(q, t_k) g(q)v_1(q)  =   \sum_{q: \rho(q) \geq {\underline{\theta}}(t_k)}  g(q)v_1(q)  
\end{equation*}
is monotone non-decreasing in $t$ since a larger $t$ leads to a smaller lower bound $\underline{\theta}(t)$ and $g(q)$ and $v_1(q)$ are both non-negative.

The utility identify follows from definitions and the payment p(t) we specified for this case: 
\begin{eqnarray*}
    u(t_k)  = \sum_{q\in Q} [g(q) \pi(q,t_k)v(q,t_k)]  - p(t_k) =     \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1})
\end{eqnarray*}
Thus $u(t_1) =    \sum_{i=2}^1(t_i - t_{i-1})P(t_{i-1}) = 0$, which can be substituted into the above equality to obtain the utility identify.  $ u(t_k) = u(t_1) + \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1}) = u(t_1) + \sum_{i=2}^k(t_i-t_{i-1}) P^\sim(t_i)$

For constraint \eqref{dis-eq:ir-t2}, we have 

\begin{align*}
u(t_1) &= \sum_{q\in Q} \pi(q,t_1) g(q) v(q,t_1)    - p(t_1) = 0 \\
u(t_N) &= \sum_{q \in Q} \pi(q,t_N) g(q) v(q,t_N)    - p(t_N)  =\sum_{i=2}^N(t_i - t_{i-1})P(t_{i-1})  \geq 0 \geq v(t_N)
\end{align*}

Finally, we argue that the payment  is non-negative. We first prove that the payment is non-decreasing in $t$ for any $t$ with $0<=F(t)<=1$.  
 We know that the threshold $\underline{\theta}(t)$ satisfies $ \underline{\varphi}(t) +  \underline{\theta}(t) = 0$. Since $\underline{\varphi}(t) = t - \frac{1 - F(t)}{f(t)} \leq t$, we have $\underline{\theta}(t) \geq -t$. 


% Next, we show $q2 \geq q_t^*$. Since $ v(t) = \int_{q \in Q} g(q)  v(q,t)\, \mathrm{d}q \geq 0$ and $g(q)\geq 0$, we know some of $v(q,t)$ in this integral must be greater than 0. And $q_t^*$ makes $v(q_t^*,t) = v_1(q_t^*)t + v_0(q_t^*) = 0$, so $q_2 \geq q_t^*$. Thus, $q_2 \geq q_t^* \geq \theta(t)$.


For any $t_k > t_j$, we have $\underline{\theta}(t_k) \leq \underline{\theta}(t_j)$. Thus, $-t \leq \underline{\theta}(t_k) \leq \underline{\theta}(t_j) $.



\begin{eqnarray*}
p(t_k) &=&  \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k)  - \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1}) \\ 
& = & \sum_{q:\rho(q)\geq\underline{\theta}(t_k)} \big[g(q) v(q, t_j) \big]   +  \sum_{q\in Q} \big[g(q) \pi(q,t_k)v_1(q)(t_k-t_j)   \big]   - u(t_j) - \sum_{i=j+1}^k(t_i - t_{i-1})P(t_{i-1}) \\ 
&  \geq & \sum_{q:\rho(q)\geq\underline{\theta}(t_j)} \big[g(q)v(q,t_j) \big]  - u(t_j) +   (t_k-t_j) P(t_k)  - \sum_{i=j+1}^k(t_i - t_{i-1})P(t_{i-1}) \\ 
&  = & \sum_{q\in Q} [g(q) \pi(q,t_j)v(q,t_j)]  - u(t_j) +   (t_k -t_j) P(t_k)  - \sum_{i=j+1}^k(t_i - t_{i-1})P(t_{i-1}) \\ 
&  =& p(t_j) +   (t_k -t_j) P(t_k)  - \sum_{i=j+1}^k(t_i - t_{i-1})P(t_{i-1}) \\ 
&  \geq & p(t_j)
\end{eqnarray*}

The first inequality is due to  $-t \leq \underline{\theta}(t_k) \leq \underline{\theta}(t_j) $  and thus  $\sum_{q:\rho(q)\geq\underline{\theta}(t_k)} \big[g(q) v(q, t_j) \big]$ sums over more positive terms compared with $\sum_{q:\rho(q)\geq\underline{\theta}(t_j)} \big[g(q)v(q,t_j) \big] $. The last inequality is due to monotonicity of $P(x)$ and our choice of $t_k>t_j$.  Therefore, to prove the non-negativity of the payment, we only need to prove $p(t_1) \geq 0$, as follows:  


\begin{align*}
p(t_1) &= \sum_{q \in Q} \pi(q,t) g(q)  v(q,t_1) - u(t_1) \\
&= \sum_{q \in Q} \pi(q,t_1) g(q)  v(q,t_1) - s(t_1) \\
&= \sum_{q \in Q} \pi(q,t_1) g(q)  v(q,t_1) \\
&= \sum_{q:\rho(q)\geq\underline{\theta}(t_1)}  g(q)  v(q,t_1) \\
& \geq 0
\end{align*}
The last inequality is because  $\underline{\theta}(t_1) \geq -t$. 



\textbf{Case 2:}

\textbf{Optimality:}

First, prove the equivalence
\begin{align*}
& v(t_N) \geq \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q)\\
\Longleftrightarrow \quad  &   v(t_1) + (t_N - t_1) \sum_{q \in Q} v_1(q) g(q)  \geq \max \{ 0,v(t_1) \} +\sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q)\\
\Longleftrightarrow \quad  &   v(t_1) -\max \{0,v(t_1) \}  \geq    \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q) - (t_N - t_1) \sum_{q \in Q} v_1(q) g(q)  \\ 
\Longleftrightarrow \quad  &   v(t_1) -\max \{0,v(t_1) \}  \geq   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q) - \sum_{i=2}^N(t_i - t_{i-1}) \sum_{q \in Q} v_1(q) g(q)  \\ 
 \Longleftrightarrow \quad  &   v(t_1) -\max \{0 , v(t_1)\} \geq  -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \bar{\theta}(t_{i}) }g(q)v_1(q)   \\
  \Longleftrightarrow \quad  &   v(t_1)   \geq  -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \bar{\theta}(t_{i}) }g(q)v_1(q)    \\ 
\end{align*}






The threshold $\bar{\theta}(t) =  -\bar{\varphi}(t)$ is picked such that $\pi(q,t) =1$ whenever $  \bar{\varphi}(t) + \rho(q) > 0$ and $\pi(q,t) =0$ whenever $ \bar{\varphi}(t) + \rho(q) < 0$. That is,  the revenue function, expressed with $t_N$ as reference point, is entry-wise maximized. This clearly achieves the maximum possible value in the first term of  the revenue $REV(\pi, p)$ expression.

The second term is maximized by choosing the minimum possible $u(t_N)$ value, i.e., $u(t_N) = v(t_N)$. With the defined payment function, we indeed choose     $u(t_N)  = \sum_{q\in Q} [g(q) \pi(q,t_N)v(q,t_N)]  - p(t_N) =    v(t_N) - \sum_{t_N}^{t_N} P(x)  dx = v(t_N)$.

Thus, this mechanism is optimal.

\textbf{Feasibility:}

Next, we argue that this choice also leads to a feasible mechanism, satisfying the characterization of Lemma \eqref{lem:feasible-M}. Since the upper-boundary virtual value function $\bar{\varphi}$ is monotone increasing, we know that the threshold $\bar{\theta}(t) = -\bar{\varphi}(t)$   is monotone non-increasing in $t$. This implies that 
\begin{equation*}
    P(t_k) = \sum_{q \in Q} \pi(q, t_k) g(q)v_1(q)  =   \sum_{q: \rho(q) \geq \bar{\theta}(t_k)}   g(q)v_1(q)  
\end{equation*}
is monotone non-decreasing in $t$ since a larger $t$ leads to a smaller $\bar{\theta}(t)$ and thus larger integral domain for $q$. 

We now prove the utility identify. By definition of $u(t)$ and our choice of payment function, we have 
\begin{eqnarray*}
    u(t_k)  = \sum_{q\in Q} [g(q) \pi(q,t_k)v(q,t_k)]  - p(t_k) =    v(t_N) - \sum_{i=k+1}^N(t_i - t_{i-1})P(t_{i}). 
\end{eqnarray*}
Thus $u(t_N) =  v(t_N) - \sum_{t_N}^{t_N} P(x)  dx = v(t_N)$, which can be substituted into the above equality to obtain the utility identify, as required by Lemma  \eqref{dis-lem:feasible-M}. 

For constraint \eqref{eq:ir-t2}, we have 
\begin{align*}
u(t_N) &= \sum_{q \in Q} \pi(q,t_N) g(q) v(q,t_N)    - p(t_N) =  v(t_N) \\
u(t_1) &= \sum_{q \in Q} \pi(q,t_1) g(q) v(q,t_1)    - p(t_1) \\
&=v(t_N) - \sum_{i=2}^N(t_i - t_{i-1})P(t_{i})\\
&\geq \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q) -  \sum_{i=2}^N(t_i - t_{i-1})P(t_{i})\\
&= \max(0,v(t_1)) +\sum_{i=2}^N(t_i - t_{i-1})P(t_{i}) -  \sum_{i=2}^N(t_i - t_{i-1})P(t_{i})\\
&\geq 0\\
\end{align*}



Finally, we argue that the payment  is non-negative. We first prove that the payment is non-increasing in $t$ for any $t$ with $F(t)>0$.  
 We know that the threshold $\bar{\theta} _t$ satisfies $ \bar{\varphi}(t) +  \bar{\theta}(t) = 0$. Since $\bar{\varphi}(t) = t +\frac{F(t)}{f(t)} > t$ due to our choice of $t$ with $F(t)>0$, we have $\bar{\theta}(t) < -t$. Note that the types with $F(t) = 0$ does not need to be taken care as their total probability measure is $0$. 


% Next, we show $q2 \geq q_t^*$. Since $ v(t) = \sum_{q \in Q} g(q)  v(q,t)\, \mathrm{d}q \geq 0$ and $g(q)\geq 0$, we know some of $v(q,t)$ in this integral must be greater than 0. And $q_t^*$ makes $v(q_t^*,t) = v_1(q_t^*)t + v_0(q_t^*) = 0$, so $q_2 \geq q_t^*$. Thus, $q_2 \geq q_t^* \geq \bar{\theta}(t)$.


For any $t_k > t_j$, we have $\bar{\theta}(t_k) \leq \bar{\theta}(t_j) < -t_k$ because $\bar{\theta}(t_k) = - t_k - \frac{F(t_k)}{f(t_k)}$ is a non-increasing function.
\begin{eqnarray*}
p(t_k) -p(t_j) &=& \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k)   - \sum_{q\in Q} g(q) \pi(q,t_j)v(q,t_j)   - \sum_{i=j+1}^K(t_i - t_{i-1})P(t_{i}) \\ 
&=& \sum_{q: \rho(q) \geq \bar{\theta}(t_k)}  g(q) v(q,t_k)   - \sum_{q: \rho(q) \geq \bar{\theta}(t_j)}  g(q) v(q,t_j)   - \sum_{i=j+1}^K(t_i - t_{i-1})P(t_{i}) \\ 
&\leq& \sum_{q: \rho(q) \geq \bar{\theta}(t_j)}  g(q) v(q,t_k)   - \sum_{q: \rho(q) \geq \bar{\theta}(t_j)}  g(q) v(q,t_j)   - \sum_{i=j+1}^K(t_i - t_{i-1})P(t_{i}) \\ 
&= & \sum_{q: \rho(q) \geq \bar{\theta}(t_j)} g(q) (v(q,t_k)-v(q,t_j))   - \sum_{i=j+1}^K(t_i - t_{i-1})P(t_{i}) \\  
&=& (t_k-t_j) \sum_{ q: \rho(q) \geq \bar{\theta}(t_j) } g(q) v_1(q)   - \sum_{i=j+1}^K(t_i - t_{i-1})P(t_{i}) \\ 
&=& (t_k-t_j) \sum_{ q \in Q} g(q) v_1(q) \pi(q,t_j)   - \sum_{i=j+1}^K(t_i - t_{i-1})P(t_{i}) \\ 
&=& (t_k-t_j) P(t_j) - \sum_{i=j+1}^K(t_i - t_{i-1})P(t_{i}) \\ 
&  \leq & 0
\end{eqnarray*}
The first inequality is due to  $\bar{\theta}(t_k) \leq \bar{\theta}(t_j) < -t_k$  and thus  $\sum_{q: \rho(q) \geq \bar{\theta}(t_j)}  g(q) v(q,t_k)  $ sums over less negative terms  compared with $\sum_{\bar{\theta}(t_k)}^{q_2} g(q) v(q,t_k)  $. The last inequality is due to monotonicity of $P(x)$ and our choice of $t_k>t_j$.  Therefore, to prove the non-negativity of the payment, we only need to prove $p(t_N) \geq 0$, as follows:  

\begin{align*}
 p(t_N) &= \sum_{q \in Q} [g(q) \pi(q,t_N)v(q,t_N)]  - v(t_N) + \sum_{i=N+1}^N(t_i - t_{i-1})P(t_{i})   \\
 &= \sum_{q \in Q} \pi(q,t_N) g(q)  v(q,t_N) - \sum_{q \in Q} g(q)  v(q,t_N)\\ 
& \geq 0
\end{align*}
The last inequality is because  $\pi(q,t_N) = 1, \forall v(q,t_N)\geq 0$. 

This concludes our proof of non-negative and non-increasing payoff for Case 2, and also concludes the proof for this case. 

\end{proof}


\begin{lemma}
 For $v(t_N)$ not in the above 2 cases where $ \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \underline{\theta}(t_{i-1})} \\ g(q)v_1(q) \leq v(t_N) < \max(0,v(t_1)) + \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q)$ (or equivalently,  $ -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \underline{\theta}(t_{i-1}) }g(q)v_1(q)  \leq  v(t_1) < -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \bar{\theta}(t_{i}) }g(q)v_1(q)$)and $\widetilde{\varphi}_q(t_i) = f(t_i)  \frac{[\underline{\varphi}(t_i) + \rho(q)]}{(t_{i+1}-t_{i}) }$ is non-decreasing in t for any q, the optimal mechanism is a threshold mechanism on $\rho(q)$ with threshold $\theta(t_i) = t_i+ (t_{i+1}-t_{i})\frac{C-F(t_i)}{f(t_i)} $, where $C \in (0,1]$ is a constant and satisfies  $\sum_t\sum_{q:}_{ \widetilde{\varphi}_q(t) + 1 >= C } g(q)  v_1(q) (t_{i+1}-t_{i})   = v(t_N)$. 
 


  The payment is determined by the following identity and is monotone non-decreasing in t when $F(t) \leq C $ and monotone non-increasing when $F(t) > C$.
  
  
Define 
\begin{align*}
\underline{p}(t_k) &= \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k)  - \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1}) \\
\bar{p}(t_k) &= \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k) -v(t_N) + \sum_{i=k+1}^N(t_i - t_{i-1})P(t_{i})
\end{align*}

The payment function for this mechanism is:
\begin{gather*}
p(t_k) =
\begin{cases}
\underline{p}(t_k) & \text{for } F(t_k) \leq C\\
\bar{p}(t_k) & \text{for } F(t_k) > C
\end{cases}
\end{gather*}

\end{lemma}
\begin{proof}

\textbf{Reduction and Optimality:}

Our initial goal is to maximize revenue function:



\begin{align*}
\text{max }  &\sum_{i=1}^{N} \sum_{q\in Q} \pi(q,t_i) g(q)  v_1(q) f(t_i) [\underline{\varphi}(t_i) + \rho(q)]  -u(t_1)  & 
\mbox{by Revenue Equation} \\
\text{subject to} & \sum_{i=1}^N \sum_{q \in Q}  \pi(q,t_{i})g(q)v_1(q) (t_{i+1}-t_{i})  \geq v(t_N)\\
& P(t) \text{is monotone in }t
\end{align*}

Now, we are going to simplify it.
% \begin{align*}
% \max_{\pi} &  \sum_{t_1}^{t_N} \sum_{q \in Q} g(q) \pi(q,t) v_1(q) f(t)  [\underline{\varphi}(t) + \rho(q)]\,\mathrm{d}q  \mathrm{d}t - u(t_1) \leq \\ \max_{\pi} &  \sum_{t_1}^{t_N} \sum_{q \in Q} g(q) \pi(q,t) v_1(q) f(t)  [\underline{\varphi}(t) + \rho(q)]\,\mathrm{d}q  \mathrm{d}t - \min_{\pi,p}{u(t_1)}
% \end{align*}
From condition $ -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \underline{\theta}(t_{i-1}) }g(q)v_1(q)  \leq  v(t_1) < -   \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) < \bar{\theta}(t_{i}) }g(q)v_1(q)$), we know $v(t_1)<0$

Thus,
\begin{equation} \label{dis-relation-v(t_N)}
\sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \underline{\theta}(t_{i-1})}  g(q)v_1(q) \leq v(t_N) < \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q) 
\end{equation}

Because of IR constraint to make sure $s(t_1) = u(t_1) - \max(0,v(t_1))  = u(t_1)  \geq 0$, we need $u(t_1) \geq 0$.

For the constraint, since we defined $t_{N+1} = t_N$
\begin{align*}
\sum_{i=1}^N \sum_{q \in Q}  \pi(q,t_{i})g(q)v_1(q) (t_{i+1}-t_{i}) &= \sum_{i=2}^N \sum_{q \in Q}  \pi(q,t_{i-1})g(q)v_1(q) (t_{i}-t_{i-1}) \\
&=\sum_{i=2}^N(t_i-t_{i-1}) \pi(q,t_{i-1})g(q)v_1(q) \\
&=\sum_{i=2}^N(t_i-t_{i-1}) P(t_{i-1}) \\
&\geq v(t_N)
\end{align*}

% At $t_1$, we just get $ \sum_{i=2}^N(t_i-t_{i-1}) P(t_{i-1})   \geq v(t_N) $
% \begin{align*} 
% \bar{p}(t_1) &= \sum_{q\in Q} g(q) \pi(q,t_1)v(q,t_1) -v(t_N) + \sum_{i=2}^N(t_i - t_{i-1})P(t_{i}) \\
% &\geq \sum_{q\in Q} g(q) \pi(q,t_1)v(q,t_1) -v(t_N) + \sum_{i=2}^N(t_i - t_{i-1})P(t_{i-1}) \\
% &\geq \sum_{q\in Q} g(q) \pi(q,t_1)v(q,t_1) \\
% & = \underline{p}(t_1) 
% \end{align*}

With this mechanism, if $F(t_1) \leq C$ 
\begin{align} 
u(t_1) &= \sum_{q\in Q} g(q) \pi(q,t_1)v(q,t_1) - p(t_1) \nonumber\\
&= \sum_{q\in Q} g(q) \pi(q,t_1)v(q,t_1) - \underline{p}(t_1) \nonumber\\
&= 0 \label{dis-u_t_1}  
\end{align} 


If $F(t_1) > C$ 
\begin{align} 
u(t_1) &= \sum_{q\in Q} g(q) \pi(q,t_1)v(q,t_1) - p(t_1) \nonumber\\
&= \sum_{q\in Q} g(q) \pi(q,t_1)v(q,t_1) - \bar{p}(t_1) \nonumber\\
&= v(t_N) - \sum_{i=2}^N(t_i - t_{i-1})P(t_{i}) \nonumber \\
&= 0 \label{dis-u_t_1}  
\end{align} 

By setting $ v(t_N) - \sum_{i=2}^N(t_i - t_{i-1})P(t_{i})$, we can make $u(t_1) = 0$. In later proof, we will show this also maximizes the first term at the same time.

Thus, $u(t_1)$ can always achieve minimized $u(t_1) = 0$, which indeed minimized the second term.

So, we reduce our goal to
\begin{align*}
\text{max }  &\sum_{i=1}^{N} \sum_{q\in Q} \pi(q,t_i) g(q)  v_1(q) f(t_i) [\underline{\varphi}(t_k) + \rho(q)] & 
\mbox{by Revenue Equation} \\
\text{subject to} & \sum_{i=1}^N \sum_{q \in Q}  \pi(q,t_{i})g(q)v_1(q) (t_{i+1}-t_{i})  \geq v(t_N)\\
& P(t) \text{is monotone in }t
\end{align*}

For the goal, we can write it in another way
\begin{align*}
&\sum_{i=1}^{N} \sum_{q\in Q} \pi(q,t_i) g(q)  v_1(q) f(t_i) [\underline{\varphi}(t_i) + \rho(q)] \\
&= \sum_{i=1}^{N} \sum_{q\in Q} \pi(q,t_i) g(q)  v_1(q) (t_{i+1}-t_{i}) f(t_i)  \frac{[\underline{\varphi}(t_i) + \rho(q)]}{(t_{i+1}-t_{i}) } \\
&= \sum_{i=1}^{N} \sum_{q\in Q} \pi(q,t_i) g(q)  v_1(q) (t_{i+1}-t_{i}) f(t_i)  \frac{[t_i - (t_{i+1}-t_{i})\frac{1-F(t_i)}{f(t_i)}  + \rho(q)]}{(t_{i+1}-t_{i}) } \\
&= \sum_{i=1}^{N} \sum_{q\in Q} \pi(q,t_i) g(q)  v_1(q) (t_{i+1}-t_{i}) f(t_i)  [\frac{t_i + \rho(q)}{(t_{i+1}-t_{i}) } - \frac{1-F(t_i)}{f(t_i)}] \\
\end{align*}

Now, the object function is 
\begin{align*}
\text{max }  &\sum_{i=1}^{N} \sum_{q\in Q} \pi(q,t_i) g(q)  v_1(q) (t_{i+1}-t_{i}) f(t_i)  \frac{[\underline{\varphi}(t_i) + \rho(q)]}{(t_{i+1}-t_{i}) } & 
\mbox{by Revenue Equation} \\
\text{subject to} & \sum_{i=1}^N \sum_{q \in Q}  \pi(q,t_{i})g(q)v_1(q) (t_{i+1}-t_{i})  \geq v(t_N)\\   \label{dis-v(t_N)-upper}
& P(t) \text{is monotone in }t
\end{align*}

Define  $\widetilde{\varphi}_q(t_i) = f(t_i)  \frac{[\underline{\varphi}(t_i) + \rho(q)]}{(t_{i+1}-t_{i}) }$. We can think this optimization problem as a fractional knapsack problem where we are required to pick at least $v(t_N)$ units of items. Each item can be picked up to $g(q)v_1(q) (t_{i+1}-t_{i})$ units since $0 \leq \pi(q,t) \leq 1 $  and each unit of this item gives $\widetilde{\varphi}_q(t)$ value.

Since $f(t_i) > 0$ and $(t_{i+1}-t_{i}) > 0$, the optimal solution is to pick all the items with $[\underline{\varphi}(t_i) + \rho(q)] \geq 0$ and if we haven't reach the units lower bound, pick the largest $\widetilde{\varphi}_q(t)$ items until we reach the units lower bound $v(t_N)$

With $\widetilde{\varphi}_q(t) $ is non-decreasing in $t$, the solution is a threshold mechanism on $\rho(q)$, because  $\widetilde{\varphi}_q(t)$ is non-decreasing on $\rho(q)$. 

By \eqref{dis-relation-v(t_N)} and optimization constraint,
\begin{equation*} 
\sum_{i=1}^N\sum_{\rho(q) \geq \underline{\theta}(t_{i})} g(q)v_1(q) (t_{i+1} - t_{i}) \leq v(t_N)  \leq \sum_{i=1}^N \sum_{q \in Q}  \pi(q,t_{i})g(q)v_1(q) (t_{i+1}-t_{i})  
\end{equation*}



Since the threshold $\underline{\theta_(t_i)}  = -\underline{\varphi}(t_i)$, this means whenever $[\underline{\varphi}(t_i) + \rho(q)] \geq 0$, $\pi(q,t_i)=1$. However, even all the positive $[\underline{\varphi}(t_i) + \rho(q)]$ terms have been chosen, we may still didn't reach $v(t_N)$. So, we may have to choose negative $[\underline{\varphi}(t_i) + \rho(q)]$ terms. And since $f(t_i)> 0$ and $(t_{i+1}-t_{i})>0$, $\widetilde{\varphi}_q(t_i) = f(t_i)  \frac{[\underline{\varphi}(t_i) + \rho(q)]}{(t_{i+1}-t_{i}) } < 0$. So, we may have to choose items with negative $\widetilde{\varphi}_q(t_i)$ value for the knapsack. The optimal way is still to choose the largest  $\widetilde{\varphi}_q(t_i)$  value item until reaching the unit lower bound $v(t_N)$. Notably, part of chosen $\widetilde{\varphi}_q(t_i)$ value is negative. 

So, we can simplify the optimization problem to

\begin{align}
\text{max }  &\sum_{i=1}^{N} \sum_{q\in Q} \pi(q,t_i) g(q)  v_1(q) (t_{i+1}-t_{i}) f(t_i)  \frac{[\underline{\varphi}(t_i) + \rho(q)]}{(t_{i+1}-t_{i}) } \nonumber \\
\text{subject to} & \sum_{i=1}^N \sum_{q \in Q}  \pi(q,t_{i})g(q)v_1(q) (t_{i+1}-t_{i})  = v(t_N) \label{dis-v-t-n} \\   
& P(t) \text{is monotone in }t \nonumber
\end{align}



\textbf{Feasibility:}

Let's prove this payment function gives us a feasible optimal mechanism. 

For $P(t)$ is monotone in $t$, Define $\rho^*_t(q)$ where $ f(t_i)  \frac{[\underline{\varphi}(t_i) + \rho^*_t(q)]}{(t_{i+1}-t_{i}) } =C$. $\rho^*_t(q)$ is non-increasing in t, since  $\widetilde{\varphi}_q(t_i) =  f(t_i)  \frac{[\underline{\varphi}(t_i) + \rho^*_t(q)]}{(t_{i+1}-t_{i}) }$  is no-decreasing in t for all q. So, larger t will include more $q$ in its sum range. 
Thus, $P(t) =  \int_{\rho(q) \geq \rho^*_{t}(q) } g(q) v_1(q)  $ is non-decreasing in $t$.


By \eqref{dis-u_t_1},$u(t_1) = 0$.

At $t_N$, we just get $ \sum_{i=2}^N(t_i-t_{i-1}) P(t_{i-1})   \geq v(t_N) $
\begin{align*} 
\bar{p}(t_N) &= \sum_{q\in Q} g(q) \pi(q,t_N)v(q,t_N) -v(t_N) + \sum_{i=N+1}^N(t_i - t_{i-1})P(t_{i}) \\
&=\sum_{q\in Q} g(q) \pi(q,t_N)v(q,t_N) -v(t_N) \\
&= \sum_{q\in Q} g(q) \pi(q,t_N)v(q,t_N)  - \sum_{i=2}^N(t_i - t_{i-1})P(t_{i-1}) \\
& = \underline{p}(t_N) 
\end{align*}



\begin{align*} 
u(t_n) &=\sum_{q\in Q} g(q) \pi(q,t_N)v(q,t_N) - \bar{p}(t_N) = v(t_n)
\end{align*}


For $\forall t_k \; s.t. \; F(t_k)\leq C$
\begin{align*} 
u(t_k)&=\sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k) - \underline{p}(t_k) \\
&= \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k)  - \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k)  + \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1}) \\
&= u(t_1) + \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1}) \\
\end{align*}

For $\forall t_k \; s.t. \; F(t_k) > C$
\begin{align*} 
u(t_k)&=\sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k) - \bar{p}(t_k) \\
&= \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k)  - \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k) +v(t_N) - \sum_{i=k+1}^N(t_i - t_{i-1})P(t_{i}) \\
&=\sum_{i=2}^N(t_i-t_{i-1}) P(t_{i-1}) - \sum_{i=k+1}^N(t_i - t_{i-1})P(t_{i}) \\
&= \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1}) \\
&= u(t_1) + \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1}) \\
\end{align*}



Now, constraints \eqref{dis-eq:buyer-utility-identify2}\eqref{dis-eq:ir-t2}\eqref{dis-eq:non-negativity} which are equivalent to IC, IR have been satisfied. 

By \eqref{dis-relation-v(t_N)}, $\sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \underline{\theta}(t_{i-1})} g(q)v_1(q) \leq v(t_N) < \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q)  $.


$$
\widetilde{\varphi}_q(t_i) = f(t_i)  \frac{[\underline{\varphi}(t_i) + \rho(q)]}{(t_{i+1}-t_{i}) } = f(t_i)  [\frac{t_i + \rho(q)}{(t_{i+1}-t_{i}) } - \frac{1-F(t_i)}{f(t_i)}] =  \frac{f(t_i)(t_i + \rho(q))}{(t_{i+1}-t_{i}) } +F(t_i) - 1
$$

As we discussed above, to satisfy \eqref{dis-v-t-n}, in addition to including all the $\frac{f(t_i)(t_i + \rho(q))}{(t_{i+1}-t_{i}) } +F(t_i) - 1 \geq 0$ which is $ \frac{f(t_i)(t_i + \rho(q))}{(t_{i+1}-t_{i}) } + F(t_i) \geq 1$ terms, we have to add some negative $\widetilde{\varphi}_q(t_i)$ terms to our knapsack where $\frac{f(t_i)(t_i + \rho(q))}{(t_{i+1}-t_{i}) } + F(t_i) < 1$.

These terms will not be too much because $v(t_N) < \sum_{i=2}^N(t_i - t_{i-1})\sum_{\rho(q) \geq \bar{\theta}(t_{i}) }g(q)v_1(q) $, which means we only need to include part of the terms where $f(t_i)  \frac{[\bar{\varphi}(t_i) + \rho(q)]}{(t_{i+1}-t_{i}) }  = \frac{f(t_i)(t_i + \rho(q))}{(t_{i+1}-t_{i}) } +F(t_i) \geq 0$ to satisfy \eqref{dis-v-t-n}.

Thus, every recommended negative $\widetilde{\varphi}_q(t_i)$ terms in the optimal policy will be included in the policy where we use $ f(t_i)  \frac{[\bar{\varphi}(t_i) + \rho(q)]}{(t_{i+1}-t_{i}) } \geq 0 $ to set $\pi(q,t) = 1$. 


Also, $s(t_1) = u(t_1) - max(0,v(t_1))= u(t_1) = 0$ and $s(t_N) = u(t_N) - max(0,v(t_N))= u(t_N) - v(t_N)= 0$. 

Now, we are going to prove $\forall t\; p(t)>0$ to satisfy the obedience constraint.

With proof above, there is a constant $C \in (0,1]$, where when $\widetilde{\varphi}_q(t_i) +1 >=C$, $\pi(q,t)=1$.
Define $\rho^*_{t_i}(q)$ where $ \frac{f(t_i)(t_i +\rho^*_{t_i}(q))}{(t_{i+1}-t_{i}) } +F(t_i) =C$. So we have $t_i+ \rho^*_{t_i}(q) =(t_{i+1}-t_{i})\frac{(C-F(t_i))}{f(t_i)}$ for any $t_i$. 


\begin{align*}
p(t_1) &= -u(t_1) + \sum_{\rho(q) \geq \rho^*_{t_1}(q)} g(q) v(q,t_1)  \\ 
&=   \sum_{\rho(q) \geq \rho^*_{t_1}(q)} g(q) v_1(q)[t_1+\rho(q)]  \\
&\geq   \sum_{\rho(q) \geq \rho^*_{t_1}(q)} g(q) v_1(q)[t_1+ \rho^*_{t_1}(q) ]  \\
&=   \sum_{\rho(q) \geq \rho^*_{t_1}(q)} g(q) v_1(q) (t_{2}-t_{1}) \frac{C - F(t_1)}{f(t_1)}  \\
&\geq 0
\end{align*}
where the last inequality is because $C\geq 0$ and $F(t_1)=0$. 

Similarly, utilizing $u(t_N) = v(t_N) = \sum_{q \in Q} g(q) v_1(q)[t_N + \rho(q)]$, we have
\begin{align*}
p(t_N) &= -u(t_N)  + \sum_{\rho(q) \geq \rho^*_{t_N}(q)} g(q) v(q,t_N)  \\ 
&=  - \sum_{q \in Q} g(q) v_1(q)[t_N + \rho(q)] + \sum_{\rho(q) \geq \rho^*_{t_N}(q) } g(q) v_1(q)[t_N+\rho(q)]  \\
&=  -   \sum_{\rho(q) <\rho^*_{t_N}(q) } g(q) v_1(q)[t_N+\rho(q)]  \\
&\geq   -   \sum_{\rho(q) <\rho^*_{t_N}(q) } g(q) v_1(q)[t_N+\rho^*_{t_N}(q)]  \\
& =  -   \sum_{\rho(q) <\rho^*_{t_N}(q) } g(q) v_1(q) (t_{N+1}-t_{N}) \frac{C - F(t_N)}{f(t_N)}     \\
&= 0
\end{align*}
where the last equality is because $t_{N+1}-t_{N} = 0$. 


Define $q^*(t)$ as the short notation for ${\rho^*_t}^{-1}(q)$.

$$
p(t_k) = \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k)  - \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1}) 
$$



\begin{align*}
&p(t_k) - p(t_{k-1})\\
=&   \sum_{q \in Q} g(q) \pi(q,t_k)v(q,t_k)  -  \sum_{i=2}^k(t_i - t_{i-1})P(t_{i-1})    - \sum_{q \in Q} g(q) \pi(q,t_{k-1})v(q,t_{k-1})  +  \sum_{i=2}^{k-1}(t_i - t_{i-1})P(t_{i-1})   \\
=&  \sum_{q \in Q} g(q) \pi(q,t_k) v(q,t_k) -(t_k - t_{k-1})\sum_{q \in Q}  \pi(q,t_{k-1})g(q)v_1(q) -\sum_{q \in Q} g(q) \pi(q,t_{k-1}) v(q,t_{k-1})\\
=&\sum_{q: \rho(q) \geq \rho^*_{t_k}(q)}g(q)v(q,t_k)-\sum_{q: \rho(q) \geq \rho^*_{t_{k-1}}(q)} g(q)v(q,t_{k-1})- (t_k - t_{k-1}) \sum_{q: \rho(q) \geq \rho^*_{t_{k-1}}(q)} g(q) v_1(q)\\
=&\sum_{q: \rho(q) \geq \rho^*_{t_{k-1}}(q)}g(q)v(q,t_k)-\sum_{q: \rho(q) \geq \rho^*_{t_{k-1}}(q)} g(q)v(q,t_{k-1}) + \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)}g(q)v(q,t_{k}) \\  
&- (t_k - t_{k-1}) \sum_{q: \rho(q) \geq \rho^*_{t_{k-1}}(q)} g(q) v_1(q)\\
=&(t_k - t_{k-1}) \sum_{q: \rho(q) \geq \rho^*_{t_{k-1}}(q)} g(q) v_1(q) + \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)}g(q)v(q,t_{k}) - (t_k - t_{k-1}) \sum_{q: \rho(q) \geq \rho^*_{t_{k-1}}(q)} g(q) v_1(q)\\
=&  \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)}g(q)v(q,t_{k})\\
=& \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)} g(q) v_1(\rho^{-1}(q)) (t_{k} + \rho(q)) \\ 
\geq& \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)} g(q) v_1(\rho^{-1}(q)) (t_{k} + \rho^*_{t_{k}}(q)) \\ 
=& \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)} g(q) v_1(\rho^{-1}(q))(t_{k+1} - t_k)\frac{C-F(t_k)}{f(t_k)} 
\end{align*}

Because of $g(q) v_1(\rho^{-1}(q))(t_{k+1} - t_k) > 0 $, we have $\forall k, s.t. \; F(t_k) \leq C, p(t_k) - p(t_{k-1}) \geq 0$. Since we have $p(t_1) \geq 0$, $p(t_k)$ is non-negative and non-decreasing $\forall k, s.t. \; F(t_k) \leq C$.


$$
\bar{p}(t_k) = \sum_{q\in Q} g(q) \pi(q,t_k)v(q,t_k) -v(t_N) + \sum_{i=k+1}^N(t_i - t_{i-1})P(t_{i})
$$

\begin{align*}
&p(t_k) - p(t_{k-1})\\
=&  \sum_{q \in Q} g(q) \pi(q,t_k) v(q,t_k) -(t_k - t_{k-1})\sum_{q \in Q}  \pi(q,t_{k})g(q)v_1(q) -\sum_{q \in Q} g(q) \pi(q,t_{k-1}) v(q,t_{k-1})\\
=&\sum_{q: \rho(q) \geq \rho^*_{t_k}(q)}g(q)v(q,t_k)-\sum_{q: \rho(q) \geq \rho^*_{t_{k-1}}(q)} g(q)v(q,t_{k-1})- (t_k - t_{k-1}) \sum_{q: \rho(q) \geq \rho^*_{t_{k}}(q)} g(q) v_1(q)\\
=&\sum_{q: \rho(q) \geq \rho^*_{t_{k}}(q)}g(q)v(q,t_k)-\sum_{q: \rho(q) \geq \rho^*_{t_{k}}(q)} g(q)v(q,t_{k-1}) + \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)}g(q)v(q,t_{k-1}) \\  
&- (t_k - t_{k-1}) \sum_{q: \rho(q) \geq \rho^*_{t_{k}}(q)} g(q) v_1(q)\\
=&(t_k - t_{k-1}) \sum_{q: \rho(q) \geq \rho^*_{t_{k}}(q)} g(q) v_1(q) + \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)}g(q)v(q,t_{k-1}) - (t_k - t_{k-1}) \sum_{q: \rho(q) \geq \rho^*_{t_{k}}(q)} g(q) v_1(q)\\
=&  \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)}g(q)v(q,t_{k-1})\\
=& \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)} g(q) v_1(\rho^{-1}(q)) (t_{k-1} + \rho(q)) \\ 
\leq& \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)} g(q) v_1(\rho^{-1}(q)) (t_{k-1} + \rho^*_{t_{k-1}}(q)) \\ 
=& \sum_{q:\rho^*_{t_{k}}(q) \leq \rho(q) < \rho^*_{t_{k-1}}(q)} g(q) v_1(\rho^{-1}(q))(t_{k} - t_{k-1})\frac{C-F(t_{k-1})}{f(t_{k-1})} 
\end{align*}


Because of $g(q) v_1(\rho^{-1}(q))(t_{k} - t_{k-1}) > 0 $, $\forall k, s.t. \; F(t_{k-1}) \geq C \Longrightarrow p(t_{k}) - p(t_{k-1}) \geq 0$.

In other words, $\forall k, s.t. \; F(t_{k}) \geq C \Longrightarrow p(t_{k}) - p(t_{k+1}) \leq 0$.

Since we have $p(t_N) \geq 0$, $p(t_{k})$ is non-negative and non-increasing $\forall t_k \; F(t_{k}) \geq C$. 


We proved $\forall t, \; p(t)\geq 0$. 
Thus, this mechanism is optimal and feasible.

\end{proof}


\begin{corollary} \label{dis-same-payment}
If recommendation policies are the same for any two types, then the payment is the same for these two types. Formally, $ \forall t_i \, \forall t_j$, where \, $ \forall q , \pi(q,t_i) = \pi(q,t_j)$, then $p(t_i) = p(t_j) $.
\end{corollary}

\begin{proof}
We can assume without generality $t_i \leq t_j$. Because $ \forall q, \pi(q,t_i) = \pi(q,t_j)$ and monotonicity of $\theta(t_i)$, we have  $ \forall t_i \leq t_k \leq t_j\, \forall q, \pi(q,t_i) = \pi(q,t_k) =\pi(q,t_j)$.
For case 1 in lemma \ref{dis-lem:two-simple-cases}.

\begin{align*}
p(t_i) &= \sum_{q \in Q} g(q) \pi(q,t_i)v(q,t_i)  - \sum_{k=2}^i(t_k - t_{k-1})P(t_{k-1}) \\
&= \sum_{q \in Q} g(q) \pi(q,t_j)v(q,t_j)  -  (t_j - t_i)\sum_{q \in Q} g(q) \pi(q,t_j)v_1(q) - \sum_{k=2}^i(t_k - t_{k-1})P(t_{k-1}) \\
&= \sum_{q \in Q} g(q) \pi(q,t_j)v(q,t_j)  -  \sum_{k=i+1}^{j} (t_k - t_{k-1}) \sum_{q \in Q} g(q) \pi(q,t_{k-1})v_1(q)    - \sum_{k=2}^i(t_k - t_{k-1})P(t_{k-1}) \\
&= \sum_{q \in Q} g(q) \pi(q,t_j)v(q,t_j)  - \sum_{k=2}^j(t_k - t_{k-1})P(t_{k-1}) \\
&= p(t_j)
\end{align*}

Ditto for other cases.


\end{proof}




==> existence.tex <==


\section{Additional Properties about the Optimal Mechanism} 







\begin{proposition}[Existence of Optimal Threshold Mechanism]
    There always exists an optimal mechanism that is a threshold mechanism. 
\end{proposition}
\begin{proof}
    \todo{need to revise the proof to make it nicer and smooth}
    From the revenue function \eqref{eq:revenue-2} using $t_2$ as the reference point, we have the following optimization problem.
    
    \begin{align*} 
        \max_{\pi} & \int_{t_1}^{t_2}  \int_{q \in Q} \left[ g(q) \pi(q,t) f(t)[v_1(q) \bar{\phi}(t) + v_0(q)]\,\mathrm{d}t \right] \mathrm{d}q \\
        \text{subject to} & \int_{t_1}^{t_2} \int_{q \in Q} g(q) \pi(q,t) v_1(q) dq dt \geq \int_{q \in Q} g(q) v(q,t_2) dq\\
        & P(t) \text{is monotone in }t
    \end{align*}
    
    
    To prove the lemma, we show that for any feasible solution to the above program, there exists a feasible threshold mechanism that weakly increases the objective function.
    
    Given a feasible mechanism $\pi(q, t)$, let threshold $\theta(t)$ be
    \begin{gather*}
        \theta(t)=\min\left\{\theta^*(t)\,\left|\, \int_{q: \rho(q) \geq \theta^*(t)}g(q)v_1(q)\,\mathrm{d}q=P(t)=\int_{q \in Q}g(q)\pi(q,t)v_1(q)\,\mathrm{d}q\right.\right\}.
    \end{gather*}
    $\theta(t)$ always exists, since the function $\int_{q: \rho(q) \geq \theta(t)}g(q)v_1(q)\,\mathrm{d}q$ is continuous and decreasing in $\theta(t)$, and $ \int_{q_2}^{q_2}g(q)v_1(q)\,\mathrm{d}q=0\le P(t)\le \int_{q \in Q}g(q)v_1(q)\,\mathrm{d}q$.
    
    Define a new allocation function as follows:
    \begin{gather*}
        \pi^*(q,t)=
        \begin{cases}
            1 & \text{ if } \rho(q)\ge \theta(t)\\
            0 & \text{ otherwise}
        \end{cases}.
    \end{gather*}
    It is clear that the corresponding $P(t)$ function is the same as the original $\pi(q,t)$: 
    \begin{gather}
        P^*(t)=\int_{q \in Q}g(q)\pi^*(q,t)v_1(q)\,\mathrm{d}q=\int_{q:\rho(q) \geq \theta(t)}g(q)v_1(q)\,\mathrm{d}q=P(t).
        \label{eq:Q_equal}
    \end{gather}
    Moreover, the left-hand-side of the $\int_{t_1}^{t_2} \int_{q \in Q} g(q) \pi(q,t) v_1(q) dq dt \geq \int_{q \in Q} g(q) v(q,t_2) dq$ constraint in this optimization problem
    \begin{gather*}
        \int_{t_1}^{t_2} \int_{q \in Q} g(q) \pi(q,t) v_1(q)\, \mathrm{d}q \mathrm{d}t=\int_{t_1}^{t_2}P(t)=\int_{t_1}^{t_2}P^*(t)\,\mathrm{d}t
    \end{gather*}
    also remains the same. The above two equations imply that $\pi^*(q,t)$ is also feasible. Now it suffices to show that $\pi^*(q,t)$ leads to a higher revenue. 
    
    Define
    \begin{gather*}
        \Phi(\rho(q), t) = f(t)\left[ \phi(t)+\rho(q) \right].
    \end{gather*}
    $\Phi(\rho(q),t)$ is monotone increasing in $\rho(q)$ and $f(t)$ is always non-negative. Thus if $\rho(q)\ge \theta(t)$, $\pi^*(q,t)=1\ge \pi(q,t)$, and $\Phi(\rho(q),t)\ge \Phi(\theta(t),t)$, and if $\rho(q)< \theta(t)$, $\pi^*(q,t)=0\le \pi(q,t)$, and $\Phi(\rho(q),t)\le \Phi(\theta(t),t)$. Therefore,
    \begin{gather}
        \left[ \pi^*(q,t)-\pi(q,t) \right]\left[ \Phi(\rho(q),t)-\Phi(\theta(t),t) \right]\ge 0, \forall q, t. \label{eq:monotone}
    \end{gather}
    The revenue difference of the two mechanisms $\pi(q,t)$ and $\pi^*(q,t)$ is:
    \begin{align*}
        &\int_{t_1}^{t_2}  \int_{q \in Q} g(q) \left[\pi^*(q,t)-\pi(q,t)\right] f(t)[v_1(q) \phi(t) + v_0(q)]\,\mathrm{d}q \mathrm{d}t\\
        =&\int_{t_1}^{t_2}  \int_{q \in Q} g(q) \left[\pi^*(q,t)-\pi(q,t)\right] v_1(q)\Phi(\rho(q),t)\,\mathrm{d}q \mathrm{d}t\\
        \ge&\int_{t_1}^{t_2}  \int_{q \in Q} g(q) \left[\pi^*(q,t)-\pi(q,t)\right] v_1(q)\Phi(\theta(t),t)\,\mathrm{d}q \mathrm{d}t\\
        =&\int_{t_1}^{t_2} \Phi(\theta(t),t) \int_{q \in Q} g(q) \left[\pi^*(q,t)-\pi(q,t)\right] v_1(q)\,\mathrm{d}q \mathrm{d}t\\
        =&\int_{t_1}^{t_2} \Phi(\theta(t),t) \left[P^*(t)-P(t)\right]\, \mathrm{d}t\\
        =&0,
    \end{align*}
    where the inequality is because of Equation \eqref{eq:monotone} and the last equation is due to Equation \eqref{eq:Q_equal}.
\end{proof}

\begin{proposition}[Information Determines Payments]
    If the signaling scheme is the same for any two different buyer types, then the payment is the same for these two types. Formally, for any $ t \not = t'$, if $  \pi(q,t) = \pi(q,t')$ for all $q$, then $p(t) = p(t') $. 
\end{proposition}

\begin{proof}
    We can assume without generality $t \leq t'$. Because $ \forall q, \pi(q,t) = \pi(q,t')$ and monotonicity of $\theta(t)$, we have  $ \forall t \leq t^* \leq t'\, \forall q, \pi(q,t) = \pi(q,t^*) =\pi(q,t')$.
    
    \begin{align*}
        p(t) &= \int_{q \in Q} g(q) \pi(q,t)v(q,t) dq -  \int_{t_1}^{t} P(x)  dx \\
        &= \int_{q \in Q} g(q) \pi(q,t')v(q,t) dq -  \int_{t_1}^{t} P(x)  dx \\
        &= \int_{q \in Q} g(q) \pi(q,t')v(q,t') dq -  (t' - t)\int_{q \in Q} g(q) \pi(q,t')v_1(q) dq - \int_{t_1}^{t} P(x)  dx \\
        &= \int_{q \in Q} g(q) \pi(q,t')v(q,t') dq -  \int_{t}^{t'} \int_{q \in Q} g(q) \pi(q,x)v_1(q) dq  dx  -  \int_{t_1}^{t} P(x)  dx \\
        &= \int_{q \in Q} g(q) \pi(q,t')v(q,t') dq -  \int_{t}^{t'} P(x)  dx  -  \int_{t_1}^{t} P(x)  dx \\
        &= \int_{q \in Q} g(q) \pi(q,t')v(q,t') dq -   \int_{t_1}^{t'} P(x)  dx \\
        &= p(t')
    \end{align*}
    
    Ditto for other cases.
    
    
\end{proof}


Now, let us discuss the relationship between $\widetilde{\phi}_q(t)$ and $\bar{\phi}(t),\underline{\phi}(t)$.

\begin{lemma}
    If $\widetilde{\phi}_q(t) = f(t)t + F(t) + f(t)\rho(q) = f(t)  [\bar{\phi}(t) + \rho(q)]$ is non-decreasing in t for any q, then $\bar{\phi}(t) $ and $\underline{\phi}(t) $ is non-decreasing in t in the range of $\rho(q)$.
\end{lemma}
\begin{proof}
    We can prove it by contradiction.
    
    If $\bar{\phi}(t) $ is not non-decreasing in t, then $\exists t_1<t_2 \; s.t. \; \bar{\phi}(t_1) > \bar{\phi}(t_2)$.
    Take $\rho(q) = - \frac{\bar{\phi}(t_1) + \bar{\phi}(t_2)}{2}$
    
    \begin{align*}
        \widetilde{\phi}_q(t_1) &= f(t_1)t_1 + F(t_1) + f(t_1)\rho(q) \\
        &= f(t_1)  [\bar{\phi}(t_1) + \rho(q)] \\
        &= f(t_1)  [\frac{\bar{\phi}(t_1) - \bar{\phi}(t_2)}{2}] \\
        &\geq 0 \\
        \widetilde{\phi}_q(t_2) &= f(t_2)t_2 + F(t_2) + f(t_2)\rho(q) \\
        &= f(t_2)  [\bar{\phi}(t_2) + \rho(q)] \\
        &= f(t_2)  [\frac{\bar{\phi}(t_2) - \bar{\phi}(t_1)}{2}] \\
        &\leq 0
    \end{align*}
    
    Contradiction. So, $\bar{\phi}(t)$ should be non-decreasing in the range of $\rho(q)$. Ditto for $\underline{\phi}(t)$.
    
    
\end{proof}

% \sz{May change this lemma to show relationship between threshold on $\rho(q)$ and threshold on $q$ 
% \begin{lemma}
% There exists a threshold mechanism that solves the above mathematical program optimally if $\frac{v_0(q)}{v_1(q)}$ is increasing in $q$.
% \end{lemma}
% \begin{proof}
%     To prove the lemma, we show that for any feasible solution to the above program, there exists a feasible threshold mechanism that weakly increases the objective function.

%     Given a feasible mechanism $\pi(q, t)$, let $q^*(t)$ be
%     \begin{gather*}
%     q^*(t)=\argmin_{q^*}\left\{q^*\,\left|\, \int_{q^*}^{q_2}g(q)v_1(q)\,\mathrm{d}q=P(t)=\int_{q \in Q}g(q)\pi(q,t)v_1(q)\,\mathrm{d}q\right.\right\}.
%     \end{gather*}
%     $q^*(t)$ always exists, since the function $\int_{q^*}^{q_2}g(q)v_1(q)\,\mathrm{d}q$ is continuous and decreasing in $q^*$, and
%     \begin{gather*}
%     \int_{q \in Q }g(q)v_1(q)\,\mathrm{d}q=0\le P(t)\le \int_{q \in Q}g(q)v_1(q)\,\mathrm{d}q.
%     \end{gather*}

%     Define a new allocation function as follows:
%     \begin{gather*}
%     \pi'(q,t)=
%     \begin{cases}
%     1 & \text{ if } q\ge q^*(t)\\
%     0 & \text{ otherwise}
%     \end{cases}.
%     \end{gather*}
%     It is clear that the corresponding $P(t)$ function is the same as the original $\pi(q,t)$: 
%     \begin{gather}
%     P^*(t)=\int_{q \in Q}g(q)\pi'(q,t)v_1(q)\,\mathrm{d}q=\int_{q^*(t)}^{q_2}g(q)v_1(q)\,\mathrm{d}q=P(t).
%     \label{eq:Q_equal}
%     \end{gather}
%     Moreover, the left-hand-side of the first constraint
%     \begin{gather*}
%     \int_{t_1}^{t_2} \int_{q \in Q} g(q) \pi(q,t) v_1(q)\, \mathrm{d}q \mathrm{d}t=\int_{t_1}^{t_2}P(t)\,\mathrm{d}t
%     \end{gather*}
%     also remains the same. The above two equations imply that $\pi'(q,t)$ is also feasible. Now it suffices to show that $\pi'(q,t)$ leads to a higher revenue. The proof is immediate if we notice that the original program is very similar to the fractional knapsack problem. However, we still include a proof here to make it self-contained.

%     Define
%     \begin{gather*}
%     \Phi(q, t) = f(t)\left[ \phi(t)+\frac{v_0(q)}{v_1(q)} \right].
%     \end{gather*}
%     $\Phi(q,t)$ is monotone increasing in $q$ since $\frac{v_0(q)}{v_1(q)}$ is increasing and $f(t)$ is always non-negative. Thus if $q\ge q^*(t)$, $\pi'(q,t)=1\ge \pi(q,t)$, and $\Phi(q,t)\ge \Phi(q^*(t),t)$, and if $q< q^*(t)$, $\pi'(q,t)=0\le \pi(q,t)$, and $\Phi(q,t)\le \Phi(q^*(t),t)$. Therefore,
%     \begin{gather}
%     \left[ \pi'(q,t)-\pi(q,t) \right]\left[ \Phi(q,t)-\Phi(q^*(t),t) \right]\ge 0, \forall q, t. \label{eq:monotone}
%     \end{gather}
%     The revenue difference of the two mechanisms $\pi(q,t)$ and $\pi'(q,t)$ is:
%     \begin{align*}
%     &\int_{t_1}^{t_2}  \int_{q \in Q} g(q) \left[\pi'(q,t)-\pi(q,t)\right] f(t)[v_1(q) \phi(t) + v_0(q)]\,\mathrm{d}q \mathrm{d}t\\
%     =&\int_{t_1}^{t_2}  \int_{q \in Q} g(q) \left[\pi'(q,t)-\pi(q,t)\right] v_1(q)\Phi(q,t)\,\mathrm{d}q \mathrm{d}t\\
%     \ge&\int_{t_1}^{t_2}  \int_{q \in Q} g(q) \left[\pi'(q,t)-\pi(q,t)\right] v_1(q)\Phi(q^*(t),t)\,\mathrm{d}q \mathrm{d}t\\
%     =&\int_{t_1}^{t_2} \Phi(q^*(t),t) \int_{q \in Q} g(q) \left[\pi'(q,t)-\pi(q,t)\right] v_1(q)\,\mathrm{d}q \mathrm{d}t\\
%     =&\int_{t_1}^{t_2} \Phi(q^*(t),t) \left[Q'(t)-P(t)\right]\, \mathrm{d}t\\
%     =&0,
%     \end{align*}
%     where the inequality is because of Equation \eqref{eq:monotone} and the last equation is due to Equation \eqref{eq:Q_equal}.
% \end{proof}

% }


% \begin{lemma}
% The solution to the above mathematical program is a threshold mechanism if the following function is monotone increasing in both $t$ and $q$:
% \begin{gather*}
%     \Phi(q, t) = f(t)\left[ \phi(t)+\frac{v_0(q)}{v_1(q)} \right].
% \end{gather*}
% \end{lemma}
% \begin{remark}
% The above condition is also equivalent to the following two conditions:
% \begin{itemize}
%     \item $\frac{v_1(q)}{v_0(q)}$ is increasing in $q$;
%     \item $\frac{f'(t)}{f(t)}\frac{v(q,t)}{v_1(q)}\ge -2$.
% \end{itemize}
% \end{remark}
% To prove this result, we first relax the second constraint and show that the solution to the relaxed program is a special class of allocation rules. Then we prove that the this special class of rules automatically satisfies the second constraint.
% \begin{proof}
% % Let
% % \begin{gather*}
% %     D_+=\{(t, q)\mid v_1(q)\phi(t)+v_0(q)\ge 0\},\\
% %     D_-=\{(t, q)\mid v_1(q)\phi(t)+v_0(q)< 0\}.
% % \end{gather*}
% % Thus the objective function can be written as:
% % \begin{gather*}
% %     \left(\int_{D_+}-\int_{D_-}\right)g(q)\pi(q,t)f(t)|v_1(q)\phi(t)+v_0(q)|\,\mathrm{d}t\mathrm{d}q.
% % \end{gather*}

% Let's relax the second constraint first. Similar to the fractional knapsack problem, the optimal solution to the relaxed program is to ``sort'' the ratio
% \begin{gather*}
%     \frac{g(q) \pi(q,t) f(t)[v_1(q) \phi(t) + v_0(q)]}{g(q) \pi(q,t) v_1(q)}=\Phi(q, t)
% \end{gather*}
% in descending order and set $\pi(q, t)=1$ greedily until the first constraint is satisfied. Therefore, the solution to the relaxed program must have the following format: 
% \begin{gather}
%     \pi_h(q, t)=
%     \begin{cases}
%     1 & \text{~if~} \Phi(q, t) \ge h\\
%     0 & \text{~otherwise}
%     \end{cases},
% \end{gather}
% where $h$ is a parameter.

% Now we show that the above class of allocation rules also satisfies the second constraint. Consider the function $\underline{q}(t|h)=\inf\{q\mid \Phi(q, t)\ge h\}$. It is easy to see that when $\Phi(q, t)$ is increasing in both $t$ and $q$, $\underline{q}(t|h)$ is always a decreasing function for all $h$, and that $\pi_h(q, t)=1$ for all $\underline{q}(t|h)\le q\le q_2$. We claim that the corresponding $P(t)$ is monotone in $t$. This is because for any $t<t'$,
% \begin{align*}
%     P(t')-P(t)&=\int_q\pi_h(q,t')g(q)v_1(q)\,\mathrm{d}q-\int_q\pi_h(q,t)g(q)v_1(q)\,\mathrm{d}q\\
%     &=\int_{\underline{q}(t'|h)}^{q_2}g(q)v_1(q)\,\mathrm{d}q-\int_{\underline{q}(t|h)}^{q_2}g(q)v_1(q)\,\mathrm{d}q\\
%     &=\int_{\underline{q}(t'|h)}^{\underline{q}(t|h)}g(q)v_1(q)\,\mathrm{d}q\\
%     &\ge 0,
% \end{align*}
% where the inequality comes from the fact that $\underline{q}(t|h)$ is a decreasing function.

% Also, $\pi_h(q, t)$ gives a threshold mechanism because $\pi_h(q, t)=1$ for all $\underline{q}(t|h)\le q\le q_2$.
% \end{proof}







% \subsection{The Case with Regular $F$ and Non-negative $v_1(q) $} 
% When $v_1(q) \geq 0$, we know that $P(t) \geq 0$ for all $t$. The minimum value of $u(t_2)$ is $\max \{ 0, v(t_2) \}$. Therefore, the maximum possible value of  $REV (\pi, p)$ will be achieved by setting $u(t_2) = \max \{ 0, v(t_2) \}$ and $\pi(q,t) = 1$ whenever $v_1(q) \phi(t) + v_0(q) \geq 0$ and $\pi(q,t) = 0$ otherwise. What remains to verify is that this mechanism does satisfy all the conditions in Lemma \ref{lem:feasible-M}. 

% Since $v_1(q) \phi(t) + v_0(q)$ is monotone increasing in $t$ when $F$ is regular and $v_1(q) \geq 0$. The $\pi$ above is a \emph{threshold signaling scheme} which signals $1$ to buyer type $t$ whenever \hf{need to assume $- \frac{ v_0(q)}{v_1(q) } $ is decreasing in $q$}   
% \begin{equation}
%      - \frac{ v_0(q)}{v_1(q) }   \leq \phi(t) 
% \end{equation}
% Since $- \frac{ v_0(q)}{v_1(q) } $ is decreasing in $q$ and $\phi(t)$ is increasing in $t$, there exists a threshold $\theta(t)$ such that $\pi(q,t) = 1$ for any $q \geq \theta(t)$ and $\pi(q,t)=0$ otherwise. Moreover, $\theta(t)$ is decreasing in $t$. This can equivalently be viewed as a therhsold mechanism on $t$ where $\pi(q,t) = 1$ whenever $t \geq \beta{q}$ where $\beta(q)$ is now an increasing function in $q$. In fact, $\beta(q)$ minimize function $U(t;q) = F(t)v(q,t) = F(t)[v_1(q)t + v_0(q) ] $. We have $U'(t;q) = f(t)[v_1(q)t + v_0(q) ] + F(t) v_1(q) = f(t) [v_1(q) \phi(t) + v_0(q)]$ which is positive for $t \geq \beta(q)$ and negative otherwise. Thus, $\beta(q)$ minimizes $U(t;q)$. 


% It is easy to verify such a threshold policy satisfy monotonicity. We only need to guarantee $u(t_1) \geq 0$, or equivalently $p(t_1) \leq \int_{q \in Q} g(q) \pi(q,t_1) v(q,t_1) dq = B_{t_1}$, and $u(t_2) \geq v(t_2)$, or equivalently $p(t_2) \leq \int_{q \in Q} g(q) \pi(q,t_2) v(q,t_2) dq - \int_{q \in Q} g(q) v(q,t_2) dq =B_{t_2}$.  Note that $p(t_2) - p(t_1) = \int_{t_1}^{t_2} p'(t)dt$ which only depends on the signaling scheme $\pi$. Therefore, we would like to figure which of the upper band is tight.

% Note that
% \begin{eqnarray}
% p(t) = \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq  - \int_{t_1}^{t} P(t) dt  - u(t_1) 
% \end{eqnarray}

% Therefore,
% \begin{eqnarray}
% p(t_2) - p(t_1) = \int_{q \in Q} g(q) \pi(q,t_2) v(q,t_2) dq - \int_{q \in Q} g(q) \pi(q,t_1) v(q,t_1) dq   - \int_{t_1}^{t_2} P(t) dt
% \end{eqnarray}
% \begin{eqnarray}
% B_{t_2} - B_{t_1} = \int_{q \in Q} g(q) \pi(q,t_2) v(q,t_2) dq - \int_{q \in Q} g(q) \pi(q,t_1) v(q,t_1) dq  - \int_{q \in Q} g(q) v(q,t_2) dq 
% \end{eqnarray}
% Therefore, it remains to compare $\int_{q \in Q} g(q) v(q,t_2) dq = v(t_2)$ and $\int_{t_1}^{t_2} P(t) dt$. 

% The following claim illustrate the fundamental difficulty in this optimization. When using $t_2$ as the basis, we know $u_1 = 0$ is guaranteed, thus $u_2$ will be changed when we adjust $\pi$ to achieve obedience. How to change $\pi$ to maximize the Rev function on page 9 with $u(t_2)$, which also depend on $\pi$. Conversely, if we use $t_1$ as basis, we know $u(t_2) = v(t_2)$ and $u(t_1)$ will change and we face the same difficulty. Myerson does not have this problem since in his problem $u(t_1) = 0$ for sure and he does not need to adjust the $\pi$. 
% \begin{claim}
% $p(t_2) - p(t_1) \leq B_{t_2} - B_{t_1} $ when using $t_1$ as basis and $p(t_2) - p(t_1) \geq B_{t_2} - B_{t_1} $ when using $t_2$ as basis. 
% \end{claim}
% \begin{proof}
% Let $\beta(q)$ denote the threshold for $t$. We have 
% \begin{eqnarray}
% & & p(t_2) - p(t_1)  - [B_{t_2} - B_{t_1}] \\
% & = & \int_{q \in Q} g(q) v(q,t_2) dq  - \int_{t_1}^{t_2} P(t) dt \\
% &=& \int_{q \in Q} g(q) v(q,t_2) dq - \int_{t_1}^{t_2} \int_{q \in Q} g(q) \pi(q,t) v_1(q) dq dt \\ 
% &=& \int_{q \in Q} g(q) v(q,t_2) dq - \int_{q \in Q} g(q) (t_2 - \beta(q)) v_1(q) dq \\
% &=& \int_{q \in Q} g(q) [v_1(q)t_2 + v_0(q)] dq - \int_{q \in Q} g(q) (t_2 - \beta(q)) v_1(q) dq \\
% &=& \int_{q \in Q} g(q) [v_1(q)\beta(q) + v_0(q)] dq 
% \end{eqnarray}
% because $v_1(q)\beta(q) + v_0(q) \leq 0$ for any $q$ when using $u_2$ as basis on Page 9 and $v_1(q)\beta(q) + v_0(q) \geq 0$ for any $q$ when using $u_1$ as basis on Page 9.  
% \end{proof}


% \begin{eqnarray}
% p(t) &=& p(t_2) - \int_{t}^{t_2} p'(x)dx   \\
% &=& p(t_2) - \int_{t}^{t_2}  \int_{q \in Q}  g(q) \frac{\partial \pi(q,x)}{\partial x}  v(q,x)    dq  dx   \\
% &=& p(t_2)  - \int_{q \in Q} g(q) \pi(q,t2) v(q,t_2) dq + \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq   + \int_{t}^{t_2} P(x) dx  \\
% &=&  \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} P(x) dx - u(t_2) \\
% &=&  \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} P(x) dx  - \max\{0, v(t_2 \}) \\ 
% &=&  \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} \int_{q \in Q} g(q) \pi(q,x) v_1(q) dq   dx  - \max\{0, v(t_2 \}) \end{eqnarray}

% If $p(t_1) = \int_{q \in Q} g(q) \pi(q,t_1) v(q,t_1)$, then $u(t_1) = 0 $. We claim $u(t_2) \geq v(t_2)$ is also satisfied, because 
% \begin{eqnarray}
% p(t) &=& p(t_2) - \int_{t}^{t_2} p'(x)dx   \\
% &=& p(t_2) - \int_{t}^{t_2}  \int_{q \in Q}  g(q) \frac{\partial \pi(q,x)}{\partial x}  v(q,x)    dq  dx   \\
% &=& p(t_2)  - \int_{q \in Q} g(q) \pi(q,t2) v(q,t_2) dq + \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq   + \int_{t}^{t_2} P(x) dx  \\
% &=&  \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} P(x) dx - u(t_2) \\
% &=&  \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} P(x) dx  - \max\{0, v(t_2 \}) \\ 
% &=&  \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} \int_{q \in Q} g(q) \pi(q,x) v_1(q) dq   dx  - \max\{0, v(t_2 \}) \end{eqnarray}


% Remains to verify $p(t) \geq 0, u(t_1) \geq 0$?

% \begin{eqnarray}
% p(t_2) &=&  \int_{q \in Q} g(q) \pi(q,t_2) v(q,t_2) dq   - \max\{0, v(t_2 \}) \\ 
% \end{eqnarray}
% $\pi(q,t_2) = 1$ whenever $q \geq \theta(t_2) $ or equivalently $ v(q,t_2) + v_1(q) \frac{F(t_2)}{f(t_2)} \geq 0 $. 



% What remains to verify is $p(t) \geq 0$, as follows:
% \begin{eqnarray}
% p(t)  &=&  \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq + \int_{t_1}^t P(x) dx   \\ 
%  &=&  \int_{q \in Q} g(q) \pi(q,t) v(q,t) dq + \int_{t_1}^t \int_{q \in Q} g(q) \pi(q,x)  v_1(q)  dq  dx   \\  
% \end{eqnarray}


% As $\odv{u(t)}{t}\ge0$, we can set $u(0)=0$. Let
% \begin{gather*}
% \phi(t|q)=v(q,t)-\pdv{v(q,t)}{t}\frac{1-F(t)}{f(t)}.
% \end{gather*}
% We have
% \begin{gather*}
% REV=\int_{q \in Q} g(q)\left[ \int_{t_1}^{t_2} f(t)\pi_t(q,1)\phi(t|q)\,\mathrm{d}t \right].
% \end{gather*}
% Similar to the Myerson auction, there is a threshold $\theta_q$ for each $q$. We may need the ``ironing'' trick and define
% \begin{gather*}
% R(\eta|q)=v\cdot \eta,
% \end{gather*}
% where $\eta=1-F(t)$. And we also have $\pdv{R(\eta|q)}{\eta}=\phi(t|q)$.

% With Equation \eqref{eq:allocation_monotonicity}, any threshold testing mechanism must satisfy that $\theta(t)$ is decreasing in $t$. If the optimal mechanism is a threshold testing mechanism, then $\theta_q$ must also be a decreasing function of $q$. With the regularity assumption, we have
% \begin{gather*}
% v(q,\theta_q)-\pdv{v(q,\theta_q)}{\theta_q}\frac{1-F(\theta_q)}{f(\theta_q)}=0.
% \end{gather*}
% Therefore, the optimal mechanism is a threshold testing mechanism if and only if
% \begin{gather*}
% \odv{\theta_q}{q}\le 0,
% \end{gather*}
% where
% \begin{gather*}
% \odv{\theta_q}{q}=-\frac{\pdv{v(q,\theta_q)}{q}-\pdv{v(q,\theta_q)}{q,\theta_q}\frac{1-F(\theta_q)}{f(\theta_q)}}{\pdv{v(q,\theta_q)}{\theta_q}-\pdv[2]{v(q,\theta_q)}{\theta_q}\frac{-f^2(\theta_q)-(1-F(\theta_q))f'(\theta_q)}{f^2(\theta_q)}}
% \end{gather*}


==> ironing-case-3.tex <==
\subsection{Ironing Non-Regular Virtual Values for case 3} 

As mentioned  in lemma \ref{midcase} We can simplify the optimization problem to
\begin{align*}
\max_{\pi} &  \int_{t_1}^{t_2} \int_{q \in Q} g(q) \pi(q,t) v_1(q) f(t)  [\underline{\phi}(t) + \rho(q)]\,\mathrm{d}q  \mathrm{d}t  \\
\text{subject to} & \int_{t_1}^{t_2} \int_{q \in Q} g(q) \pi(q,t) v_1(q) dq dt = v(t_2)\\
& P(t) \text{is monotone in }t
\end{align*}

$\underline{\phi}(t) = t - \frac{1-F(t)}{f(t)}$


Without regularity where $\widetilde{\phi}_q(t) =  f(t)[\underline{\phi}(t) + \rho(q)] =  f(t)t + F(t) + f(t)\rho(q) -1$ is non-decreasing in $t$ for any $q$, this mechanism will not be feasible, since $P(t)$ will not be monotone non-decreasing in $t$. So, we are going to use ironing trick \cite{RePEc:inm:ormoor:v:6:y:1981:i:1:p:58-73} to extend our solution to general case.

For information buyer $t$, we now define four functions which have the unit interval [0,1] as their domain. First, for any $w$ in [0,1], let

$$
h_q(w) = f(F^{-1}(w))F^{-1}(w) + F^{-1}(w) + f(F^{-1}(w))\rho(q) -1  = \widetilde{\phi}_q(F^{-1}(w) )
$$

and let

$$
H_q(w) = \int_{0}^{w} h(r) dr
$$

Next let $L_q: [0,1] \rightarrow \mathbb{R}$ be the convex hull of the function $H_q(\cdot)$,

\begin{align*}
    L_q(w) &= \text{conv} \; H_q(w)\\
    &= \min\{\omega H_q(r_1) + (1-\omega)H_q(r_2) \| \\ 
    &{\omega,r_1,r_2} \subset [0,1] \; \text{and} \; \omega r_1 + (1-\omega)r_2 = w \}
\end{align*}

That is $L_q(\cdot)$ is the highest convex function on $[0,1]$ such that $\forall w \; L_q(w) \leq H_q(w)$.

As a convex function, $L_q$ is continuously differentiable except at countbaly many points and its derivative is monotone increasing. We define $l_q: [0,1] \rightarrow \mathbb{R}$ so that
$$
l_q(w) = L_q'(w)
$$
whenever this derivative is defined, and we extend $l_q(\cdot)$ to all of $[0,1]$ by right-continuity.
We define $\bar{c}_q : [t_1,t_2] \rightarrow \mathbb{R}$ so that
$$
\bar{c}_q(t) = l_q(F(t))
$$

It is straightforward to check that, in the regular case when $c_q(\cdot)$ is non-decreasing, we get $L_q = H_q, l_q = h_q, \bar{c}_q = \widetilde{\phi}_q(t)$.

We can now state our main result: the optimal mechanism is a threshold mechanism on $\rho(q)$ with threshold $\theta(t) = \bar{c}_{t}^{-1}(C)  $, where $C$ is a constant between -1 to 0 and satisfies  $\int_{(t,q):   \bar{c}_q(t) >= C } g(q)  v_1(q) dq dt = v(t_2)$. 

\sz{After ironing, we do not know whether $\bar{c}_q(t)$ is increasing on $\rho(q)$ and we do not have the formula of $\bar{c}_q(t)$, so we can't define the threshold in a close form. But we can assume it for now.}

\begin{lemma} \label{ironing-lemma}
With recommendation policy,
    \begin{gather*}
    \bar{\pi}(q,t)=
    \begin{cases}
    1 & \text{ if } \rho(q)\ge \bar{c}_{t}^{-1}(C) \\
    0 & \text{ otherwise}
    \end{cases}.
    \end{gather*}
and payment function
$$
\bar{p}(t) = \int_{q\in Q} [\bar{\pi}(q,t)g(q) v(q,t)] dq -  \int_{t_1}^{t}\int_{q \in Q} \bar{\pi}(q,t) g(q) v_1(q)dq  dx
$$
Above $(\bar{\pi}(q,t) , \bar{p}(t) ) $ represents an optimal information selling mechanism for lemma \ref{lem:optimal-case1} without requiring $\widetilde{\phi}_q(t)$ is non-decreasing for any $q$.
\end{lemma}



\begin{proof}





\begin{align}
REV (\pi, p) =&\int_{q \in Q} g(q)\left[ \int_{t_1}^{t_2} f(t)\pi(q,t) v_1(q) [\underline{\phi}(t) + \rho(q)]\,\mathrm{d}t \right] \mathrm{d}q  -u(t_1) \nonumber \\
= &\int_{q \in Q} \int_{t_1}^{t_2} [\underline{\phi}(t) + \rho(q)] f(t)\pi(q,t)  g(q) v_1(q) dt dq  \nonumber \\
= &\int_{q \in Q} \int_{t_1}^{t_2} h(F(t)) \pi(q,t)  g(q) v_1(q) dt dq  \nonumber \\
= &\int_{q \in Q} \int_{t_1}^{t_2} \bar{c}(t) \pi(q,t)  g(q) v_1(q) dt dq \nonumber\\ 
&+ \int_{q \in Q} \int_{t_1}^{t_2} [h(F(t))- l(F(t))]\pi(q,t)  g(q) v_1(q) dt dq  \nonumber \\
= &\int_{q \in Q} \int_{t_1}^{t_2} \bar{c}(t) \pi(q,t)  g(q) v_1(q) dt dq \nonumber \\ 
& - \int_{t_1}^{t_2} [H(F(t))- L(F(t))] d P(t)  \label{ironing-rev}
\end{align}


Now consider $(\bar{\pi}(q,t) , \bar{p}(t) ) $ as defined in the lemma. Observe that $\bar{\pi}(q,t)$ always sets $\pi(q,t) = 1, \; \forall q,t, \; s.t.\; \rho(q)\ge \bar{c}_{t}^{-1}(C)$. Thus, any other $\pi(q,t)$ will choose some term $< C$ to substitute the term $\leq C$. So, we have,

\begin{equation} \label{ironing-1}
\int_{q \in Q} \int_{t_1}^{t_2} [\bar{c}(t) + \rho(q)] f(t)\bar{\pi}(q,t)  g(q) v_1(q) dt dq \geq \\ \int_{q \in Q} \int_{t_1}^{t_2} [\bar{c}(t) + \rho(q)] f(t)\pi(q,t)  g(q) v_1(q) dt dq
\end{equation}

$$   P(t) = \int_{q \in Q}  \pi(q, t)  g(q) v_1(q)dq $$

Using integration by parts, we derive the following equations. \sz{Because the first term is weakly increasing, how to prove similar things like the following is critical. Where we do not have $f(t)$ in the second term.}

\begin{align*}
& \int_{q \in Q} \int_{t_1}^{t_2} [h(F(t))- l(F(t))] f(t)\pi(q,t)  g(q) v_1(q) dt dq \\
&= \int_{t_1}^{t_2} [h(F(t))- l(F(t))] f(t)P(t) dt \\
&= [H(F(t))- L(F(t))] P(t) \|_{t=t_1}^{t_2}  - \int_{t_1}^{t_2} [H(F(t))- L(F(t))] d P(t) 
\end{align*}

\begin{align*}
& \int_{q \in Q} \int_{t_1}^{t_2} [h(F(t))- l(F(t))]\pi(q,t)  g(q) v_1(q) dt dq \\
&= \int_{t_1}^{t_2} [h(F(t))- l(F(t))]P(t) dt \\
\end{align*}

If we want to use integral by parts, we need to compute $\int h(F(t)) dt $
\begin{align*}
& \int h(F(t) dt = \int \frac{1}{f(t)} h(F(t))f(t) dt\\
&= \frac{1}{f(t)} H(F(t)) -  \int (\frac{1}{f(t)})' h(F(t)f(t) dt \\
&= \frac{1}{f(t)} H(F(t)) - (\frac{1}{f(t)})' H(F(t)) + \int (\frac{1}{f(t)})'' h(F(t))f(t) dt \\
&= \sum_{i=0}^{n}(-1)^i \frac{1}{f(t)}^{(i)} H(F(t))  + (-1)^n \cdot \int (\frac{1}{f(t)})^{(n)} h(F(t))f(t) dt  \\
\end{align*}


Because $L$ is the convex hull of $H$ on $[0,1]$ and H is continuous, so $L(0) = H(0)$ and $L(1) = H(1)$. Thus the endpoint terms in $ [H(F(t))- L(F(t))] P(t) \|_{t=t_1}^{t_2}$ are $0$.

With $\bar{p}(t)$, $u(t_1) = 0$.


For any $\pi(q,t)$ which satisfies \eqref{eq:signal-monotonicity}, since $H \geq L$ and we are looking for a feasible mechanism where $P(t)$ is monotone non-decreasing, we must have 
\begin{equation} \label{ironing-2}
\int_{t_1}^{t_2} [H(F(t))- L(F(t))] d P(t) \geq 0
\end{equation}



To see that $ \bar{P}(t) = \int_{q \in Q}  \pi(q, t)  g(q) v_1(q)dq $ satisfies \eqref{eq:signal-monotonicity}, observe first that $\bar{c}(t)$ is a non-decreasing function of $t$, because $F$ and $l$ are both non-decreasing functions. Thus, $\bar{\pi}(q,t)$ is non-decreasing on $t$ and $\bar{P}(t)$ is also non-decreasing on $t$.

Since $L$ is the convex hull of $H$, we know that $L$ must be flat when ever $L < H$; that is, if $L(r)<H(r)$ then $l'(r) = L''(r) = 0$. So, if $H(F(t))-L(F(t)) > 0$ then $\bar{c}(t)$ and $\bar{P}(t)$ are constant in some neighborhood of $t$. This implies that

\begin{equation} \label{ironing-3}
\int_{t_1}^{t_2} [H(F(t))- L(F(t))] d \bar{P}(t) = 0
\end{equation}

Substituting \eqref{ironing-1} \eqref{ironing-2} \eqref{ironing-3} into \eqref{ironing-rev}, we can see $\pi(q,t)$ maximizes the revenue function, subject to \eqref{eq:signal-monotonicity}. 

This fact, together lemma \ref{lem:optimal-case1} proves our main theorem \ref{thm:opt-scheme}.


\end{proof}

==> irregular.tex <==

\subsection{Ironing Non-Regular Virtual Values} 
\todo{need to revise this section to make it nicer and smooth}


Without regularity where $\underline{\phi}(t) = t - \frac{1-F(t)}{f(t)}$ is non-decreasing in $t$, this mechanism will not be feasible, since $P(t)$ will not be monotone non-decreasing in $t$. So, we are going to use ironing trick introduced by \cite{RePEc:inm:ormoor:v:6:y:1981:i:1:p:58-73} and defined in definition \ref{def:ironing} to extend our solution to general case.


Now, we can extend our lemma on case 1 to a more general case without requiring $\underline{\phi}(t)$ is non-decreasing, since we can iron $\underline{\phi}(t)$ to get an non-decreasing $\underline{\phi}^+(t)$.

We now show in lemma \ref{ironing-lemma} after ironing, revenue is weakly increased.

\begin{lemma} \label{ironing-lemma}
    With recommendation policy,
    \begin{gather*}
        {\pi}^*(q,t)=
        \begin{cases}
            1 & \text{ if } \rho(q)\ge -\underline{\phi}^+(t)\\
            0 & \text{ otherwise}
        \end{cases}.
    \end{gather*}
    and payment function
    $$
    {p}^*(t) = \int_{q\in Q} {\pi}^*(q,t)g(q) v(q,t) \,\dd q -  \int_{t_1}^{t}P_{{\pi}^*}(x) \,\dd x.
    $$
    Above $({\pi}^*, {p}^* ) $ represents an optimal information selling mechanism for Lemma \ref{lem:optimal-case1} without requiring $\underline{\phi}(t)$ is non-decreasing.
\end{lemma}

\begin{proof}
    When the lower virtual value function is not monotone non-decreasing, the mechanism defined in Lemma \ref{lem:optimal-case1} is infeasible. We still consider the following revenue function for any feasible mechanism
    \begin{gather*}
        REV ({\pi}, {p})=\int_{q \in Q} \int_{t_1}^{t_2} \left[\underline{\phi}(t) + \rho(q)\right] f(t){\pi}(q,t)  g(q) v_1(q) \,\dd t \dd q-u(t_1).
    \end{gather*}
    The proof contains the following 2 steps:
    \begin{enumerate}
        \item Show that mechanism $(\pi^*,p^*)$ is feasible, thus the above revenue function applies;
        \item Prove that mechanism $(\pi^*,p^*)$ maximizes the revenue function.
    \end{enumerate}
    
    The first step is omitted as it is the same as in the proof of Lemma \ref{lem:optimal-case1}. We start step 2 by manipulating the revenue function. Let $\underline{H}(\cdot)$, $\underline{h}(\cdot)$, $\underline{L}(\cdot)$ and $\underline{l}(\cdot)$ be the corresponding functions defined in Definition \ref{def:ironing} when ironing the lower virtual value function $\underline{\phi}(t)$. 
    
    We can write the first term of the revenue function as follows:
    \begin{align*}
        &\int_{q \in Q} \int_{t_1}^{t_2} \left[\underline{\phi}(t) + \rho(q)\right] f(t){\pi}(q,t)  g(q) v_1(q) \,\dd t \dd q  \\
        = &\int_{q \in Q} \int_{t_1}^{t_2} \left[\underline{\phi}^+(t) + \rho(q)\right] f(t){\pi}(q,t)  g(q) v_1(q) \,\dd t \dd q \\ 
        &+ \int_{q \in Q} \int_{t_1}^{t_2} [\underline{h}(F(t))- \underline{l}(F(t))] f(t){\pi}(q,t)  g(q) v_1(q) \,\dd t \dd q.
    \end{align*}
    This is because, by definition, $\underline{\phi}^+(t)=\underline{l}(F(t))$ and $\underline{\phi}(t)=\underline{h}(F(t))$. Using integration by parts, we can simplify the second term
    \begin{align*}
        & \int_{q \in Q} \int_{t_1}^{t_2} [\underline{h}(F(t))- \underline{l}(F(t))] f(t){\pi}(q,t)  g(q) v_1(q) \,\dd t \dd q \\
        =& \int_{t_1}^{t_2} [\underline{h}(F(t))- \underline{l}(F(t))] P_{{\pi}}(t) \,\dd F(t) \\
        =& [\underline{H}(F(t))- \underline{L}(F(t))] P_{{\pi}}(t) |_{t_1}^{t_2}  - \int_{t_1}^{t_2} [\underline{H}(F(t))- \underline{L}(F(t))] \,\dd P_{{\pi}}(t) \\
    \end{align*}
    Because $\underline{L}$ is the ``convex hull'' of $\underline{H}$ on $[0,1]$, $\underline{L}(0) = \underline{H}(0)$ and $\underline{L}(1) = \underline{H}(1)$. Thus the  term $ [\underline{H}(F(t))- \underline{L}(F(t))] P_{{\pi}}(t)|_{t_1}^{t_2}$ is simply $0$, and we have 
   \begin{align}
    REV ({\pi}, {p}) 
    = &\int_{q \in Q} \int_{t_1}^{t_2} \left[\underline{\phi}^+(t) + \rho(q)\right] f(t){\pi}(q,t)  g(q) v_1(q) \,\dd t \dd q \nonumber \\ 
    & - \int_{t_1}^{t_2} [\underline{H}(F(t))- \underline{L}(F(t))] \,\dd  P_{{\pi}}(t) -u(t_1)  \label{ironing-rev}
\end{align}
    
    Now consider mechanism $({\pi}^*, {p}^*)$. $\pi^*$ maximizes the first term since ${\pi}^*(q,t) = 1, \forall q,t$ with $\rho(q)+\underline{\phi}^+(t)\ge 0$. Also, by definition, we have
    \begin{gather*}
        u(t)=\int_{q\in Q} {\pi}^*(q,t)g(q) v(q,t) \,\dd q-p(t)=\int_{t_1}^{t}P_{{\pi^*}}(x) \,\dd x.
    \end{gather*}
    Thus we have $u(t_1)=0$. 
    
    As for the second term, note that $\underline{H}(F(t))- \underline{L}(F(t))\ge 0$ by definition, and $\dd P_{\pi}(t)\ge0$ for any feasible mechanism. Thus the second term is always non-negative. However, we claim that with mechanism $({\pi}^*, {p}^*)$, this term is actually 0. The only interesting case is when $\underline{H}(F(t))> \underline{L}(F(t))\ne 0$. In this case, $t$ must lie in an ironed interval $I$. Thus $\underline{L}(z)$ is linear in the interval $I$, where $z=F(t)$. This implies that $\underline{\phi}^+(t)=\underline{l}(z)=\underline{L}'(z)$ is constant. So
    \begin{gather*}
        P_{{\pi}^*}(t)=\int_{ q \in Q}{\pi}^*(q,t)g(q)v_1(q)\,\dd q=\int_{ q :\rho(q)\ge -\underline{\phi}^+(t)}g(q)v_1(q)\,\dd q
    \end{gather*}
    is also constant in the interval $I$, which leads to $\dd P_{\widetilde{\pi}}(t)$ being 0.
    
    Therefore, mechanism $({\pi}^*, {p}^*)$ optimizes all 3 terms in Equation \eqref{ironing-rev} simultaneously, hence optimal.
   
%
%    {\bfseries Step 2.} Now we prove that mechanism $(\underline{\pi}^+,\underline{p}^+)$ is feasible. Since the ironed virtual value function $\underline{\phi}^+(t)=-\underline{\theta}_t^+$ is monotone non-decreasing, the function
%    \begin{gather*}
%        P_{\underline{\pi}^+}(t)=\int_{ q \in Q} g(q)\underline{\pi}^+(q,t)v_1(q)\,\dd q=\int_{ q:\rho(q)\ge\underline{\theta}_t^+} g(q)v_1(q)\,\dd q
%    \end{gather*}
%    is monotone non-decreasing as the integral domain expands as $t$ increases. Thus constraint \eqref{eq:signal-monotonicity} is satisfied.
%    
%    To prove that mechanism $(\underline{\pi}^+,\underline{p}^+)$ satisfies constraint \eqref{eq:buyer-utility-identify2}, observe that
%    \begin{gather*}
%        u(t)  = \int_{q\in Q} g(q) \underline{\pi}^+(q,t)v(q,t)\,\dd q - \underline{p}^+(t)=\int_{t_1}^{t}P_{\underline{\pi}^+}(x) \,\dd x.
%    \end{gather*}
%    So $u(t_1)=0$, and 
%    \begin{gather*}
%        u(t)  = u(t_1)+\int_{t_1}^{t}P_{\underline{\pi}^+}(x) \,\dd x.
%    \end{gather*}
%
%    As for constraint \eqref{eq:ir-t2}, we already have $u(t_1)=0$. For $u(t_2)$, 
%    \begin{align*}
%        u(t_2) =& \int_{t_1}^{t_2}P_{\underline{\pi}^+}(x) \,\dd x   \\
%        =& \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) \,\dd q \dd x \\
%        =&  \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) \,\dd q  \dd x + \max\left\{0, - \int_{t_1}^{t_2} \int_{q: \rho(q) \leq \underline{\theta}_x}  g(q) v_1(q) \,\dd q  \dd x \right\} \\
%        =&  \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) \,\dd q  \dd x + \max\left\{0,v(t_1)\right\} \\
%        \geq& v(t_2)
%    \end{align*}
%    
%    Similar to the proof of Lemma \ref{lem:virtual_value_order}, the interval $[0, 1]$ can be partitioned into a set of ironed intervals and non-ironed intervals. Let $z=F(t)$. If $z$ falls in a non-ironed interval, we have $\underline{H}(z) = \underline{L}(z)$. Otherwise, if $z$ falls in an ironed interval $I$, then $\underline{L}(z)$ is linear in $z$ in the interval $I$. So $\underline{\theta}_t^+=-\underline{\phi}^+(t)=-\underline{l}(z)=-\underline{L}'(z)$ is a constant. It follows that 
%    \begin{gather*}
%        P_{\underline{\pi}^+}(t)=\int_{ q \in Q} g(q)\underline{\pi}^+(q,t)v_1(q)\,\dd q=\int_{ q:\rho(q)\ge\underline{\theta}_t^+} g(q)v_1(q)\,\dd q
%    \end{gather*}
%    is also a constant. Therefore, in either case, we have that
%    \begin{gather*}
%        \int_{t_1}^{t_2} [\underline{H}(F(t))- \underline{L}(F(t))] \,\dd  P_{\underline{\pi}}(t)=0
%    \end{gather*}
%
%    
%    
%    Since $L$ is the convex hull of $H$, we know that $L$ must be flat when ever $L < H$; that is, if $L(r)<H(r)$ then $l'(r) = L''(r) = 0$. So, if $H(F(t))-L(F(t)) > 0$ then $\underline{\phi}^+(t)$ and $\bar{P}(t)$ are constant in some neighborhood of $t$. This implies that
%    \begin{equation} \label{ironing-3}
%        \int_{t_1}^{t_2} [H(F(t))- L(F(t))] d \bar{P}(t) = 0
%    \end{equation}
%    
%      
%    
%    To see that $ P_{\underline{\pi}^+}(t) = \int_{q \in Q}  \pi(q, t)  g(q) v_1(q)dq $ satisfies \eqref{eq:signal-monotonicity}, observe first that $\underline{\phi}^+(t)$ is a non-decreasing function of $t$, because $F$ and $l$ are both non-decreasing functions. Thus, $\bar{\pi}(q,t)$ is non-decreasing on $t$ and $\bar{P}(t)$ is also non-decreasing on $t$.
%    
%    
%    
%    Substituting \eqref{ironing-1} \eqref{ironing-2} \eqref{ironing-3} into \eqref{ironing-rev}, we can see $\pi(q,t)$ maximizes the revenue function, subject to \eqref{eq:signal-monotonicity}. 
%    
%    This fact, together lemma \ref{lem:optimal-case1} proves our main theorem \ref{thm:opt-scheme}.
%    
%    
%
%From equations \ref{ironing-rev} and \ref{ironing-3}, the revenue function can be written in two formats:
%\begin{align}
%    REV (\pi, p) = &\int_{q \in Q} \int_{t_1}^{t_2} [\underline{\phi}(t) + \rho(q)] f(t)\pi(q,t)  g(q) v_1(q) dt dq \label{rev-format-1} \\ 
%    = &\int_{q \in Q} \int_{t_1}^{t_2} [\underline{\phi}^+(t) + \rho(q)] f(t)\pi(q,t)  g(q) v_1(q) dt dq \label{rev-format-2}
%\end{align}
%
%Recommendation policy $\pi^*(q,t)$ maximizes revenue \ref{rev-format-1}
%\begin{gather*}
%    \pi^*(q,t)=
%    \begin{cases}
%        1 & \text{ if } \rho(q)\geq -\underline{\phi}(t)\\
%        0 & \text{ otherwise}
%    \end{cases}.
%\end{gather*}
%
%Recommendation policy $\bar{\pi}(q,t)$ maximizes revenue \ref{rev-format-2}
%\begin{gather*}
%    \bar{\pi}(q,t)=
%    \begin{cases}
%        1 & \text{ if } \rho(q)\geq -\underline{\phi}^+(t)\\
%        0 & \text{ otherwise}
%    \end{cases}.
%\end{gather*}
%
%So, the two recommendation policy $\bar{\pi}(q,t)$ and $\pi^*(q,t)$ above will both achieve the optimal revenue and have the same integral. Although $\pi^*(q,t)$ may not feasible when $\underline{\phi}(t)$ is not non-decreasing in $t$, since in that case $P(t) = \int_{\rho(q) \geq - \underline{\phi}(t)}v_1(q) g(q) dq$ is not monotone no-decreasing in $t$.
%
%Thus, we will have
%
%
%
%\begin{align} \label{revenue-equality}
%    \int_{t_1}^{t_2}\int_{q \in Q}  [\underline{\phi}(t) + \rho(q)] f(t)  \pi^*(q,t) g(q) v_1(q) dq dt =  \int_{t_1}^{t_2}\int_{q\in Q} [\underline{\phi}^+(t) + \rho(q)] \bar{\pi}(q,t) f(t) g(q) v_1(q) dq dt 
%\end{align}
%
%
%
%    
%  
%    
%    
%    
%    Now we should additionally prove that after the ironing procedure this mechanism is feasible and satisfy constraint \ref{eq:buyer-utility-identify2} \ref{eq:ir-t2} \ref{eq:non-negativity}.
%    
%    The utility identify follows from definitions and the payment p(t) we specified for this case: 
%    \begin{eqnarray*}
%        u(t)  = \int_{q\in Q} [g(q) \pi(q,t)v(q,t)] dq - p(t) =     \int_{t_1}^{t} P(x)  dx  
%    \end{eqnarray*}
%    Thus $u(t_1) =   \int_{t_1}^{t_1} P(x)  dx = 0$, which can be substituted into the above equality to obtain the utility identify.  $ u(t)= u(t_1) + \int_{t_1}^{t} P(x)  dx $
%    
%    For constraint \eqref{eq:ir-t2}, with ironing, we now have $\underline{\theta}(t) = -\underline{\phi}^+(t)$ and thus,  
%    
%    \begin{align*}
%        u(t_1) &= \int_{q \in Q} \pi(q,t_1) g(q) v(q,t_1) dq   - p(t_1) = 0 \\
%        u(t_2) &= \int_{q \in Q} \pi(q,t_2) g(q) v(q,t_2) dq   - p(t_2) = \int_{t_1}^{t_2}P(x) dx   = \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) dq  dx \\
%        &=  \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) dq  dx + \max(0, - \int_{t_1}^{t_2} \int_{q: \rho(q) \leq \underline{\theta}_x}  g(q) v_1(q) dq  dx ) \\
%        &=  \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) dq  dx + \max(0,v(t_1) ) \\
%        &\geq v(t_2)
%    \end{align*}
%    
%    Now, we are going to prove non-negativity by showing that with $\underline{\theta}(t) = -\underline{\phi}^+(t)$, we still have:  $\forall t\geq t', \; -t \leq \underline{\theta}(t) \leq \underline{\theta}(t') $.
%    
%    This still holds because suppose there are $k$ ironing intervals. Ironing i happens between $[t^i_{s},t^i_{e}]$, we have $[t^i_{s},t^i_{e}]$, we have $\forall t \in [t^i_{s},t^i_{e}], \; \underline{\phi}^+(t^i_{e}) =  \underline{\phi}^+(t) =  \underline{\phi}^+(t^i_{s})$. 
%    
%    
%    For any $t$ not in any $[t^i_{s},t^i_{e}]$ intervals, $\underline{\phi}^+(t) = \underline{\phi}(t) < t $. Thus, $-t \leq \underline{\theta}(t)$
%    
%    For any $t$ in $[t^i_{s},t^i_{e}]$ intervals, $\underline{\phi}^+(t) = l(F(t)) = l(F(t^i_{s})) = L'(F(t^i_{s})) \leq H'(F(t^i_{s})) = h(F(t^i_{s})) = \underline{\phi}(t^i_{s}) \leq t^i_{s} \leq t $. Thus, $-t \leq \underline{\theta}(t)$.
%    
%    Thus, $\forall t, \; -t \leq \underline{\theta}(t)$.
%    
%    Since  $\underline{\phi}^+(t)$ is non-decreasing in $t$ and $\underline{\theta}(t) = -\underline{\phi}^+(t)$, $\underline{\theta}(t)$ is non-increasing in $t$.
%    
%    Thus, we can conclude that $\forall t\geq t', \; -t \leq \underline{\theta}(t) \leq \underline{\theta}(t') $.
\end{proof}



\textbf{For Case 2}


We can also apply the ironing procedure defined on lemma \ref{ironing-lemma} to lemma \ref{lem:optimal-case2} with $\bar{\phi}(t) = t + \frac{F(t)}{f(t)}$, because it has similar object function.


Proof in lemma \ref{lem:optimal-case2} holds except we should additionally prove that under the ironing procedure and $\bar{\theta}(t) = -\bar{\phi}^+(t)$, we still have:  $\forall t\geq t', \; \bar{\theta}(t) \leq \bar{\theta}(t') \leq -t$

This still holds because suppose there are $k$ ironing intervals. Ironing i happens between $[t^i_{s},t^i_{e}]$, we have $\forall t \in [t^i_{s},t^i_{e}], \; \bar{\phi}^+(t^i_{e}) =  \bar{\phi}^+(t) =  \bar{\phi}^+(t^i_{s})$. 

For any $t$ not in any $[t^i_{s},t^i_{e}]$ intervals, $\bar{\phi}^+(t) = \bar{\phi}(t) \geq t $. Thus, $\bar{\theta}(t) \leq -t $

For any $t$ in $[t^i_{s},t^i_{e}]$ intervals, $\bar{\phi}^+(t) = l(F(t)) = l(F(t^i_{e})) = L'(F(t^i_{e})) \geq H'(F(t^i_{e})) = h(F(t^i_{e})) = \bar{\phi}(t^i_{e}) \geq t^i_{e} \geq t $. Thus, $\bar{\theta}(t) \leq -t $.


Since  $\bar{\phi}^+(t)$ is non-decreasing in $t$ and $\bar{\theta}(t) = -\bar{\phi}^+(t)$, $\bar{\theta}(t)$ is non-increasing in $t$.

Thus, we can conclude that $\forall t\geq t', \; \bar{\theta}(t) \leq \bar{\theta}(t') \leq -t$

So, ironing procedure will also works on  lemma \ref{lem:optimal-case2}.




% \begin{lemma} \label{lem:non-change}
% After conducting the ironing procedure, an instance will stay in its original case.
% \end{lemma}

% \begin{proof}
% Before using the ironing procedure,
% \begin{gather*}
%     V_L=\max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\underline{\phi}(t)} g(q) v_1(q) dqdx
% \end{gather*}

% After using the ironing procedure on $\underline{\phi}(t)$, the value of $v(t_1)$ will not change. 
% Now, we are going to prove the second term will not change.


% Consider the mechanism we showed in lemma \ref{lem:optimal-case1}, where the optimal information selling mechanism is the threshold mechanism $\underline{\pi}$ with threshold $\underline{\theta}_t =  -\underline{\phi}^+(t) $ for each type $t$ and it will point-wise maximize revenue function \eqref{eq:revenue-1} and give us:
% \begin{equation}
%     Rev = \int_{q \in Q}\int_{t_1}^{t_2}  [\underline{\phi}(t) + \rho(q)] f(t)  \underline{\pi}(q,t) \; dt \; g(q) v_1(q) dq
% \end{equation}
% This revenue set an upper-bound for any feasible mechanism.



% From weakly increase of optimal revenue proof in lemma \ref{ironing-lemma}, we show the new threshold mechanism $\underline{\pi}$ with threshold $\underline{\theta}_t =  -\underline{\phi}^+(t) $ for each type $t$ can reach this upper-bound, thus we have
% \begin{align*} 
%     \int_{q \in Q}\int_{t_1}^{t_2}  [\underline{\phi}(t) + \rho(q)] f(t)  \underline{\pi}(q,t) \; dt \; g(q) v_1(q) dq  =  \int_{q\in Q} \int_{t_1}^{t_2} [\underline{\phi}^+(t) + \rho(q)] \underline{\pi}^+(q,t) f(t) \; dt \; g(q) v_1(q) dq 
% \end{align*}
% since right-hand-side weakly increases the left side which is the optimal revenue, we get this equation.

% Note that the $\underline{\pi}$ in this setting may not be feasible if $\underline{\phi}(t)$ is not regular, but its revenue achieves and equals the upper-bound revenue of feasible mechanism.


% For the inner integral on $t$, we can transfer it as the following
% \begin{align*} 
% &\int_{t_1}^{t_2}  [\underline{\phi}(t) + \rho(q)] f(t)  \underline{\pi}^+(q,t) dt =\int_{t_1}^{t_2} [h(F(t)) + \rho(q)] f(t)  \underline{\pi}^+(q,t) dt \\
% & = \int_{t_1}^{t_2} [l(F(t)) + \rho(q)] f(t)  \underline{\pi}^+(q,t) dt + \int_{t_1}^{t_2} [h(F(t)) - l(F(t))] f(t)  \underline{\pi}^+(q,t) dt \\
% &= \int_{t_1}^{t_2} [l(F(t)) + \rho(q)] f(t)  \underline{\pi}^+(q,t) dt + [H(F(t))- L(F(t))] \underline{\pi}^+(q,t) \|_{t=t_1}^{t_2}   - \int_{t_1}^{t_2} [H(F(t))- L(F(t))] d \underline{\pi}^+(q,t) \\
% &= \int_{t_1}^{t_2} [l(F(t)) + \rho(q)] f(t)  \underline{\pi}^+(q,t) dt \\
% &= \int_{t_1}^{t_2} [\underline{\phi}^+(t) + \rho(q)] f(t)  \underline{\pi}^+(q,t) dt
% \end{align*}

% The second last equation holds for the same reason we discussed in ironing section.

% Thus, we have
% \begin{align*} 
% \int_{q \in Q}\int_{t_1}^{t_2}  [\underline{\phi}(t) + \rho(q)] f(t)  \underline{\pi}(q,t) \; dt \; g(q) v_1(q) dq  &=  \int_{q\in Q} \int_{t_1}^{t_2} [\underline{\phi}(t) + \rho(q)] \underline{\pi}^+(q,t) f(t) \; dt \; g(q) v_1(q) dq \\
% \int_{q \in Q}\int_{t_1}^{t_2}  \underline{\pi}(q,t)  g(q) v_1(q) dq dt  &=  \int_{q\in Q} \int_{t_1}^{t_2}  \underline{\pi}^+(q,t) g(q) v_1(q) dq dt \\
%  \int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\underline{\phi}(t)} g(q) v_1(q) dqdx &= \int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\underline{\phi}^+(t)} g(q) v_1(q) dqdx
% \end{align*}

% So, the second term of $V_L$ also stays the same. So the boundary for case 1 $V_L$ will not change.

% Ditto, $V_R$ will not change.

% Thus, the boundary to classify instances will not change.
% Since we will use the $v(t_2)$ which will not be changed by ironing of an instance to determine its case, the instance will stay in the same case after ironing procedure. 




% \end{proof}





Now, we are going to discuss how to solve the case in case 3 where $V_L < v(t_2) < V_H$ and iron it accordingly.


\begin{lemma} \label{midcase}
\item If $V_L < v(t_2) < V_H$, with combined virtual value function $\widetilde{\phi}^+(t)$ which is the ironed version of $\widetilde{\phi}(t) = C \underline{\phi}(t) + (1-C) \bar{\phi}(t) $, where $C \in (0,1) $ is a constant that satisfies $\iint_{(t,q):  \widetilde{\phi}_q(t)>= C } g(q)  v_1(q)\,dq \dd t = v(t_2)$.
The optimal mechanism is a threshold mechanism with threshold $\widetilde{\theta}(t) =-\widetilde{\phi}^+(t)$ for each type $t$.
The payment is determined by the following equation and is monotone non-decreasing in $t$ when $F(t)\leq C$ and monotone non-increasing when $F(t)>C$:
\begin{gather*}
p(t) = \int_{q \in Q} g(q) \pi(q,t)v(q,t) \,dq -  \int_{t_1}^{t} P_{\widetilde{\pi}}(x)\,dx.
\end{gather*}  
\end{lemma}


\begin{proof}
From equation \ref{eq:revenue-1} and \ref{eq:revenue-2}, we can combine the revenue function by using $C$ fraction of equation \ref{eq:revenue-1} and $(1-C)$ fraction of equation \ref{eq:revenue-2}, where $C$ is an arbitrary constant. Since equation \ref{eq:revenue-1} and \ref{eq:revenue-2} are just two different view of revenue, change $C$ will not affect the value of its combination.

Now, we have the following revenue function for mechanism with $u(t) =  u(t_1) +   \int_{t_1}^{t} P(x)  dx$ and it will not change on $C$.

\begin{align} 
REV = & C \left[\int_{q \in Q} g(q)\int_{t_1}^{t_2} f(t)\pi(q,t) v_1(q) \left(\underline{\phi}(t) + \rho(q)\right)\,\dd t \, \dd q -u(t_1) \right] \\
&+ (1-C)  \left[\int_{q \in Q} g(q) \int_{t_1}^{t_2} f(t)\pi(q,t)v_1(q) [ \bar{\phi}(t) + \rho(q)]\,\mathrm{d}t  \mathrm{d}q -u(t_2) \right] \nonumber \\
= & \int_{t_1}^{t_2}\int_{q\in Q} [C \underline{\phi}(t) + (1-C)\bar{\phi}(t) - \rho(q)] \pi(q,t) f(t) g(q) v_1(q) dq dt - C\cdot u(t_1) - (1-C)u(t_2) \label{combined-revenue}
% = & \int_{t_1}^{t_2}\int_{q\in Q} [t+\frac{F(t)}{f(t)} - \frac{C}{f(t)}] \pi(q,t) f(t) g(q) v_1(q) dq dt - C \cdot u(t_1) - (1-C)u(t_2)
% = & \int_{t_1}^{t_2}\int_{q\in Q} [C \underline{\phi}(t) + (1-C)\bar{\phi}(t) \rho(q)] \pi(q,t) f(t) g(q) v_1(q) dq dt - C\cdot \left[u(t_2) - \int_{t_1}^{t_2}P(x) dx \right] - (1-C)u(t_2)\\
% = & \int_{t_1}^{t_2}\int_{q\in Q} [C \underline{\phi}(t) + (1-C)\bar{\phi}(t) \rho(q)] \pi(q,t) f(t) g(q) v_1(q) dq dt + C\int_{t_1}^{t_2}P(x) dx  - u(t_2)\\
\end{align}




Now, our goal is to maximize revenue function:
\begin{align*}
    \text{max }  REV (\pi, p) =&\int_{t_1}^{t_2}\int_{q\in Q} [C \underline{\phi}(t) + (1-C)\bar{\phi}(t) - \rho(q)] \pi(q,t) f(t) g(q) v_1(q) dq dt - C\cdot u(t_1) - (1-C)u(t_2) \\
    \text{subject to } & P(t) \text{ is monotone non-decreasing in } t  \\
        & u(t_2) \geq v(t_2), u(t_1) \geq 0  \\ 
        & p(t) \geq 0, \forall t \in [T]. 
\end{align*}

% \begin{align*}
% p(t) &= \int_{q \in Q} g(q) \pi(q,t)v(q,t) dq -  \int_{t_1}^{t} P(x)dx \\
% & = \int_{q\in Q} g(q) \pi(q,t)v(q,t)dq  + \int_{t}^{t_2} P(x)dx- v(t_2)
% \end{align*}

Now, given an optimal feasible mechanism with recommendation policy $\pi^*(q,t)$ and payment function $p^*(t)$ which solves above optimization problem optimally, we are going to prove there is a threshold mechanism which can weakly increase this revenue. This threshold mechanism has the following definition.

This threshold mechanism has the threshold $\widetilde{\theta}(t) =-[C\underline{\phi}(t)+(1-C)\bar{\phi}(t)]$, where $C$ is a constant and satisfies:
\begin{gather*}
\int_{t_1}^{t_2} \int_{\rho(q) \geq - \widetilde{\phi}(t) } g(q) v_1(q) dq dt = v(t_2)
\end{gather*}

And the recommendation policy is:
\begin{gather*}
\pi(q,t)=
\begin{cases}
    1 & \text{ if } \rho(q)\ge -\widetilde{\phi}(t)\\
    0 & \text{ otherwise}
\end{cases}.
\end{gather*}



The payment is determined by the following equation :
\begin{gather*}
    p(t) = \int_{q \in Q} g(q) \pi(q,t)v(q,t) \,dq -  \int_{t_1}^{t} P(x)\,dx.
\end{gather*}        


Now, we are going to prove it.
The given optimal feasible mechanism with recommendation policy $\pi^*(q,t)$ gives us the following revenue.

$$
REV ^*(\pi^*, p^*) =\int_{t_1}^{t_2}\int_{q\in Q} [C \underline{\phi}(t) + (1-C)\bar{\phi}(t) - \rho(q)] \pi^*(q,t) f(t) g(q) v_1(q) dq dt - C\cdot u^*(t_1) - (1-C)u^*(t_2) 
$$
Since this function is directly got by equation \ref{combined-revenue}, changing $C$ in this function will not affect it values. So, we can set $C$ such that
$$    \int_{t_1}^{t_2} \int_{\rho(q) \geq - \widetilde{\phi}(t)} g(q) v_1(q) dq dt = v(t_2) $$
without changing $REV ^*(\pi^*, p^*)$.

There exists a constant $C \in (0,1)$ which satisfies the above condition, because
from the condition of case 3 where $V_L < v(t_2) < V_H$, we have 
\begin{gather*}
\max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) \,dqdx < v(t_2) < \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) \,dqdx
\end{gather*}

With the equivalence \ref{remark:case_1_condition_eq}, 
\begin{align*}
    &   v(t_2) \geq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx  
    \Longleftrightarrow  v(t_1)   \geq  -   \int_{t_1}^{t_2} \int_{q: \rho(q) \leq \bar{\theta}_x}  g(q) v_1(q) dq  dx    
\end{align*}

by contrapositive, we can get the following equivalence,
\begin{align}
    v(t_2) <\max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx  
    \Longleftrightarrow  v(t_1)   <  -   \int_{t_1}^{t_2} \int_{q: \rho(q) \leq \bar{\theta}_x}  g(q) v_1(q) dq  dx      \label{case3-v1-v2-2}
\end{align}

Since case 3's condition includes the antecedent of equivalence \ref{case3-v1-v2-2} and  $\forall q \;  g(q)v_1(q) \geq 0 $, we get 
\begin{align*}
v(t_1)   <  -   \int_{t_1}^{t_2} \int_{q: \rho(q) \leq \bar{\theta}_x}  g(q) v_1(q) dq  dx \leq 0
\end{align*}

Now, because $\bar{\theta}_x = -\underline{\phi}(t) $, $\underline{\theta}_x = -\bar{\phi}(t) $ and $v(t_1) < 0 $, case 3's condition can be written as,
\begin{gather*}
\int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\underline{\phi}(t)} g(q) v_1(q) \,dqdx < v(t_2) < \int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\bar{\phi}(t)} g(q) v_1(q) \,dqdx
\end{gather*}

When C = 0, we have
\begin{equation} \label{C_0}
int_{t_1}^{t_2} \int_{\rho(q) \geq - C \underline{\phi}(t) - (1-C) \bar{\phi}(t)  } g(q) v_1(q) dq dt = \int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\underline{\phi}(t)} g(q) v_1(q) \,dqdx < v(t_2)
\end{equation}

When C = 1, we have
\begin{equation} \label{C_1}
\int_{t_1}^{t_2} \int_{\rho(q) \geq - C \underline{\phi}(t) - (1-C) \bar{\phi}(t)  } g(q) v_1(q) dq dt = \int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\bar{\phi}(t)} g(q) v_1(q) \,dqdx > v(t_2)
\end{equation}


Now, we are going to show this function is continuous on $C \in (0,1)$. We can write 
\begin{align*}
     \int_{t_1}^{t_2} \int_{q: \rho(q) \geq -\widetilde{\phi}(t)} g(q) v_1(q) \,\dd q\dd t &= \int_{t_1}^{t_2} \int_{\rho(q) \geq - C \underline{\phi}(t) - (1-C) \bar{\phi}(t)  } g(q) v_1(q) dq dt \\
     &= \int_{t_1}^{t_2} \int_{\rho(q) \geq - (t+\frac{F(t)}{f(t)}+\frac{C}{f(t)}) } g(q) v_1(q) dq dt \\
     &= Y(C)
\end{align*}    

\sz{see note lemma 4.11 how to set C and D}

Now, we can see that with $\pi(q,t)$ and $p(t)$ in the threshold mechanism. We have 
\begin{align}
u(t_1) &= \int_{q \in Q}   g(q) \pi(q,t_1)v(q,t_1) dq -p(t_1) = \int_{t_1}^{t_1} P(x) = 0  \label{case3-ut1}\\
u(t_2) &= \int_{q \in Q}   g(q) \pi(q,t_2)v(q,t_2) dq -p(t_2) = \int_{t_1}^{t_1} P(x) = \int_{t_1}^{t_2} \int_{\widetilde{\phi}_q(t)>= C } g(q) v_1(q) dq dt = v(t_2)  \label{case3-ut2}   
\end{align}

Since to satisfy IR constraint \ref{eq:ir-t2}, we must have $ u(t_2) \geq v(t_2), u(t_1) \geq 0$ for any feasible mechanism. Thus,
\begin{align}
u(t_1) &\leq u^*(t_1) \label{case3-opt1} \\
u(t_2) &\leq u^*(t_2) \label{case3-opt2}  
\end{align}

Since the threshold policy $\pi(q,t) =  1 \geq \pi^*(q,t) $ whenever $[C \underline{\phi}(t) + (1-C)\bar{\phi}(t) - \rho(q)]\geq 0$ and  $\pi(q,t) =  0 \leq \pi^*(q,t) $ whenever $[C \underline{\phi}(t) + (1-C)\bar{\phi}(t) - \rho(q)] < 0$, and $f(t)g(q)v_1(q) \geq 0$, we 
have 
\begin{align}
\int_{t_1}^{t_2}\int_{q\in Q} [C \underline{\phi}(t) + (1-C)\bar{\phi}(t) - \rho(q)] \pi(q,t) f(t) g(q) v_1(q) dq dt \geq \nonumber \\ \int_{t_1}^{t_2}\int_{q\in Q} [C \underline{\phi}(t) + (1-C)\bar{\phi}(t) - \rho(q)] \pi^*(q,t) f(t) g(q) v_1(q) dq dt \label{case3-opt3} 
\end{align}

Based on inequality \ref{case3-opt1} \ref{case3-opt2} \ref{case3-opt3}, we have

\begin{align*}
REV (\pi, p) &=\int_{t_1}^{t_2}\int_{q\in Q} [C \underline{\phi}(t) + (1-C)\bar{\phi}(t) - \rho(q)] \pi(q,t) f(t) g(q) v_1(q) dq dt - C\cdot u(t_1) - (1-C)u(t_2) \\
& \geq\int_{t_1}^{t_2}\int_{q\in Q} [C \underline{\phi}(t) + (1-C)\bar{\phi}(t) - \rho(q)] \pi^*(q,t) f(t) g(q) v_1(q) dq dt - C\cdot u^*(t_1) - (1-C)u^*(t_2) \\
& = REV ^*(\pi^*, p^*) 
\end{align*}

So, threshold mechanism $(\pi(q,t),p(t))$ is an optimal mechanism.

Now, applying the ironing procedure on
$\widetilde{\phi}(t) = C \underline{\phi}(t) + (1-C) \bar{\phi}(t)  = t+\frac{F(t)-C}{f(t)}$.
We will get $\widetilde{\phi}^+(t)$ which is non-decreasing on t. 
For the same reason we proved in the ironing section, the recommendation policy that is
\begin{gather*}
\pi(q,t)=
\begin{cases}
    1 & \text{ if } \rho(q)\ge -\widetilde{\phi}^+(t)\\
    0 & \text{ otherwise}
\end{cases}.
\end{gather*}

with the payment function
\begin{gather*}
    p(t) = \int_{q \in Q} g(q) \pi(q,t)v(q,t) \,dq -  \int_{t_1}^{t} P(x)\,dx.
\end{gather*}        
can weakly increase the revenue.
So, now the optimal mechanism is this new $((\pi(q,t),p(t))$ defined with $\widetilde{\phi}^+(t)$. 

\textbf{Feasibility:}

Now, we are going to prove this mechanism $((\pi(q,t),p(t))$ is also feasible.




Since $\widetilde{\phi}^+(t) = C \underline{\phi}(t) + (1-C) \bar{\phi}(t) $ is non-decreasing in t, larger $t$ will lets $P(t) = \int_{t_1}^{t_2} \int_{\rho(q) >=  - \widetilde{\phi}^+(t) } g(q) v_1(q) dq dt$ includes more $g(q)v_1(q)$ term which are positive for any q. So we have $P(x)$ is non-decreasing. Thus, constraint \ref{eq:signal-monotonicity} is satisfied.

Since $u(t_1) = 0$,
\begin{align*}
u(t)= \int_{q \in Q}  \left[ g(q) \pi(q,t)v(q,t) \right] dq -p(t) = \int_{t_1}^{t} P(x)dx = u(t_1) + \int_{t_1}^{t} P(x)dx
\end{align*}

Thus, constraint \ref{eq:buyer-utility-identify2} is satisfied.

\begin{align*}
u(t_1) &= \int_{q \in Q}   g(q) \pi(q,t_1)v(q,t_1) dq -p(t_1) = \int_{t_1}^{t_1} P(x) = 0  \\
u(t_2) &= \int_{q \in Q}   g(q) \pi(q,t_2)v(q,t_2) dq -p(t_2) = \int_{t_1}^{t_1} P(x) = \int_{t_1}^{t_2} \int_{\rho(q) >= -\widetilde{\phi}^+(t) } g(q) v_1(q) dq dt = v(t_2)  
\end{align*}

Thus, constraint \ref{eq:ir-t2} is satisfied.

% Now, we are going to prove payment non-negativity by showing that with $\widetilde{\theta}(t) = -\widetilde{\phi}^+(t)$, we have:  $\forall t\geq t' \text{ where } F(t)\leq C, F(t')\leq C, \; \text{we have }-t \leq \widetilde{\theta}(t) \leq \widetilde{\theta}(t') $.

% This holds because suppose there are $k$ ironing intervals. Ironing i happens between $[t^i_{s},t^i_{e}]$, we have $[t^i_{s},t^i_{e}]$, we have $\forall t \in [t^i_{s},t^i_{e}], \; \widetilde{\phi}^+(t^i_{s}) =  \widetilde{\phi}^+(t) =  \widetilde{\phi}^+(t^i_{e})$. 


% For any $t$ not in any $[t^i_{s},t^i_{e}]$ intervals and $F(t)\leq C$, $\widetilde{\phi}^+(t) = \widetilde{\phi}(t) = t+\frac{F(t)-C}{f(t)} \leq t $. Thus, $-t \leq \widetilde{\theta}(t)$

% For any $t$ in $[t^i_{s},t^i_{e}]$ intervals and $F(t)\leq C$, $\widetilde{\phi}^+(t) = l(F(t)) = l(F(t^i_{s})) = L'(F(t^i_{s})) \leq H'(F(t^i_{s})) = h(F(t^i_{s})) = \widetilde{\phi}(t^i_{s}) \leq t^i_{s}+\frac{F(t^i_{s})-C}{f(t^i_{s})} \leq t $. Thus, $-t \leq \widetilde{\theta}(t)$.

% Thus, $\forall t, F(t)\leq C, \text{ we have } -t \leq \widetilde{\theta}(t)$.

% Since  $\widetilde{\phi}^+(t)$ is non-decreasing in $t$ and $\widetilde{\theta}(t) = -\widetilde{\phi}^+(t)$, $\widetilde{\theta}(t)$ is non-increasing in $t$.

% Thus, we can conclude that $\forall t\geq t' \text{ where } F(t)\leq C, F(t')\leq C, \; \text{we have }-t \leq \widetilde{\theta}(t) \leq \widetilde{\theta}(t') $.

% \vspace{1cm}
% --------------------------case 2--------------------

% Now, we are going to prove with $\widetilde{\theta}(t) = -\widetilde{\phi}^+(t)$, we have: $\forall t\geq t' \text{ where } F(t)> C, F(t')>C, \; \text{we have } \widetilde{\theta}(t) \leq \widetilde{\theta}(t') \leq -t$

% This holds because suppose there are $k$ ironing intervals. Ironing i happens between $[t^i_{s},t^i_{e}]$, we have $\forall t \in [t^i_{s},t^i_{e}], \; \widetilde{\phi}^+(t^i_{s}) =  \widetilde{\phi}^+(t) =  \widetilde{\phi}^+(t^i_{e})$. 

% For any $t$ not in any $[t^i_{s},t^i_{e}]$ intervals and $F(t)> C$, $\widetilde{\phi}^+(t) = \widetilde{\phi}(t) = t+\frac{F(t)-C}{f(t)} \geq t $. Thus, $\widetilde{\theta}(t) \leq -t $

% For any $t$ in $[t^i_{s},t^i_{e}]$ intervals and $F(t)> C$, $\widetilde{\phi}^+(t) = l(F(t)) = l(F(t^i_{e})) = L'(F(t^i_{e})) \geq H'(F(t^i_{e})) = h(F(t^i_{e})) = \widetilde{\phi}(t^i_{e}) \geq t^i_{e}+\frac{F(t^i_{e})-C}{f(t^i_{e})}  \geq t $. Thus, $\widetilde{\theta}(t) \leq -t $.


% Since  $\widetilde{\phi}^+(t)$ is non-decreasing in $t$ and $\widetilde{\theta}(t) = -\widetilde{\phi}^+(t)$, $\widetilde{\theta}(t)$ is non-increasing in $t$.

% Thus, we can conclude that $\forall t\geq t' \text{ where } F(t)> C, F(t')>C, \; \text{we have } \widetilde{\theta}(t) \leq \widetilde{\theta}(t') \leq -t$


Now, we are going to prove payment non-negativity.

First we are going to show $\forall t, F(t)\leq C, \text{ we have } \widetilde{\phi}^+(t) \leq t $.
This holds because suppose there are $k$ ironing intervals. Ironing i happens between $[t^i_{s},t^i_{e}]$, we have $[t^i_{s},t^i_{e}]$, we have $\forall t \in [t^i_{s},t^i_{e}], \; \widetilde{\phi}^+(t^i_{s}) =  \widetilde{\phi}^+(t) =  \widetilde{\phi}^+(t^i_{e})$. 


For any $t$ not in any $[t^i_{s},t^i_{e}]$ intervals and $F(t)\leq C$, $\widetilde{\phi}^+(t) = \widetilde{\phi}(t) = t+\frac{F(t)-C}{f(t)} \leq t $. 

For any $t$ in $[t^i_{s},t^i_{e}]$ intervals and $F(t)\leq C$, $\widetilde{\phi}^+(t) = l(F(t)) = l(F(t^i_{s})) = L'(F(t^i_{s})) \leq H'(F(t^i_{s})) = h(F(t^i_{s})) = \widetilde{\phi}(t^i_{s}) \leq t^i_{s}+\frac{F(t^i_{s})-C}{f(t^i_{s})} \leq t^i_{s} \leq t $. 

Thus, $\forall t, F(t)\leq C, \text{ we have } \widetilde{\phi}^+(t) \leq t $.


Now, we are going to prove $\forall t, F(t) > C, \text{ we have } \widetilde{\phi}^+(t) \geq t $.

This holds because suppose there are $k$ ironing intervals. Ironing i happens between $[t^i_{s},t^i_{e}]$, we have $\forall t \in [t^i_{s},t^i_{e}], \; \widetilde{\phi}^+(t^i_{s}) =  \widetilde{\phi}^+(t) =  \widetilde{\phi}^+(t^i_{e})$. 

For any $t$ not in any $[t^i_{s},t^i_{e}]$ intervals and $F(t)> C$, $\widetilde{\phi}^+(t) = \widetilde{\phi}(t) = t+\frac{F(t)-C}{f(t)} \geq t $. 

For any $t$ in $[t^i_{s},t^i_{e}]$ intervals and $F(t)> C$, $\widetilde{\phi}^+(t) = l(F(t)) = l(F(t^i_{e})) = L'(F(t^i_{e})) \geq H'(F(t^i_{e})) = h(F(t^i_{e})) = \widetilde{\phi}(t^i_{e}) \geq t^i_{e}+\frac{F(t^i_{e})-C}{f(t^i_{e})} \geq t^i_{e}  \geq t $. 


Thus, $\forall t, F(t) > C, \text{ we have } \widetilde{\phi}^+(t) \geq t $.

Now, we can conclude $\forall t, F(t)\leq C, \text{ we have } \widetilde{\phi}^+(t) \leq t $ 
and  
$\forall t, F(t) > C, \text{ we have } \widetilde{\phi}^+(t) \geq t $.



\begin{align*}
    p(t_1) &= -u(t_1) + \int_{\rho(q) \geq -\widetilde{\phi}^+(t) } g(q) v(q,t_1) dq \\ 
    &=  \int_{\rho(q) \geq -\widetilde{\phi}^+(t) } g(q) v_1(q)[t_1+\rho(q)] dq \\
    &\geq  \int_{\rho(q) \geq -\widetilde{\phi}^+(t) } g(q) v_1(q)[t_1 - \widetilde{\phi}^+(t_1)] dq \\
    &\geq  \int_{\rho(q) \geq -\widetilde{\phi}^+(t) } g(q) v_1(q)[t_1 - t_1] dq \\
    &= 0
\end{align*}


where the last inequality is because  $\forall t, F(t)\leq C, \text{ we have } \widetilde{\phi}^+(t) \leq t $.

Similarly, utilizing $u(t_2) = v(t_2) = \int_{q \in Q} g(q) v_1(q)[t_2 + \rho(q)]$, we have
\begin{align*}
    p(t_2) &= -u(t_2)  + \int_{\rho(q) \geq -\widetilde{\phi}^+(t) } g(q) v(q,t_2) dq \\ 
    &=  - \int_{q \in Q} g(q) v_1(q)[t_2 + \rho(q)] + \int_{\rho(q) \geq -\widetilde{\phi}^+(t) } g(q) v_1(q)[t_2+\rho(q)] dq \\
    &=  -   \int_{\rho(q) \leq -\widetilde{\phi}^+(t) } g(q) v_1(q)[t_2+\rho(q)] dq \\
    &\geq   -   \int_{\rho(q) \leq -\widetilde{\phi}^+(t) } g(q) v_1(q)[t_2-\widetilde{\phi}^+(t_2)] dq \\
    &\geq   -   \int_{\rho(q) \leq -\widetilde{\phi}^+(t) } g(q) v_1(q)[t_2-t_2)] dq \\
    &= 0
\end{align*}
where the last inequality is because $\forall t, F(t) > C, \text{ we have } \widetilde{\phi}^+(t) \geq t $.




Since
\begin{align*}
    p(t)=&\int_{q \in Q} g(q) \pi(q,t)v(q,t) \,\mathrm{d}q -\int_{t_1}^{t} P(x)  \,\mathrm{d}x\\
    =&\int_{q:\rho(q)\ge -\widetilde{\phi}^+(t)}g(q)v(q, t)\,\mathrm{d}q-\int_{t_1}^t \int_{q \in Q} g(q) \pi(q,x) v_1(q)\,\mathrm{d}q\mathrm{d}x\\
    =&\int_{q:\rho(q)\ge -\widetilde{\phi}^+(t)}g(q)v(q, t)\,\mathrm{d}q-\int_{t_1}^t \int_{q:\rho(q)\ge -\widetilde{\phi}^+(x)} g(q) v_1(q)\,\mathrm{d}q\mathrm{d}x
\end{align*}

the differential of $p(t)$ is

\sz{change sum to integral}
\begin{align*}
    \mathrm{d}p(t)=&\left[\int_{q:\rho(q)\ge -\widetilde{\phi}^+(t)}g(q)\frac{\partial v(q,t)}{\partial t}\,\mathrm{d}q\right]\mathrm{d}t+\left[\frac{\mathrm{d}}{\mathrm{d}\widetilde{\phi}^+(t)}\int_{q:\rho(q)\ge -\widetilde{\phi}^+(t)}g(q)v(q, t)\,\mathrm{d}q\right]\mathrm{d}\widetilde{\phi}^+(t)\\
    &-\left[\int_{q:\rho(q)\ge -\widetilde{\phi}^+(t)} g(q) v_1(q)\,\mathrm{d}q\right]\mathrm{d}t\\
    =&\left[\frac{\mathrm{d}}{\mathrm{d}\widetilde{\phi}^+(t)}\int_{q:\rho(q)\ge -\widetilde{\phi}^+(t)}g(q)v(q, t)\,\mathrm{d}q\right]\mathrm{d}\widetilde{\phi}^+(t)\\
 %   =&\left[\ \mathrm{d} \int_{q:\rho(q)\ge -\widetilde{\phi}^+(t)}g(q)v_1(q)[t+\rho(q)]\,\mathrm{d}q\right] \\
    =&  \int_{q: -\widetilde{\phi}^+(t) + \mathrm{d}\widetilde{\phi}^+(t)   \geq \rho(q)\ge -\widetilde{\phi}^+(t)}g(q)v_1(q)[t+\rho(q)]\,\mathrm{d}q   \\ 
      \geq &  \int_{q: -\widetilde{\phi}^+(t) + \mathrm{d}\widetilde{\phi}^+(t)   \geq \rho(q)\ge -\widetilde{\phi}^+(t)}g(q)v_1(q)[t   -\widetilde{\phi}^+(t) ]\,\mathrm{d}q   \\ 
    \geq & 0 \\  
  %  =&\left[\sum_{q:\rho(q)=-\widetilde{\phi}^+(t)}g(q)v(q,t)\right]\mathrm{d}\widetilde{\phi}^+(t)\\
 %   =&\left[\sum_{q:\rho(q)=-\widetilde{\phi}^+(t)}g(q) v_1(q)[t - \widetilde{\phi}^+(t)] \right]\mathrm{d}\widetilde{\phi}^+(t) 
\end{align*}
where the last inequality is due to our choice of $t$ with $ F(t)\leq C$ so that $ \widetilde{\phi}^+(t) \leq t $.  
% \begin{align*}
% \mathrm{d}p(t)
% =&\left[\sum_{q:\rho(q)=-\widetilde{\phi}^+(t)}g(q) v_1(q)[t - \widetilde{\phi}^+(t)] \right]\mathrm{d}\widetilde{\phi}^+(t) \\
% \geq&\left[\sum_{q:\rho(q)=-\widetilde{\phi}^+(t)}g(q) v_1(q)[t - t] \right]\mathrm{d}\widetilde{\phi}^+(t) \\
% = 0
% \end{align*}



Therefore, when $F(t)\le C$, $dp(t)$ is a non-negative. $\forall t, \; F(t) \leq C$, $p(t)$ is a non-decreasing function of $t$ .

$\forall t, F(t) > C, \text{ we have } \widetilde{\phi}^+(t) \geq t $, Thus,
\begin{align*}
\mathrm{d}p(t)
=&\left[\sum_{q:\rho(q)=-\widetilde{\phi}^+(t)}g(q) v_1(q)[t - \widetilde{\phi}^+(t)] \right]\mathrm{d}\widetilde{\phi}^+(t) \\
\leq&\left[\sum_{q:\rho(q)=-\widetilde{\phi}^+(t)}g(q) v_1(q)[t - t] \right]\mathrm{d}\widetilde{\phi}^+(t) \\
= 0
\end{align*}


Therefore, when $F(t) > C$, $dp(t)$ is a non-positive. $\forall t, \; F(t) \leq C$, $p(t)$ is a non-increasing function of $t$. 

We also have $p(t_1)\geq 0$ and $p(t_2)\geq 0$. Thus, $p(t)$ is non-negative and non-decreasing $\forall t, \; F(t) \leq C$ and non-negative and non-increasing $\forall t, \; F(t) \leq C$.

Thus, constraint \ref{eq:non-negativity} is satisfied.
Now, all constraints in lemma \ref{lem:feasible-M} are satisfied. We proved this mechanism is optimal and feasible.


$\dd x  \mathrm{d} \mathrm{d}x$ 

\end{proof}


==> monotonicity.tex <==
\begin{lemma}
\label{lem:virtual_value_order}
Define ${\phi}_c(t) = c\underline{\phi}(t) + (1-c) \bar{\phi}(t)$. Then we have for any $0 \leq c < c' \leq 1$, ${\phi}_c^+ (t) \geq {\phi}_{c'}^+(t)$ for any $t$. Moreover,  ${\phi}_1^+ (t) = \underline{\phi}^{+}(t)< t< \bar{\phi}^{+}(t) ={\phi}_0^+ (t) , \forall t \in (t_1, t_2)$.
\end{lemma}

 

\begin{proof}
 We will instead consider the function $\phi$ in a new variable space $z = F(t) \in [0,1]$, as opposed to the original space $t$. Therefore, let $l_c(z) = \phi_c^+(F^{-1}(z))$ and $h_c(z) = \phi_c(F^{-1}(z))$. Recall that the ironing procedure satisfies $L_c(z) =  \int_{0}^z l_c(r) \, \dd r$   is the convex hull of $H_c(z) =  \int_{0}^z h_c(r) \, \dd r$. 
 
Note that during the ironing of function $H_c(z)$, it divided the compact variable space $[0,1]$ into a finite number of small intervals with breaking points $0=z_0, z_1, \cdots, z_k = 1$ on which for any interval $[z_i, z_{i+1}]$: (1) either $H_c(z) = L_c(z)$ for any $z \in [z_i, z_{i+1}]$; (2) $l_c(z)$ is a constant and $H_c(z) \geq L_c(z)$ for any $z \in [z_i, z_{i+1}]$. In later case, we will call $[z_i, z_{i+1}]$ an \emph{ironing interval} and say $H_c(z)$ is at \emph{ironing state} in this interval.  We call $z_i$ the \emph{ironing starting point} and  $z_{i+1}$ the \emph{ironing ending point}. Similarly, in former case, we call $[z_i, z_{i+1}]$ an \emph{un-ironing interval} and say $H_c(z)$ is at \emph{un-ironing state} in this interval. Note that in this case, $z_i$ will be an ironing ending point and $z_{i+1} $ will be an ironing starting point. In fact, in the sequence $0=z_0, z_1, \cdots, z_k = 1$, ironing starting and ending points show up alternately.  The following are a few useful properties that will be needed.
\begin{enumerate}
    \item If $z \not = 0, 1$ is an ironing starting or ending point, then $h_c(z) = l_c(z)$ and $H_c(z) = L_c(z)$. 
    \item if $[z_i, z_{i+1}]$ is an ironing interval for $H_c(z)$, then we have $l_c(z) = \frac{H_c(z_{i+1}) - H_c(z_i)}{z_{i+1} - z_i}$ for any  $z \in [z_i, z_{i+1}]$ 
    \item For any $z \in [0,1]$  we have  $h_c(z) = t+\frac{F(t)}{f(t)}-\frac{c}{f(t)}  \geq  t+\frac{F(t)}{f(t)}-\frac{c'}{f(t)} = h_{c'}(z)$  where $t = F^{-1}(z)$.
    \item Due to property (3) above,  for any $z$  we have  $H_c(\bar{z}) - H_c(z) \geq    H_{c'}(\bar{z}) - H_{c'}(z)$ for any $\bar{z} > z$. Moreover,  $H_c(0)  =    H_{c'}(0) = 0$. 
\end{enumerate}

 
Similarly, we can also have a sequence of ironing starting and ending points for the function $H_{c'}(z)$. Let us merge all the ironing starting and ending points of $H_c(z)$ and $H_{c'}(z)$ together, and list them in order as $0 = z_0, z_1, \cdots, z_k = 1$. Notably, within any interval $[z_i, z_{i+1}]$, both function $H_c(z)$ and $H_{c'}(z)$ can only have a single state, either ironing state or un-ironing state. 

We first prove $l_c(0) \geq l_{c'}(0)$. This follows a case analysis about whether $0$ is an ironing ending or starting point for $H_c$.  
\begin{itemize}
    \item If $0$ is an ironing ending point for both $H_c, H_{c'}$, meaning both functions are not on ironing state at $0$ and its neighborhood, we know $l_c(0) = h_c(0) \geq h_{c'}(0) =   l_{c'}(0)$, as desired.  
    \item If $0$ is an ironing ending point only for  $H_c$ but an ironing starting point for $H_{c'}$, this means  $H_c$  is  on un-ironing state at $0$ and its neighborhood whereas $H_{c'}$ is on ironing state. Then we have  we know $l_c(0) = h_c(0) \geq h_{c'}(0)   \geq l_{c'}(0)$, as desired. 
    \item If $0$ is an ironing starting point for $H_c$ (it does not matter it is an ironing ending or starting point for $ H_{c'}$), this means $H_c$     is  on ironing state at $0$ and its neighborhood. Let $\bar{z} \geq z_1$ be the immediate next ironing ending point for $H_c$. Suppose, for the sake of contradiction, that $l_c(0) < l_{c'}(0)$. We thus have 
    \begin{align*}
    H_c(\bar{z}) - H_c(0) &= l_c(0) \cdot (\bar{z} - 0)  & \mbox{by Property (2) above } \\
    & <  l_{c'}(0) \cdot (\bar{z} - 0)  & \mbox{by assumption} \\ 
    & \leq  L_{c'}(\bar{z}) - L_{c'}(0)   & \mbox{by convexity of $L_{c'}$}  \\
     & \leq  H_{c'}(\bar{z}) - H_{c'}(0)   & \mbox{$L_{c'}(0) = H_{c'}(0), L_{c'}(\bar{z}) \leq  H_{c'}(\bar{z})$}  
    \end{align*} 
     This contradicts Property (4) above.  
    Therefore, we must  $l_c(0)   \geq    l_{c'}(0)$, as desired.  
\end{itemize}    
 
 
Next, we will prove that for any $i=0,\cdots, k-1$ and any interval   $[z_i, z_{i+1}]$ ---  more conveniently denoted as $[a,b]$ with interval lower bound $a$ and upper bound $b$ ---  we will have $l_c(z) \geq l_{c'}(z)$ for any $z \in [a,b]$. 

Our proof uses an induction argument over the intervals indexed by $i$. Specifically, suppose we already have $l_c(a) \geq l_{c'}(a)$, we will show $l_c(z) \geq l_{c'}(z)$ for any $z \in [a,b]$. This, together with the base case for $a=0$ as proved above, will prove the monotonicity of $l_c(z)$ on $c$.  

The proof  uses a case analysis about whether then ending point $b$ of the interval $[a,b]$ is an ironing starting point or ending point for $H_c$ or for $H_{c'}$. Note that there will be four cases here. This is because we do not know whether $b$ is an ironing point on $H_c$ or on $H_{c'}$ and thus have to consider both possibilities. Here, we will use the crucial property that both  $H_c$ and $H_{c'}$ will have the same state, i.e., ironing or un-ironing state, within $[a,b]$ due to our choice of $a,b$. 
\begin{itemize}
    \item If  $b$ is an ironing ending point for function $H_{c'}$, we have for any $z \in [a,b]$ 
      \begin{align*}
     l_c(z) & \geq l_c(a)  & \mbox{by convexity of $L_c$ } \\
    & \geq   l_{c'}(a)  & \mbox{by induction hypothesis} \\ 
    &  =  l_{c'}( z)    & \mbox{$H_{c'}$ is at ironing state in $[a,b]$}
    \end{align*} 
    
    \item If  $b$ is an ironing starting point for function $H_{c'}$,  this means  $H_{c'}$ is at un-ironing state within $[a,b]$. If $H_c$ is also at un-ironing state within $[a,b]$, then we have $l_c(z) = h_c(z) \geq h_{c'}(z) = l_{c'}(z)$ as desired. Thus, we now consider the case that $H_c$ is at ironing state within $[a,b]$. Let $\bar{z} \geq b$ be the immediate next ironing ending point for $H_c$. Suppose, for the sake of contradiction, that $l_c(z) < l_{c'}(z)$ for some $z\in [a,b]$. Since $H_c$ is at ironing state within $[a,\bar{z}]$, we know that $l_c(r) = l_c(z)  < l_{c'}(z) \leq l_{c'}(r)$ for any $r \in [b, \bar{z}]$ since $l_{c'}(z)$ is monotone non-decreasing in $z$. Therefore, we have  
    \begin{align*}
    H_c(\bar{z}) - H_c(b) & \leq  L_c(\bar{z}) - L_c(b) & \mbox{$L_{c}(\bar{z}) = H_{c}(\bar{z}), L_{c}(b) \leq  H_{c}(b)$} \\ 
    & \leq l_c(b) \cdot (\bar{z} - b)  & \mbox{$H_c$ is at ironing state in $[a,\bar{z}]$} \\
    & <  l_{c'}(b) \cdot (\bar{z} - b)  & \mbox{by assumption} \\ 
    & \leq  L_{c'}(\bar{z}) - L_{c'}(b)   & \mbox{by convexity of $L_{c'}$}  \\
     & \leq  H_{c'}(\bar{z}) - H_{c'}(b)   & \mbox{$b$ is an ironing starting point for  $H_{c'}$}  
    \end{align*} 
      This contradicts Property (4) above.  
    Therefore, we must  $l_c(z)   \geq    l_{c'}(z)$ for all $z \in [a,b]$, as desired. Note that one corner case for this situation is when $\bar{z}$ happens to equal $b$, i.e., $b$ is both the ironing starting point of $H_{c'}$ and ironing ending point of $H_c$. Our argument above does not apply to this corner situation since the strict ``$<$'' above becomes ``$=$''. However, this corner case can  be proved via a simpler argument: $\forall z\in[a,b]$, $l_c(z) = l_c(b) = h_c(b) \geq h_{c'}(b) \geq h_{c'}(z) = l_{c'}(z)$ where the second equality is due to the fact that $b$ is an ironing ending point of $H_c$ and the last equality is due to the fact that  $H_{c'}$ is at un-ironing state within $[a,b]$. 
    
    \item If  $b$ is an ironing starting point for function $H_{c}$,  this means  $H_{c}$ is at un-ironing state within $[a,b]$. If $H_{c'}$ is also at un-ironing state within $[a,b]$, then we have $l_c(z) = h_c(z) \geq h_{c'}(z) = l_{c'}(z)$ as desired. If $H_{c'}$ is   at ironing state within $[a,b]$, then we have $l_c(z)   \geq l_c(a) \geq \ l_{c'}(a) = l_{c'}(z)$ as desired. 
    
    \item Finally, if   $b$ is an ironing ending point for function $H_{c}$,  this means  $H_{c}$ is at  ironing state within $[a,b]$. If $H_{c'}$ is also at ironing state within $[a,b]$, then we have  $l_c(z)   = l_c(a) \geq l_{c'}(a) = l_{c'}(z)$ as desired. If $H_{c'}$ is   at the un-ironing state within $[a,b]$, then we have $l_c(z) = l_c(b) = h_c(b) \geq h_{c'}(b) \geq  l_{c'}(z)$ where: (1) the first equality is because $H_c$ is at ironing state within $[a,b]$; (2) second equality is because $b$ is an ironing ending point for $H_c$ and the last inequality is because $H_{c'}$ is at un-ironing state within $[a,b]$ and thus $h_{c'}(z) = l_{c'}(z)$ is monotone non-decreasing in $z$.  
\end{itemize}
 \end{proof}

 



% % \sz{Previous ideas in here are commented out.}
% \begin{proof}
% \sz{There are three possible ways. The first way is the following.}


% \begin{align*}
% {\phi}_c(t) = c\underline{\phi}(t) + (1-c) \bar{\phi}(t) = t+\frac{F(t)}{f(t)}-\frac{c}{f(t)}
% \end{align*}

% Suppose $\epsilon$ is an arbitrary small number and $\epsilon > 0$. Then we are going to show $\forall t \in (0,1)$, we have ${\phi}_c^+ (t) \geq {\phi}_{c+\epsilon}^+(t)$.

% For any $t$, we use the term "ironed" to describe ${\phi}_c^+ (t) \neq {\phi}_c(t)$ at $t$ and "not ironed" to describe ${\phi}_c^+ (t) = {\phi}_c(t)$ at $t$.

% Function ${\phi}_c^+ (t)$ may have many "ironed" intervals. If function ${\phi}_c^+ (t)$ at $t$ is ironed, suppose $t$ is in $i$th ironed interval of function ${\phi}_c^+ (t)$, define $t_c^{s_i}$ as the start point of this ironed interval and $t_c^{e_i}$ as the end point of this ironed interval. We have $t \in [t_c^{s_i},t_c^{e_i}]$ and ${\phi}_c^+ (t_c^{s_i})  = {\phi}_c^+ (t) = {\phi}_c^+ (t_c^{e_i}) $.

% \textbf{Important properties}\\
% 1. ${\phi}_c^+ (t_c^{s_i})  = {\phi}_c^+ (t) = {\phi}_c^+ (t_c^{e_i}) $ \blue{ironed} \\
% 2. ${\phi}_c^+ (t_c^{s_i})  = {\phi}_c (t_c^{s_i}) $ \blue{unironed}\\ 
% 3. ${\phi}_c (t)   >  {\phi}_{c+\epsilon} (t) $\\
% 4. ${\phi}_c (t_c^{s_i})   =  {\phi}_c^+ (t_c^{s_i}) $  The $\phi$ of at the begin of an ironing interval is greater or equal to $\phi^+$.\\
% 5. ${\phi}_c (t_c^{e_i})  = {\phi}_c^+ (t_c^{e_i}) $  The $\phi$ of at the end of an ironing interval is less or equal to $\phi^+$. \\ \blue{4,5 - boundary view of ironing. This was $\leq, \geq$. This equation represents the property of largest convex hull.}  \\
% 6. $H(z) \geq L(z)$ \blue{Integral view of ironing} \\
% 7. $L_c(z) \geq L_{c+\epsilon}(z)$ \blue{Large convex hull} \\
% 8. ${\phi}_c^+ (t) = L(t_c^{s_i}) - L(t_c^{e_i}) = H(t_c^{s_i}) - H(t_c^{e_i})$ \blue{ slope view of ironing}
% \sz{Feel like we have all properties. But we can't pin down the ironed intervals start point relation between $c$ and $c+\epsilon$.}

% % \sz{Shrink 4,5 to equation relationship  doesn't help.}
% % \sz{Is it possible to strength 4,5 to equation relationship if we can show $phi(t)$ is not constant at any interval in other words $\phi(t) \neq \phi(t+\epsilon)$. So, we can possibly prove the convex hull is got by tangent lines. }

% Given any $t \in (0,1)$ there are four possible cases:


% \textbf{Case 1:}
% Both ${\phi}_c^+ (t)$ and ${\phi}_{c+\epsilon}^+(t)$ are not ironed at $t$.
% \begin{align*}
% {\phi}_c^+ (t) =  {\phi}_c(t) = t+\frac{F(t)}{f(t)}-\frac{c}{f(t)} > t+\frac{F(t)}{f(t)}-\frac{c+\epsilon}{f(t)} = {\phi}_{c+\epsilon}(t) = {\phi}_{c+\epsilon}^+(t)    
% \end{align*}


% \textbf{Case 2:} \blue{facing similar problem as case 3.}
% ${\phi}_c^+ (t)$ is ironed and ${\phi}_{c+\epsilon}^+(t)$ is not ironed at $t$.



% \begin{align*}
% {\phi}_c^+ (t) =  {\phi}_c^+ (t_c^{e_i}) ={\phi}_c (t_c^{e_i}) =  t_c^{e_i}+\frac{F(t_c^{e_i})}{f(t_c^{e_i})}-\frac{c}{f(t_c^{e_i})} \red{>} t+\frac{F(t)}{f(t)}-\frac{c+\epsilon}{f(t)} = {\phi}_{c+\epsilon}(t) = {\phi}_{c+\epsilon}^+(t)    
% \end{align*}


% \textbf{Case 3:}
% ${\phi}_c^+ (t)$ is not ironed and ${\phi}_{c+\epsilon}^+(t)$ is ironed at $t$. Assume the start point of the ironed interval of  ${\phi}_{c+\epsilon}^+(t)$ that contains $t$ is $t_{c+\epsilon}^{s_j}$.



% \begin{align*}
% &{\phi}_c^+ (t) =  {\phi}_c(t) \\ 
% &{\phi}_{c}(t_{c+\epsilon}^{s_j}) > {\phi}_{c+\epsilon}(t_{c+\epsilon}^{s_j}) \geq {\phi}_{c+\epsilon}^+(t_{c+\epsilon}^{s_j}) = {\phi}_{c+\epsilon}^+(t)
% \end{align*}

% Since we also have 
% $$
% {\phi}_c^+ (t) \geq  {\phi}_c^+ (t_{c+\epsilon}^{s_j}) 
% $$

% Now, the questions becomes how to prove

% \blue{
% $$
% {\phi}_c^+ (t_{c+\epsilon}^{s_j}) \geq {\phi}_c (t_{c+\epsilon}^{s_j})
% $$
% }

% $$
% \frac{d(\phi_c(t)}{dt} = \frac{d(t +\frac{F(t)}{f(t)} - \frac{c}{f(t)})}{dt} =  \frac{d(t +\frac{F(t)}{f(t)})}{dt} -  \frac{f'(t) c}{f^2(t)}
% $$
% There are two small cases:

% \begin{prop}
% Can we prove the following with the fact of larger largest convex hull?

% If $\phi^+_c(t)$ ironed $\Longrightarrow$ $\phi^+_{c+\epsilon}(t)$ ironed.

% \begin{proof}
% From lager largest convex hull, we know:
% \begin{align*}
% L_c(t) &\geq L_{c+\epsilon}(t) \\
% \int_0^{F^{-1}(t)} \phi_c^+(t) &\geq \int_0^{F^{-1}(t)}  \phi_{c+\epsilon}^+(t)     
% \end{align*}

% \end{proof}
% \end{prop}s





% \textbf{Case 3.1:} 
% If ${\phi}_c(t_{c+\epsilon}^{s_j})$ is not ironed, we have 
% \begin{align} \label{c3.1}
% {\phi}_c^+ (t) \geq  {\phi}_c^+ (t_{c+\epsilon}^{s_j}) =  {\phi}_c(t_{c+\epsilon}^{s_j}) \geq {\phi}_{c+\epsilon}^+(t)
% \end{align}

% \textbf{Case 3.2:} 
% If ${\phi}_c(t_{c+\epsilon}^{s_j})$ is ironed, given $t_{c+\epsilon}^{s_j} \leq t$  prove  \blue{${\phi}_c(t) \geq {\phi}_c(t_{c+\epsilon}^{s_j})$.} 

% Inequality \eqref{c3.1}  doesn't hold because,
% \begin{align*}
% {\phi}_c^+ (t) \geq  {\phi}_c^+ (t_{c+\epsilon}^{s_j}) \red{=}  {\phi}_c(t_{c+\epsilon}^{s_j}) \geq {\phi}_{c+\epsilon}^+(t)
% \end{align*}
% The red $\red{=}$ is very hard to prove.

% So, we need to thinks from another direction, where 
% \begin{align} \label{c3.2}
% {\phi}_c^+ (t) =  {\phi}_c(t) \red{\geq}   {\phi}_c(t_{c+\epsilon}^{s_j})  > {\phi}_{c+\epsilon}(t_{c+\epsilon}^{s_j}) \geq {\phi}_{c+\epsilon}^+(t_{c+\epsilon}^{s_j}) = {\phi}_{c+\epsilon}^+(t)
% \end{align}

% This is also very hard because $\phi(t)$ is not non-decreasing and we may have ${\phi}_c(t_{c+\epsilon}^{s_j}) > {\phi}_c(t)$.
% And we can't reduce this to 
% \begin{align*}
% {\phi}_c(t_{c+\epsilon}^{s_j}) \leq   max_{t_{c}^{s_{i-1}}\leq t \leq t_{c}^{e_{i-1}}}({\phi}_c(t_{c}^{s_{i-1}}))
% \end{align*}
 
% Below graph will be a counter example of it,

% \begin{figure}[H]
% \includegraphics[scale=0.3]{fig/phi(t)-counter-1.png}
% \end{figure}
% There are infinite ${\phi}_c(t)$, so we can't prove \eqref{c3.2} by deduction.
% % \blue{Unless we doesn't realize some very straight properties of larger convex hull and ironing properties.} 

% Now we need to prove by contradiction \blue{(Still need extra properties of larger convex hull and ironing properties)} or find an counterexample.

% The logic of ironing, sharply decreasing $f(t)$ $\Rightarrow$ $\phi(t)$ decreasing  $\Rightarrow$ ironing.

% Suppose $c=0.1, \epsilon = 0.8$ for finding counterexample easier,
% the example needs to be strong enough that shows red $\red{\geq}$ in \eqref{c3.2} doesn't hold and reverse another $\geq$ in that inequality.
% \sz{Thinking counterexample prove no threshold?}

% \begin{align*}
% \phi_{0.1}(t) = t + \frac{F(t)}{f(t)} - \frac{0.1}{f(t)} \\
% \phi_{0.9}(t) = t + \frac{F(t)}{f(t)} - \frac{0.9}{f(t)}
% \end{align*}



% Find what direction the ironing interval will go.

% The view from Jason Hartline is from price-posting on quantile space to give intuition. And it returns to Myerson's appoarches after giving this intuition.


% \vspace{1cm}

% \textbf{Case 4:}
% Both ${\phi}_c^+ (t)$ and ${\phi}_{c+\epsilon}^+(t)$ are ironed at $t$.
% This case will combine the proof of case 2 and 3.

% There should be symmetry in proof.
% If we proved case 3.2, we can extend it to solve all cases.








\clearpage
\end{proof}












% \sz{second way}
% \begin{align*}
% {\phi}_c(t) = c\underline{\phi}(t) + (1-c) \bar{\phi}(t) = t+\frac{F(t)}{f(t)}-\frac{C}{f(t)}
% \end{align*}

% For any $c<c'$, for any z, we have  $h_c(z) > h_{c'}(z)$.
% Thus, $H_c(z)>H_{c'}(z)$.
% Thus, the convex hull of $H_{c'}(z)$ must be included in the convex hull $H_{c}(z)$.

% \begin{align*}
% H_{c'}(z) &= \int_0^z h_{c'}(z) dz \\
% &= \int_0^z F_{-1}(z) -\frac{z}{f(F_{-1}(z))}  - \frac{C'}{f(F_{-1}(z))} dz
% \end{align*}

% \begin{align*}
% H_c(z) - H_{c'}(z)&= \int_0^z \frac{C'-C}{f(F_{-1}(z))} dz \\
% \end{align*}

% For the unchanged intervals, we have 
% \begin{align*}
% l_c(z) - l_{c'}(z) = h_c(z) - h_{c'}(z) = t+\frac{F(t)}{f(t)}-\frac{c}{f(t)} - (t+\frac{F(t)}{f(t)}-\frac{c'}{f(t)}) = \frac{c'-c}{f(t)}  \geq 0 \\
% \end{align*}
% For a changed intervals suppose this intervals is $[z_s,z_e]$ , since we are finding the convex hull, for any $z_s\leq z \leq z_e$, we have $l_c(z_s) = l_c(z) = l_c(z_e) $

% Suppose for an arbitrary $z$, when $L_c(z)$ is in an changed interval $[z_s,z_e]$ and $L_{c'}(z)$ is not in changed interval.
% \sz{show $(L_c(z) - L_{c'}(z))$ is an integral on positive term}


% \begin{align*}
% (L_c(z) - L_{c'}(z))'& =  (L_c(z) - H_{c'}(z))'  \\
% & =  (H_c(z_s) + (H_c(z_e) - H_c(z_s))\frac{z-z_s}{z_e-z_s} - H_{c'}(z))' \\
% & =  (H_c(z_s) - H_c(z_s)\frac{z-z_s}{z_e-z_s} + H_c(z_e)\frac{z-z_s}{z_e-z_s}  - H_{c'}(z))' \\
% & =  (\frac{z_e}{z_e-z_s}H_c(z_e) - H_c(z_e)\frac{z}{z_e-z_s} + H_c(z_s)\frac{z}{z_e-z_s} - H_c(z_s)\frac{z_s}{z_e-z_s} - H_{c'}(z))' \\
% & = \frac{H_c(z_e) - H_c(z_s)}{z_e-z_s} - h_{c'}(z) \\
% & = \frac{\int_{z_s}^{z_e}h_c(z) dz}{z_e-z_s}  - h_{c'}(z) \\
% & \geq \frac{\int_{z_s}^{z_e}h_c(z) dz}{z_e-z_s}  - l_{c'}(z_e) \\
% \end{align*}

% % \begin{align*}
% % (L_c(z) - L_{c'}(z))'& =  (L_c(z) - H_{c'}(z))'  \\
% % & =  (H_c(z_s) + (H_c(z_e) - H_c(z_s))\frac{z-z_s}{z_e-z_s} - H_{c'}(z))' \\
% % & =  (H_c(z_s) - H_c(z_s)\frac{z-z_s}{z_e-z_s} + H_c(z_e)\frac{z-z_s}{z_e-z_s}  - H_{c'}(z))' \\
% % & =  (\frac{z_e}{z_e-z_s}H_c(z_s) - H_c(z_e)\frac{z}{z_e-z_s} + H_c(z_s)\frac{z}{z_e-z_s} - H_c(z_s)\frac{z_s}{z_e-z_s} - H_{c'}(z))' \\
% % & = \frac{H_c(z_e) - H_c(z_s)}{z_e-z_s} - h_{c'}(z) \\
% % & = \frac{\int_{z_s}^{z_e}h_c(z) dz}{z_e-z_s}  - h_{c'}(z) \\
% % & \geq \frac{\int_{z_s}^{z_e}h_c(z) dz}{z_e-z_s}  - h_{c'}(z_e) \\
% % \end{align*}

% % \begin{align*}
% % (L_c(z) - L_{c'}(z))'& =  (L_c(z) - H_{c'}(z))'  \\
% % & =  (H_c(z_s) + (H_c(z_e) - H_c(z_s))\frac{z-z_s}{z_e-z_s} - H_{c'}(z))' \\
% % % & =  (H_c(z_s) - H_c(z_s)\frac{z-z_s}{z_e-z_s} + H_c(z_e)\frac{z-z_s}{z_e-z_s}  - H_{c'}(z))' \\
% % % & =  (\frac{z_e}{z_e-z_s}H_c(z_s) - H_c(z_e)\frac{z}{z_e-z_s} + H_c(z_s)\frac{z}{z_e-z_s} - H_c(z_s)\frac{z_s}{z_e-z_s} - H_{c'}(z))' \\
% % & = \frac{H_c(z_e) - H_c(z_s)}{z_e-z_s} - h_{c'}(z) \\
% % & = \frac{\int_{z_s}^{z_e}h_c(z) dz}{z_e-z_s}  - h_{c'}(z) \\
% % \end{align*}

% \begin{align*}
% (L_c(z) - L_{c'}(z))'& =  (L_c(z) - H_{c'}(z))' \geq 0 \\
% l_c(z) - l_{c'}(z) &  \geq 0 \\
% l_c(z) &  \geq l_{c'}(z) \\
% \end{align*}


% Then, some how we can get $l_c(z) \geq l_{c'}(z)$ 


% \sz{The second possible way is to show:}
% $$
%  \int_{t_1}^{t_2} \int_{q: \rho(q) \geq - \phi(x)} g(q) v_1(q) \,\dd q\dd x = \int_{t_1}^{t_2} \int_{q: \rho(q) \geq - \phi^+(x)} g(q) v_1(q) \,\dd q\dd x
% $$
% If we can prove this, we can show the this whole term is decreasing in C, thus we  can use binary search to find C. Also, we can show the boundary doesn't change after ironing.

% Now, we are going to prove the last term also doesn't change after ironing.
% Consider the following term,
% \begin{align*}
% \int_{t_1}^{t_2} \int_{q: \rho(q) \geq - \phi(x)} g(q) v_1(q) \,\dd q\dd x & = 
% \int_{t:  -\phi(t) \leq \rho(q) } \int_{q \in Q }  g(q) v_1(q) \,\dd q\dd t  \\
% &= \int_{q \in Q }  \int_{t:  -\phi(t) \leq \rho(q) }  1 \, \dd t \,g(q)  v_1(q) \,\dd q \\
% &= \int_{q \in Q }  \int_{t:  -\phi(t) \leq \rho(q) }  1 \, \dd t\,\dd q \; \int_{q \in Q }  \,g(q)  v_1(q) \,\dd q \\
% \end{align*}
% If we have $ \int_{q \in Q }  \int_{t:  -\phi(t) \leq \rho(q) }  1 \, \dd t\,\dd q \; = \int_{q \in Q }  \int_{t:  -\phi^+(t) \leq \rho(q) }  1 \, \dd t\,\dd q \;$ Then,
% \begin{align*}
%  \int_{q \in Q }  \int_{t:  -\phi(t) \leq \rho(q) }  1 \, \dd t\,\dd q \; \int_{q \in Q }  \,g(q)  v_1(q) \,\dd q &=  \int_{q \in Q }  \int_{t:  -\phi^+(t) \leq \rho(q) }  1 \, \dd t\,\dd q \; \int_{q \in Q }  \,g(q)  v_1(q) \,\dd q\\
% &= \int_{q \in Q }  \int_{t:  -\phi^+(t) \leq \rho(q) }  1 \, \dd t \,g(q)  v_1(q) \,\dd q \\
% &= \int_{t:  -\phi^+(t) \leq \rho(q) } \int_{q \in Q }  g(q) v_1(q) \,\dd q\dd t \\
% &=  \int_{t_1}^{t_2} \int_{q: \rho(q) \geq - \phi^+(x)} g(q) v_1(q) \,\dd q\dd x \\
% \end{align*}

% From above derivation, we can see an equivalence (which helps us prove it or show a counterexample of it). 
% \begin{align*}
%  \int_{q \in Q }  \int_{t:  -\phi(t) \leq \rho(q) }  1 \, \dd t\,\dd q \; &= \int_{q \in Q }  \int_{t:  -\phi^+(t) \leq \rho(q) }  1 \, \dd t\,\dd q \; \Longleftrightarrow \\
%  \int_{t_1}^{t_2} \int_{q: \rho(q) \geq - \phi(x)} g(q) v_1(q) \,\dd q\dd x & = \int_{t_1}^{t_2} \int_{q: \rho(q) \geq - \phi^+(x)} g(q) v_1(q) \,\dd q\dd x \\
% \end{align*}
% Thus, the key is to show the following red equation, and we only need to consider changed interval in ironing, and each interval should hold for themselves. For each interval with $[t_s,t_e]$, we have 1.$H(F^{-1}(t_s)) - H(F^{-1}(t_e)) = L(F^{-1}(t_s)) - L(F^{-1}(t_e))$ \\
% 2. $l(F^{-1}(t)) = L(F^{-1}(t'))$ for any $t,t'$ in $[t_s,t_e]$. This means the right term will suddenly include all $t$ in $[t_s,t_e]$.
% \begin{align*} \color{red}
%  \int_{q \in Q }  \int_{t:  -\phi(t) \leq \rho(q) }  1 \, \dd t\,\dd q \; = \int_{q \in Q }  \int_{t:  -\phi^+(t) \leq \rho(q) }  1 \, \dd t\,\dd q \;
% \end{align*}
% (It is indeed true that this equation holds for the Example 2 in page 12, and this should not be a coincidence.)


% \begin{align*} 
%   \int_{q \in Q }  \int_{t:  -\phi(t) \leq \rho(q), \; t\in [t_s,t_e]}  1 \, \dd t\,\dd q \; &=  \int_{q \in Q }   \int_{t \geq \phi^{-1}(- \rho(q)) }^{t_e}  1 \, \dd t\,\dd q \; \\
% \end{align*}
% We have 
% \begin{align*} 
%  \frac{\partial \int_{q \in Q }   \int_{t \geq \phi^{-1}(- \rho(q)) }^{t_e}  1 \, \dd t\,\dd q \;}{\partial t} 
% \end{align*}

% When $ \phi^{-1}(- \rho(q)) < t_s$, above partial derivative is 0.

% When $ \phi^{-1}(- \rho(q)) \geq t_s$, above partial derivative is:
% \begin{align*} 
%  \frac{\partial \int_{q \in Q }   \int_{t \geq \phi^{-1}(- \rho(q)) }^{t_e}  1 \, \dd t\,\dd q \;}{\partial t} &=   \int_{q \in Q }   - \phi^{-1}(- \rho(q))   \dd q  
% \end{align*}


% \begin{align*} 
%  \int_{q \in Q }  \int_{t:  -\phi(t) \leq \rho(q), \; t\in [t_s,t_e]}  1 \, \dd t\,\dd q \; &=  \int_{q \in Q }  \int_{z:  -\phi(F^{-1}(z)) \leq \rho(q) } (F^{-1}(z))' \, \dd z\,\dd q \; \\
%  &=  \int_{q \in Q }  \int_{z:  -h(z) \leq \rho(q) }  (F^{-1}(z))' \, \dd z\,\dd q \; \\
% \end{align*}

% \begin{align*} 
%  \int_{q \in Q }  \int_{t:  -\phi(t) \leq \rho(q), \; t\in [t_s,t_e]}  1 \, \dd t\,\dd q \; &=  \int_{q \in Q }  \int_{z:  -\phi(F^{-1}(z)) \leq \rho(q) } \, 1 \dd (F^{-1}(z))\,\dd q \; \\
%  &=  \int_{q \in Q }  \int_{z:  -h(z) \leq \rho(q) }  1 \, \dd (F^{-1}(z))\,\dd q \; \\
% \end{align*}

% In ironed version, $-\phi^+(t)$ is a constant for $ t\in [t_s,t_e]$
% \begin{align*} 
%  \int_{q \in Q }  \int_{t:  -\phi^+(t) \leq \rho(q), \; t\in [t_s,t_e]}  1 \, \dd t\,\dd q \; &=  (t_s-t_e)\int_{q: \rho(q)\geq -\phi^+(t_s) }  1 \, \dd q \\
% \end{align*}

% \begin{align*} 
% \frac{\partial (t_s-t_e)\int_{q: \rho(q)\geq -\phi^+(t_s) }  1 \, \dd q }{\partial q} & = - (t_s-t_e)  \rho^{-1}( -\phi^+(t_s))\\
% & =  -\int_{t_s}^{t_e} - \rho^{-1}( -\phi^+(t)) dt \\
% & =  -\int_{t_s}^{t_e} - \rho^{-1}( -\phi^+(t)) dt \\
% \end{align*}

% \end{proof}

% Define the lower threshold $\underline{\theta}_t$ and the upper threshold $\bar{\theta}_t$ as:
% \begin{gather*}
%     \underline{\theta}_t = -\underline{\phi}^+(t) \quad \mathrm{and}\quad \bar{\theta}_t = -\bar{\phi}^+(t), \forall t \in T,
% \end{gather*}
% and denote by $\underline{\pi}(q,t)$ and $\bar{\pi}(q,t)$ the corresponding recommendation schemes. For ease of presentation, we also define the following function with respect to a recommendation scheme $\pi$:
% \begin{gather}
%     P_{\pi}(t) = \int_{q \in Q}  \pi(q, t) g(q) v_1(q) \,\dd q.
%     \label{eq:def_P}
% \end{gather}
% In particular, if $\pi$ is a threshold mechanism with threshold $\theta_t$, we have
% \begin{gather*}
%     P_{\pi}(t) = \int_{q:\rho(q)\ge \theta_t} g(q) v_1(q) \,\dd q.
% \end{gather*}

==> notes.tex <==

\section{Previous work}
% We first consider the case where $Q,T$ are independent.  By \cite{chen2020selling}, we know that the optimal mechanism is a ``consulting mechanism" which, upon seeing the product quality,  charges the buyer of type $t$ a payment $p_t$ and meanwhile makes an incentive compatibility recommendation based on signaling scheme $\pi_t(q,a)$ where action $a \in \{ 0, 1 \}$. 

We thus can formulate the problem as the following convex program (CP).

\begin{lp}\label{lp:OptScheme}
	\maxi{ \sum_{t} f(t) \cdot p(t)}
	\st
	\qcon{ \sum_{q} \pi(q,t) g(q) v(q,t) \geq 0  }{t} 
	\qcon{ \sum_{q} (1-\pi(q,t)) g(q) v(q,t)  \leq 0  }{t} 
	\con{ \sum_{q} \pi(q,t) g(q) v(q,t)- p_t \geq}
	\qcon{  \quad \max \{ \sum_{q} \pi_{t'}(q,1) g(q)  v(q,t) , 0 \} + \max \{ \sum_{q} \pi_{t'}(q,0) g(q) v(q,t), 0 \}   - p_{t'} }{t, t'} 
	\qcon{ \sum_{q} \pi_t(q,1) \cdot v(q,t)  - p_t \geq \max\{  0,  \bar{v}_t \}  }{t} 
	\qcon{ \pi_t(q,1) + \pi_t(q,0) = g(q) }{q, t}
	\qcon{\pi_t(q,0), \pi_t(q,1) \geq 0}{q,t} 
\end{lp}
where the first two are obedience constraints, enforcing the recommendation is obedient (recall that $0$ is the utility of taking action $0$). The third constraint is the incentive compatible constraint, enforcing that a buyer of type $t$ should not misreport type $t'$. The forth constraint  describes individual rationality. That is, participating the information selling mechanism should  lead to utility that is at least the utility of no participation  $\max\{  0,  \bar{v}_t \}  $. The last two constraints are feasibility of the information selling scheme. 

\subsection{Characterization of Optimal Mechanism}
We start by simplifying CP \ref{lp:OptScheme} with a few claims. 
\begin{claim}
There always exists an optimal solution to CP \ref{lp:OptScheme}  such that $p_t \geq 0$ for all $t$. Therefore,  the first constraint is dominated by the forth constraint in this optimal solution. 
\end{claim}
\begin{proof}
If $p_t < 0$ for some $t$ in some optimal solution. Then by changing to  $p_t = 0$ (higher payment) and  $\pi_t$ to revealing no information (less information) will always increase revenue. Moreover, this will not violate any incentive compatibility constraint neither since deviating to $t$ from any other type $t'$ now will only pay more but gets less information.   
\end{proof}

\begin{claim}
The third constraint can be reduced to  $\sum_{q} \pi_t(q,1) \cdot v(q,t) - p_t 
 \geq  \sum_{q} \pi_{t'}(q,1) \cdot v(q,t) - p_{t'}$. 
\end{claim}
\begin{proof}
Note that if both $\max \{ \sum_{q} \pi_{t'}(q,1) \cdot v(q,t), 0 \} $ and $ \max \{ \sum_{q} \pi_{t'}(q,0) \cdot v(q,t) , 0 \} $ achieve the maximum at the non-zero term, then the third constraint will be implied by the fifth constraint. It can also be shown that it can never be the case that the first max is achieved at zero but the second is achieved at the non-zero term. When both max are zero, the third term is dominated by the forth. So the only remaining situation is what stated in the claim. 
\end{proof}

Utilizing the above two claims,  CP \eqref{lp:OptScheme} can be reduced to the following LP: 
\begin{lp}\label{lp:OptScheme-simple}
	\maxi{ \sum_{t} f(t) \cdot p_t}
	\st
	\qcon{ \sum_{q} \pi_t(q,0) \cdot v(q,t)  \leq 0  }{t} 
	\qcon{\sum_{q} \pi_t(q,1) \cdot v(q,t) - p_t 
		\geq  \sum_{q} \pi_{t'}(q,1) \cdot v(q,t) - p_{t'} }{t, t'} 
	\qcon{ \sum_{q} \pi_t(q,1) \cdot v(q,t)  - p_t \geq \max\{  0,  \bar{v}_t \}  }{t} 
	\qcon{ \pi_t(q,1) + \pi_t(q,0) = g(q) }{q, t}
	\qcon{\pi_t(q,0), \pi_t(q,1) \geq 0}{q,t} 
\end{lp}


Slightly re-writing this LP:
\begin{lp}\label{lp:OptScheme-variant}
	\maxi{ \sum_{t} f(t) \cdot p_t}
\st
\qcon{ \sum_{q} \pi_t(q,0) \cdot v(q,t)  \leq 0  }{t} 
\qcon{\sum_{q} \big[ \pi_{t'}(q,1)  - \pi_{t}(q,1)\big] \cdot v(q,t) + p_t  - p_{t'} \leq 0  }{t, t'} 
\qcon{  p_t - \sum_{q} \pi_t(q,1) \cdot v(q,t)  \leq  - \max\{  0,  \bar{v}_t \}  }{t} 
\qcon{ \pi_t(q,1) + \pi_t(q,0) = g(q) }{q, t}
\qcon{\pi_t(q,0), \pi_t(q,1) \geq 0}{q,t}  
\end{lp}


Let $y_t, \beta_{t,t'},  \lambda_t, w_{q,t}$ be the corresponding dual variables for first four constraints , we obtain the following dual program. 
\begin{lp}\label{lp:OptScheme-dual}
	\mini{ \sum_{t} \sum_{q}  g(q) \cdot w_{q,t}  -  \sum_{t} \lambda_t \cdot \max \{ 0,  \bar{v}(t)  \} }
	\st
	\qcon{  -  v(q,t)  \cdot \big[  \lambda_t + \sum_{t'}  \beta_{t,t'}  \big] +  \sum_{t'}  v(q,t')  \cdot  \beta_{t',t}  + w_{q,t} \geq 0}{q, t}
	\qcon{  v(q,t)  \cdot  y_t      + w_{q,t} \geq 0}{q, t}  
	\qcon{ \sum_{t'} \beta_{t,t'}  - \sum_{t'}  \beta_{t',t} + \lambda_t  = f(t) }{t}
	\qcon{y,  \beta,  \lambda  \geq 0}{q,t} 
\end{lp}

\begin{claim}
LP \eqref{lp:OptScheme-dual} always has an optimal solution such that $y_t = \infty$ wh
\end{claim}


%
%\begin{lp}
%	\mini{ \sum_{t} \sum_{q}  g(q) \cdot w_{q,t} + \sum_{t} \min \{ 0, \alpha - \bar{v}(t)  \} }
%	\st
%	\qcon{ - ( v(q,t) - \alpha  ) \cdot x_t  - (v(q,t) -\alpha  ) \cdot \sum_{t'}  (\beta_{t,t'} +\gamma_{t,t'})+  \sum_{t'}  ( v(q,t') -\alpha ) \cdot  \beta_{t',t} -  \lambda_t ( v(q,t) -\alpha )  + w_{q,t} \geq 0}{q, t} 
%	\qcon{ ( v(q,t) - \alpha  ) \cdot y_t  +   \sum_{t'}  ( v(q,t') -\alpha ) \cdot  \gamma_{t',t}  + w_{q,t} \geq 0}{q, t}  
%	\qcon{ \sum_{t'} [  \beta_{t,t'} + \gamma_{t,t'} ] - \sum_{t'} [\beta_{t',t} + \gamma_{t',t}]  + \lambda_t  = 0 }{t}
%	\qcon{x, y, \alpha, \beta, \gamma, \lambda  \geq 0}{q,t} 
%\end{lp}
%
%
%
%\begin{lp}\label{lp:OptScheme-variant}
%	\maxi{ \sum_{t} f(t) \cdot p_t}
%	\st
%	\qcon{ \sum_{q} \pi_t(q,1) \cdot ( \alpha -v(q,t)) \leq 0  }{t} 
%	\qcon{ \sum_{q} \pi_t(q,0) \cdot (v(q,t) - \alpha) \leq 0  }{t} 
%%	\qcon{ \sum_{q} \pi_t(q,0)(v(q,t) - \alpha) + p_t- p_{t'} \leq 0}{t,t'} 
%	\qcon{  \sum_{q} [\pi_{t'}(q,1) - \pi_t(q,1)] \cdot (v(q,t) - \alpha)  + p_t - p_{t'}  \leq 0 }{t, t'} 
%	\qcon{  \sum_{q} [\pi_{t'}(q,0) - \pi_t(q,1)] \cdot (v(q,t) - \alpha)  + p_t - p_{t'}  \leq 0 }{t, t'}  
%	\qcon{ p_t - \sum_{q} \pi_t(q,1) \cdot (v(q,t) - \alpha)  \leq \min \{ 0, \alpha - \bar{v}(t)  \}}{t} 
%	\qcon{ \pi_t(q,1) + \pi_t(q,0) = g(q) }{q, t}
%	\qcon{\pi_t(q,0), \pi_t(q,1) \geq 0}{q,t} 
%\end{lp}
%
%Let $x_t, y_t, \beta_{t,t'}, \gamma_{t,t'}, \lambda_t, w_{q,t}$ be the corresponding dual variables, we obtain the following dual program. 
%\begin{lp}
%	\mini{ \sum_{t} \sum_{q}  g(q) \cdot w_{q,t} + \sum_{t} \min \{ 0, \alpha - \bar{v}(t)  \} }
%	\st
%	\qcon{ - ( v(q,t) - \alpha  ) \cdot x_t  - (v(q,t) -\alpha  ) \cdot \sum_{t'}  (\beta_{t,t'} +\gamma_{t,t'})+  \sum_{t'}  ( v(q,t') -\alpha ) \cdot  \beta_{t',t} -  \lambda_t ( v(q,t) -\alpha )  + w_{q,t} \geq 0}{q, t} 
%	\qcon{ ( v(q,t) - \alpha  ) \cdot y_t  +   \sum_{t'}  ( v(q,t') -\alpha ) \cdot  \gamma_{t',t}  + w_{q,t} \geq 0}{q, t}  
%	\qcon{ \sum_{t'} [  \beta_{t,t'} + \gamma_{t,t'} ] - \sum_{t'} [\beta_{t',t} + \gamma_{t',t}]  + \lambda_t  = 0 }{t}
%	\qcon{x, y, \alpha, \beta, \gamma, \lambda  \geq 0}{q,t} 
%\end{lp}
%
%Re-writing the Dual: 
%\begin{lp}\label{lp:OptScheme-Dual}
%	\mini{ \sum_{t} \sum_{q}  g(q) \cdot w_{q,t}  + \sum_{t} \min \{ 0, \alpha - \bar{v}(t)  \} }
%	\st
%	\qcon{  -  (v(q,t) -\alpha  ) \cdot \big[ x_t + \lambda_t + \sum_{t'}  (\beta_{t,t'} +\gamma_{t,t'}) \big] +  \sum_{t'}  ( v(q,t') -\alpha ) \cdot  \beta_{t',t}  + w_{q,t} \geq 0}{q, t}
%		\qcon{ ( v(q,t) - \alpha  ) \cdot  y_t    +   \sum_{t'}  ( v(q,t') -\alpha ) \cdot  \gamma_{t',t}  + w_{q,t} \geq 0}{q, t}  
%			\qcon{ \sum_{t'} [ \beta_{t,t'} + \gamma_{t,t'} ] - \sum_{t'} [ \beta_{t',t} + \gamma_{t',t}]  + \lambda_t  = f(t) }{t}
%	\qcon{x, y, \alpha, \beta, \gamma, \lambda  \geq 0}{q,t} 
%\end{lp}
%
%
%After removing $x, \gamma$ for the above LP, we have:
%\begin{lp}
%	\mini{ \sum_{t} \sum_{q}  g(q) \cdot w_{q,t}  + \sum_{t} \lambda_t \cdot \min \{ 0, \alpha - \bar{v}(t)  \} }
%	\st
%	\qcon{  -  (v(q,t) -\alpha  ) \cdot \big[  \lambda_t + \sum_{t'}  \beta_{t,t'}  \big] +  \sum_{t'}  ( v(q,t') -\alpha ) \cdot  \beta_{t',t}  + w_{q,t} \geq 0}{q, t}
%	\qcon{ ( v(q,t) - \alpha  ) \cdot  y_t      + w_{q,t} \geq 0}{q, t}  
%	\qcon{ \sum_{t'} \beta_{t,t'}  - \sum_{t'}  \beta_{t',t} + \lambda_t  = f(t) }{t}
%	\qcon{x, y, \alpha, \beta,  \lambda  \geq 0}{q,t} 
%\end{lp}

%This can be further simplified:
%\begin{lp}
%	\mini{ \sum_{t} \sum_{q}  g(q) \cdot w_{q,t}  + \sum_{t} \lambda_t \cdot \min \{ 0, \alpha - \bar{v}(t)  \} }
%	\st
%	\qcon{  -  (v(q,t) -\alpha  ) \cdot   f(t)  +  \sum_{t'}  ( v(q,t') -v(q,t)) \cdot  \beta_{t',t}  + w_{q,t} \geq 0}{q, t}
%	\qcon{ ( v(q,t) - \alpha  ) \cdot  y_t      + w_{q,t} \geq 0}{q, t}
%	\qcon{ \sum_{t'} \beta_{t,t'}  - \sum_{t'}  \beta_{t',t} + \lambda_t  = f(t) }{t} 
%	\qcon{ y, \beta,  \lambda  \geq 0}{q,t} 
%\end{lp}


\todo{Want to argue that the above LP and its dual have the desired property as in Conjecture 1.  One idea is to 
 prove that for any fixed $t$, there is some $\theta_t$ such that the  first constraint in the above dual is tight when $q > \theta_t$ and the second constraint is tight when $q < \theta_t$.  }

%At the end of the day, it boils down to compare
%\begin{eqnarray*}
%&& \bigg[ -  (v(q,t) -\alpha  ) \cdot \big[ x_t + \lambda_t + \sum_{t'}  (\beta_{t,t'} +\gamma_{t,t'}) \big] +  \sum_{t'}  ( v(q,t') -\alpha ) \cdot  \beta_{t',t}  \bigg] \\
%& &  \qquad - \bigg[  ( v(q,t) - \alpha  ) \cdot [y_t  + \sum_{t'} \alpha_{t,t'}]  +   \sum_{t'}  ( v(q,t') -\alpha ) \cdot  \gamma_{t',t}  \bigg] \\ 
%& = & -  (v(q,t) -\alpha  ) \cdot \big[ x_t + y_t  + \lambda_t + \sum_{t'}  ( \alpha_{t,t'} + \beta_{t,t'} +\gamma_{t,t'}) \big] +  \sum_{t'}  ( v(q,t') -\alpha ) \cdot  [\beta_{t',t}  -  \gamma_{t',t}] \\ 
%& = & -  (v(q,t) -\alpha  ) \cdot \big[ x_t + y_t  + f(t) + \sum_{t'} [\alpha_{t',t} + \beta_{t',t} + \gamma_{t',t}]    \big] +  \sum_{t'}  ( v(q,t') -\alpha ) \cdot  [\beta_{t',t}  -  \gamma_{t',t}] \\  
%\end{eqnarray*}

\section{Previous Random Thoughts}

\subsection{Myersonian Approach for Continuous $Q,T$}
Here we consider the case where both $t\in[0,\infty)$ and $q\in[0,\infty)$ are continuous. Assume that $v(q,0)=0,\forall q$, and $q\sim G(q)$ and $t\sim F(t)$.

 
Thus,
\begin{gather}
\Ex_{q\sim G}\left[ \left(\pi_{t'}(q,1)-\pi_{t}(q,1)\right)v(q,t) \right]\le p_{t'}-p_t\le \Ex_{q\sim G}\left[ \left(\pi_{t'}(q,1)-\pi_{t}(q,1)\right)v(q,t') \right],\nonumber\\
\Ex_{q\sim G}\left[ \left(\pi_{t'}(q,1)-\pi_{t}(q,1)\right)\left(v(q,t')-v(q,t)\right) \right]\ge 0.\label{eq:allocation_monotonicity}
\end{gather}
Equation \eqref{eq:allocation_monotonicity} is called allocation monotonicity in the standard auction setting.

Define
\begin{gather*}
u(t)= \Ex_{q\sim G}\left[ \pi_{t}(q,1)v(q,t) \right]-p_t
\end{gather*}
With Equation \eqref{eq:ic1} and \eqref{eq:ic2}, we also get:
\begin{align*}
u(t)&\ge \Ex_{q\sim G}\left[ \pi_{t'}(q,1)v(q,t') \right]-p_{t'}+\Ex_{q\sim G}\left[ \pi_{t'}(q,1)\left( v(q,t)-v(q,t') \right) \right]\\
&=u(t')+\Ex_{q\sim G}\left[ \pi_{t'}(q,1)\left( v(q,t)-v(q,t') \right) \right].
\end{align*}
Therefore,
\begin{gather*}
\Ex_{q\sim G}\left[ \pi_{t'}(q,1)\left( v(q,t)-v(q,t') \right) \right]\le u(t)-u(t')\le \Ex_{q\sim G}\left[ \pi_{t}(q,1)\left( v(q,t)-v(q,t') \right) \right].
\end{gather*}
Assume $t'<t$, divide the above inequality by $t-t'$, and let $t'\to t$,
\begin{gather*}
\odv{u(t)}{t}=\Ex_{q\sim G}\left[ \pi_{t}(q,1)\pdv{v(q,t)}{t} \right].
\end{gather*}

\begin{align*}
REV&=\int_{0}^{+\infty}f(t)p_t\,\mathrm{d}t\\
&=\int_{0}^{+\infty}f(t)\left(\Ex_{q\sim G}\left[ \pi_{t}(q,1)v(q,t)-u(t) \right]\right)\,\mathrm{d}t\\
&=\int_{0}^{+\infty}f(t)\left(\Ex_{q\sim G}\left[ \pi_{t}(q,1)v(q,t)-\int_{0}^{t}\odv{u(s)}{s}\mathrm{d}s-u(0) \right]\right)\,\mathrm{d}t\\
&=\int_{0}^{+\infty}f(t)\left(\Ex_{q\sim G}\left[ \pi_{t}(q,1)v(q,t) \right]\right)\,\mathrm{d}t-\int_{0}^{+\infty}\int_{s}^{+\infty}f(t)\odv{u(s)}{s}\,\mathrm{d}t\,\mathrm{d}s-u(0)\\
&=\int_{0}^{+\infty}f(t)\left(\Ex_{q\sim G}\left[ \pi_{t}(q,1)v(q,t) \right]\right)\,\mathrm{d}t-\int_{0}^{+\infty}(1-F(s))\odv{u(s)}{s}\,\mathrm{d}s-u(0)\\
&=\Ex_{q\sim G}\left[\int_{0}^{+\infty}f(t)\left(\pi_{t}(q,1)v(q,t) \right)\right]\,\mathrm{d}t-\int_{0}^{+\infty}(1-F(t))\Ex_{q\sim G}\left[ \pi_{t}(q,1)\pdv{v(q,t)}{t} \right]\,\mathrm{d}t-u(0)\\
&=\Ex_{q\sim G}\left[ \int_{0}^{+\infty}f(t)\pi_t(q,1)\left(v(q,t)-\pdv{v(q,t)}{t}\frac{1-F(t)}{f(t)}\right)\,\mathrm{d}t \right]-u(0)
\end{align*}
As $\odv{u(t)}{t}\ge0$, we can set $u(0)=0$. Let
\begin{gather*}
\varphi(t|q)=v(q,t)-\pdv{v(q,t)}{t}\frac{1-F(t)}{f(t)}.
\end{gather*}
We have
\begin{gather*}
REV=\Ex_{q\sim G}\left[ \int_{0}^{+\infty}f(t)\pi_t(q,1)\varphi(t|q)\,\mathrm{d}t \right].
\end{gather*}
Similar to the Myerson auction, there is a threshold $\theta_q$ for each $q$. We may need the ``ironing'' trick and define
\begin{gather*}
R(\eta|q)=v\cdot \eta,
\end{gather*}
where $\eta=1-F(t)$. And we also have $\pdv{R(\eta|q)}{\eta}=\varphi(t|q)$.

With Equation \eqref{eq:allocation_monotonicity}, any threshold testing mechanism must satisfy that $\theta_t$ is decreasing in $t$. If the optimal mechanism is a threshold testing mechanism, then $\theta_q$ must also be a decreasing function of $q$. With the regularity assumption, we have
\begin{gather*}
v(q,\theta_q)-\pdv{v(q,\theta_q)}{\theta_q}\frac{1-F(\theta_q)}{f(\theta_q)}=0.
\end{gather*}
Therefore, the optimal mechanism is a threshold testing mechanism if and only if
\begin{gather*}
\odv{\theta_q}{q}\le 0,
\end{gather*}
where
\begin{gather*}
\odv{\theta_q}{q}=-\frac{\pdv{v(q,\theta_q)}{q}-\pdv{v(q,\theta_q)}{q,\theta_q}\frac{1-F(\theta_q)}{f(\theta_q)}}{\pdv{v(q,\theta_q)}{\theta_q}-\pdv[2]{v(q,\theta_q)}{\theta_q}\frac{-f^2(\theta_q)-(1-F(\theta_q))f'(\theta_q)}{f^2(\theta_q)}}
\end{gather*}



\hf{
The feasible mechanism characterization with general $v(q,t)$  is the following, which I do not know how to prove 

\begin{lemma}\label{lem:feasible}
A mechanism $(\pi, p)$ is feasible if and only if it satisfies the following constraints:
\begin{eqnarray} 
&& \int_{q_1}^{q_2} g(q) [\pi(q,t) - \pi(q,t')][v(q,t) - v(q,t')] \geq 0 \\ 
&& u(t) = u(t_1) + \int_{q_1}^{q_2}\int_{t_1}^{t}  g(q) \pi(q,x) \frac{\partial v(q,x)}{\partial x}  dx, \, \, \, \forall t \in [T] \\ 
& & u(t_2) \geq v(t_2) \\  
& & p(t) \geq 0, \, u(t) \geq 0 \, \, \, \forall t \in [T]
 \end{eqnarray}
\end{lemma}
\begin{proof}

An equivalence to Condition (20) is the 
\begin{equation}
p'(t) =  \int_{q_1}^{q_2}  g(q) \frac{\partial \pi(q,t)}{\partial t}  v(q,t)    dq, \, \, \, \forall t \in [T] 
\end{equation}
This comes from the definition of $u(t):$
\begin{equation}
u(t) =  \int_{q_1}^{q_2}  g(q)  \pi(q,t)  v(q,t)    dq - p(t), \, \, \, \forall t \in [T] 
\end{equation}





Therefore, the IC constraint is equivalent to 
\begin{eqnarray}
&& \int_{t'}^t \int_{q_1}^{q_2} \left[ g(q) \pi(q,s) \frac{\partial v(q,s)}{\partial s}   \right] dq  ds \geq \int_{q_1}^{q_2} \pi(q, t') \cdot g(q) [v(q,t) - v(q,t')] dq \\
&\Longleftrightarrow&  \int_{q_1}^{q_2} g(q) \Bigg[ \int_{t'}^t  \left[ \pi(q,s) \frac{\partial v(q,s)}{\partial s}   \right] ds - \pi(q, t')  [v(q,t) - v(q,t')]  \Bigg]  dq  \geq 0 \\ 
&\Longleftrightarrow&  \int_{q_1}^{q_2} g(q) \Bigg[ \int_{t'}^t  \left[ \pi(q,s) \frac{\partial v(q,s)}{\partial s}   \right] ds - \int_{t'}^t \pi(q, t') \frac{\partial v(q,s)}{ \partial s} ds  \Bigg]  dq  \geq 0 \\  
&\Longleftrightarrow&  \int_{q_1}^{q_2} g(q) \Bigg[ \int_{t'}^t  \left[ [\pi(q,s) - \pi(q, t')] \frac{\partial v(q,s)}{\partial s}   \right] ds \Bigg]  dq  \geq 0 \\   
&\Longleftrightarrow&  \int_{q_1}^{q_2} g(q) \Bigg[   [\pi(q,s) - \pi(q, t')]v(q,s)|_{t'}^t -    \int_{t'}^t  \left[ \frac{\partial \pi(q,s)}{\partial s} v(q,s)  \right] ds     \Bigg]  dq  \geq 0 \\    
&\Longleftrightarrow&  \int_{q_1}^{q_2} g(q) \Bigg[   [ \pi(q,t) - \pi(q, t')]v(q,t) -    \int_{t'}^t  \left[ \frac{\partial \pi(q,s)}{\partial s} v(q,s)  \right] ds     \Bigg]  dq  \geq 0 \\     
&\Longleftrightarrow& \int_{q_1}^{q_2} g(q) \Bigg[  \int_{t'}^t  \left[ \frac{\partial \pi(q,s)}{\partial s} [v(q,t) - v(q,s)]  \right] ds     \Bigg]  dq  \geq 0 
\end{eqnarray} 
\end{proof}

}





\subsection{Other Directions to Pursue }
One reasonable simplification is to assume $v(q,t) = q \cdot t$ (this is the click through rate setting where $q$ is the CTR and $t$ is advertiser's value per click).  


%\begin{question}
%What is the optimal information selling mechanism for threshold tests?
%\end{question}
\begin{question}
The above setting can be generalized to the cases where there are multiple threshold test principals in the market, and examine the equilibrium prices of threshold tests. 
\end{question}
\begin{question}
The above setting can be generalized to cases where there is also the product seller in the market who knows $q$. However, he is not trusted by the purchasing agent. He would like to turn to the principal to choose a threshold test for his product. In this case, what is the principal's optimal mechanism. 

What if the buyer also does not know the quality of his product, but may have a better distribution, i.e., an additional signal about $q$?
\end{question}
\begin{question}
Threshold tests happen a lot in practice, like used car inspection, house inspection, GRE test, SAT exam. In exam test, the agent has a slightly different utility function, he will get a utility $u(\theta)$ for passing a test with threshold $\theta$ and utility $0$ for not passing the test. What is the optimal threshold test pricing for such exam tests?
\end{question}

==> optimal-hf.tex <==
\section{The Optimal Mechanism}


Here we consider the case where both $t\in T = [t_1, t_2]$ and $q\in Q = [q_1, q_2]$ are continuous. Assume $q\sim G(q)$ and $t\sim F(t)$ are independent. As a useful notation, let $v(t) = \Ex_{q \sim G} v(q,t) = \int_{q \in Q} g(q) v(q,t) dq $ denote the expected utility of buyer type $t$ for taking action $1$ without any additional information. 

One special type of scheme of our interest is the threshold test scheme. 
\begin{definition}[Threshold Testing]
An information selling scheme $\{ \pi_t \}_{t\in \T}$ is a \emph{threshold testing} scheme if for any buyer type $t$, there exists a threshold $\theta_t$ such that: (1)   $\pi_t(q,1) = g(q)$ for any $q > \theta_t$; (2)   $\pi_t(q,0) = 0$ for any $q < \theta_t$. 

A threshold testing scheme is \emph{monotone} if $\theta_t \geq \theta_{t'}$ whenever $t \geq t'$. 
\end{definition}
That is, a threshold test will always recommend action 1 (purchase) whenever the quality passed the threshold $\theta_t$ and recommend action 0 (not purchasing) if the quality did not pass. Note that if the quality $q = \theta_t$, the seller is allowed to recommend action 0 or 1 randomly. The threshold testing scheme is monotone if a higher type always has a higher threshold. Note that such threshold testing are ubiquitous in reality, e.g., used car inspection, car smoke check,   house inspection, medical tests, production inspection, etc.  

Our first main conjecture is the follows. 
\begin{conjecture}
There always exists an optimal information selling mechanism that is a monotone threshold test. 
\end{conjecture}


\subsection{Problem Formulation}
An information selling scheme consists of a signaling scheme $\pi: Q \times T \to [0,1] $, where $\pi(q, t) \in [0,1]$ is the probability of recommending action $1$ at quality $q$ conditioning on buyer type $t$, and a payment function $p(t)$. The information seller's objective is thus to maximize the following objective of revenue:
\begin{equation}\label{cons:obj}
\text{ Seller's Objective: } \quad \max_{\pi, p} \int_{t\in T} f(t) p(t) dt  
\end{equation}

The mechanism $(\pi, p)$ needs to satisfy the following sets of conditions. 

The first set of constraints is the obedience constraint for the signaling scheme. That is, when action $1$ is recommended to a buyer type $t$, the expected conditional buyer utility of taking action $1$ is $ \frac{ \Ex_{q\sim G}\left[ \pi(q,t)v(q,t) \right] }{ \Ex_{q\sim G} [\pi(q,t)] }$, which should indeed be at least $0$, i.e., the utility of action $0$.  This constraint can be mathematically expressed as $\int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t) dq  \geq  0$. Conversely,  when action $0$ is recommended to a buyer type $t$, the expected conditional buyer utility of taking, again, action $1$ is $ \frac{ \Ex_{q\sim G}\left[ (1 - \pi(q,t)) \cdot v(q,t) \right] }{ \Ex_{q\sim G} [1 - \pi(q,t)] }$, which should be at most $0$. This constraint can be mathematically expressed  $\int_{q \in Q} [1- \pi(q, t)] \cdot g(q) v(q,t) dq \leq  0$ or equivalently $\int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t) dq  \geq \int_{q \in Q}  g(q) v(q,t) dq  = v(t)  $. As a consequence, the obedience constraint can be   summarized into the following constraint: 
\begin{eqnarray}\label{cons:obedience}
\text{Obedience Constraint: } \quad & & \int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t) dq \geq   \max \{ 0, v(t) \}, \, \, \, \forall t \in [T]
\end{eqnarray}

The second set of constraint is the incentive compatibility (IC) constraint. That is, each buyer type $t$ has no incentive to misreport any other type $t'$. Note that, given any obedient signaling scheme, the expected utility of buyer type $t$ from the scheme, under truthful reporting,  is $\int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t)$. Therefore, the IC  constraint can be expressed as follows:
\begin{equation}\label{cons:IC}
\text{IC Constraint: } \quad \int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t) dq - p(t) \geq \int_{q \in Q} \pi(q, t') \cdot g(q) v(q,t) dq  - p(t'), \, \, \, \forall, t, t' \in [T] 
\end{equation}

Our last set of constraint is the individual rationality (IR) constraint, expressed as follows. 
\begin{equation}\label{cons:IR}
    \text{IR Constraint: } \quad \int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t) dq - p(t) \geq  \max \{ 0, v(t) \}, \, \, \, \forall, t  \in [T]  
\end{equation} 

Therefore, the seller's optimization problem is to find feasible mechanism $(\pi, p)$ to maximize Objective \eqref{cons:obj} subject to Constraints \eqref{cons:obedience}, \eqref{cons:IC} and \eqref{cons:IR}. Note that the payment function $p(t)$ is allowed to be negative for now (\todo{cite previous papers}), though as we shall see later that at optimality it will always be non-negative. The key difference of selling information and classic single-item auction design is that the buyer utility is the expected utility over the item quality whereas the buyer's utility in single-item auction is the expected utility over other bidders' values. Moreover, we have an additional constraint, i.e., the obedience constraint.  \todo{add discussions here}.   

\subsection{Feasible Mechanisms}
We now characterize the set of \emph{feasible mechanisms} that satisfy Constraints  \eqref{cons:obedience}, \eqref{cons:IC} and \eqref{cons:IR}. Observe that the obedience constraint and the IR constraint differ only by the payment term. However, neither of them implies the other because it is not clear that whether the payment function is always non-negative or not. \todo{explain why this is not obviously true}  Our first step is to get rid of the Obedience constraints by proving that there always exists an optimal mechanism that has non-negative payment for any type $t$.
\begin{lemma}\label{lem:positive-pay}
There exists an optimal IC, IR and obedient mechanism in which $p(t) \geq 0$ for all $t \in T$.
\end{lemma}
\begin{proof}
Let $(\bar{\pi}, \bar{p})$ be any IC, IR and obedient optimal mechanism. We construct a different mechanism $(\pi^*, p^)$ which  satisfies the same constraints and remains optimal but $p^*(t) \geq 0$ for any $t$. For convenience, we divide the buyer types into two sets: $T^+ = \{ t\in [T]: \bar{p}(t) \geq 0 \}$ is the set of types who have non-negative payments in mechanism  $(\bar{\p}, \bar{p})$ and $T^- = T \setminus T^+$ is the set of types who have negative payment. 

The $(\pi^*, p^)$ is constructed from $(\bar{\pi}, \bar{p})$ as follows: 
\begin{enumerate}
    \item  The mechanism for any $t \in T^+$ remains the same: for any $t\in T^+$,  let $p^*(t) = \bar{p}(t)$ and $\pi^*(q,t) = \bar{\pi}(q, t)$ for all $q \in Q$;
    \item The mechanism for any $t \in T^-$ becomes no information and no payment:  for any $t \in T^-$, let $p^*(t) = 0$, and  $\pi^*(q,t) = 1$ for all $q \in Q$ if if $v(t) \geq 0$ and  $\pi^*(q,t) = 0$ for all $q \in Q$ if $v(t) \leq  0$
\end{enumerate} 
So far, the constructed mechanism $(\pi^*, p^)$ has three useful properties: (1) it yields revenue at least that of $(\bar{\pi}, \bar{p})$ by construction; (2) all the buyer types' payments are non-negative now; (3) Individual rationality constraint is satisfied at every buyer type. The third property follows from the construction: the utility of any buyer type $t \in T^+$ did not change and the utility of a type $t \in T^-$ now pays $0$ and receives no information (i.e., always being recommended action 1 or 0, depending on $v(t) \geq 0$ or not), so IR constraint is always  satisfied.   

However, the major issue with the constructed mechanism $(\pi^*, p^*)$ above is that it is not incentive compatible, i.e., bidder type $t$ may want to misreport $t'$. We first argue that the IC constraint for any $t \in T^+$ is already satisfied. First of all, any type $t \in T^+$ would not have incentive to deviate to another type $t' \in T^+$ due to the original IC constraint of $(\bar{\pi}, \bar{p})$ and the fact that the mechanism for types in $T^+$ remains the same. We claim that any type $t \in T^+$ would not have incentive to deviate to a type $t'$ in $T^-$ as well. This is because the information for $t' \in T^-$ is less (since revealing no information) and the payment is more (since $p^*(t') = 0 > \bar{p}(t')$). Therefore, if in mechanism $(\bar{\pi}, \bar{p})$ the buyer type $t$ does not have incentives to deviate to $t'$, it remains to be true for $(\pi^*, p^*)$.  

However, buyer type $t \in T^_$ may indeed have incentive to deviate to some type $t' \in T^+$ since they want to receive beneficial information under some amount of payment.  Here comes our last step of the construction --- adjusting  the above $(\pi^*, p^*)$  to make any type $t \in T^-$ to also satisfy IC without decreasing the revenue neither violates the IR and obedient constraint.  To do so, for any $t \in T^-$, let $t' \in T^+$ be the most profitable deviation of type $t$, i.e., the deviation that maximize type $t$'s utility. We adjust $(\pi^*, p^*)$ simply by adopting the scheme of type $t'$ to the type $t$ --- i.e.,  resetting $\pi^*(t) = \bar{\pi}(t')$ and $p^*(t) = \bar{p}(t')$. After such adjustment, the IC constraint for any type $t \in T^-$ are satisfied by construction because each of these types has indeed their most profitable mechanism. Meanwhile, this will also maintain the IC constraint for any type $t \in T^+$ since the adjustment did not adding more menus. Note that IR constraints remains satisfied since the utility of any type $t \in T^+$  is non-decreasing int his adjustment. The revenue did not decrease as the payment $p^*(t)$ did not decrease in our adjustment for any $t \in T^+$. The only non-obvious part to verify is the obedience constraint. Indeed, the obedience constraints may be violated for type $t \in T^-$ during this adjustment since the  recommended optimal action for the $t' \in T^+$ might not be optimal for $t$. To achieve obedience, we simply ``rename" the recommended action for $t$ to indeed be his optimal action. This restores the obedience constraint for $t$. Noe that, this will either not change the revealed information or lead to less revealed information (when type $t$'s optimal action are the same under $\bar{\pi}(\cdot, t')$), and thus will not hurt the IC constraints.  
\end{proof}

As a consequence of Lemma \ref{lem:positive-pay}, we will henceforth restrict out design space to the mechanisms which only uses non-negative payments. For these mechanisms, we can safely omit the obedience constraint \eqref{cons:obedience}. We start by analyzing the IC Constraints. First,  Constraint \eqref{cons:IC} can be re-arranged as follows:
\begin{equation*}
\int_{q \in Q} [\pi(q, t) - \pi(q, t')] \cdot g(q) v(q,t)  dq\geq p(t)  - p(t'), 
\end{equation*}
Therefore, the IC constraint implies the following two inequalities about any two types $t, t'$: 
\begin{gather}
\int_{q \in Q} [\pi(q, t) - \pi(q, t')] \cdot g(q) v(q,t) dq \geq  p(t)  - p(t'), \label{eq:ic1}\\
\int_{q \in Q} [\pi(q, t') - \pi(q, t)] \cdot g(q) v(q,t') dq \geq  p(t')  - p(t).\label{eq:ic2}
\end{gather}

Combining Inequality \eqref{eq:ic1} and \eqref{eq:ic2}, we obtain the following constraint for any pair of types $t, t'$:
\begin{gather*}
\int_{q \in Q} [\pi(q, t') - \pi(q, t)] \cdot g(q) v(q,t) dq \leq p(t')  - p(t) \leq \int_{q \in Q} [\pi(q, t') - \pi(q, t)] \cdot g(q) v(q,t') dq . 
\end{gather*} 

\hf{I think this approach only works when $v(q,t)$ is a linear function of $t$, i.e., $v(q,t) = v_1(q)t + v_0$. In. the following derivations, I assumed $v(q,t) = v_1(q)t + v_0(q)$. }

Therefore, the right-hand side of the above inequality must be at least its left-hand side. This implies the following \emph{necessary condition} for any IC information selling mechanism $(\pi, p)$. That is, for any $t, t' \in T$, we have 
\begin{eqnarray*}
0 &\leq&  \int_{q \in Q} [\pi(q, t') - \pi(q, t)] \cdot g(q) [v(q,t') - v(q, t)]dq \\ 
& = &  \int_{q \in Q} [\pi(q, t') - \pi(q, t)] \cdot g(q) v_1(q)[ t' - t]dq   
\end{eqnarray*}
Define $$   Q(t) = \int_{q \in Q}  \pi(q, t) \cdot g(q) v_1(q)dq. $$ A simple case analysis for $t' > t$ or $t' < t$ implies that the above inequality is equivalent to  $Q(t)$ is monotone non-decreasing in $t$. Note that $Q(t)$ can be interpreted as the expected \emph{weighted} probability of being recommended action $1$, where the weights are $v_1(q)$ and indicate the significance of buyer type $t$ in his value function. 
%To interpret Equation \eqref{eq:signal_monotone}, note that if we fix a quality $q$, the inequality $[\pi(q, t') - \pi(q, t)] \cdot g(q) [v(q,t') - v(q, t)] \geq 0$ means if the value of buyer type $t'$ is larger (i.e., $v(q,t') \geq  v(q, t)$), then his probability of being recommended action $1$ is also higher (i.e., $\pi(q, t') \geq  \pi(q, t)$ ).  Therefore, Equation \eqref{eq:signal_monotone}  can be interpreted as the enforcement of such monotonicity on average over the random choice of the quality. 
We thus term this the \emph{signaling monotonicity}. Note that this is similar to Myerson's allocation monotonicity condition as in auction design, but is different. \todo{cite and add discussions here} 

We now derive a relation between signaling scheme $\pi$ and payment rule $p$ for any IC mechanism. We start by deriving the buyer's utility. Note that any buyer of type $t$ will derive non-zero utilities only from the action recommendation of $1$ since an action recommendation of $0$ will lead to buyer utility $0$. Therefore, a buyer of type $t$ has the following utility:  
\begin{gather*}
\text{Utility of Buyer Type }t: \quad u(t)= \int_{q \in Q} \left[ g(q) \pi(q,t)v(q,t) \right] dq -p(t)
\end{gather*}

Re-arranging Inequality \eqref{eq:ic1}, we have 
\begin{eqnarray*}
 u(t) &=& \int_{q \in Q} \left[ g(q) \pi(q,t)v(q,t) \right] dq -p(t) \\
 &\geq& \int_{q \in Q} \left[ g(q) \pi(q,t')v(q,t) \right] dq -p(t')  & \mbox{by Ineq. \eqref{eq:ic1}} \\
 &=& \int_{q \in Q} \left[ g(q) \pi(q,t')v(q,t) \right] dq + u(t') - \int_{q \in Q} \left[ g(q) \pi(q,t')v(q,t') \right] dq & \mbox{Def of $u(t')$}\\ 
 &=& \int_{q \in Q} \left[ g(q) \pi(q,t')[ v(q,t) - v(q, t')]  \right] dq + u(t')  & \mbox{Algebraic Manipulation}\\ 
 &=& (t-t') Q(t') + u(t')  & \mbox{Def. of $Q(t)$ and $v(q,t)$}\\   
\end{eqnarray*}

As a consequence, Inequality \eqref{eq:ic1} implies  $u(t) -u(t') \geq (t-t')Q(t') $. Together with a similar derivation from Inequality \eqref{eq:ic2}, we thus have the following inequality 
\begin{gather*}
(t-t') Q(t')  \le u(t)-u(t')\le (t-t') Q(t).
\end{gather*}
Note that the above inequality holds for any $t, t'$. Therefore, by letting $t' \to t$ from the left side and dividing all terms simultaneously by $t - t'$, we obtain the following identify about $u(t)$: \todo{we made differentiability assumption of $u(t)$}
\begin{gather}\label{eq:buyer-utility-identify1}
\odv{u(t)}{t}= Q(t)
\end{gather}
Note that, when $t' \to t$ from the right side, we shall obtain the same identify as \eqref{eq:buyer-utility-identify1}. 
Note that both the signaling monotonicity and the payment payment identify are the necessary outcomes of the incentive compatibility constraints, more precisely, the outcome of Constraints \eqref{eq:ic1} and \eqref{eq:ic2}. Next, we show that these two conditions are also sufficient.  
\begin{lemma}\label{lem:feasible-M}
A mechanism $(\pi, p)$ is feasible if and only if it satisfies the following constraints:
\begin{eqnarray}\label{eq:signal-monotonicity}
&& Q(t) \text{ is monotone non-decreasing in } t \\\label{eq:buyer-utility-identify2}
&& u(t) = u(t_1) + \int_{t_1}^{t} Q(x)  dx, \, \, \, \forall t \in [T] \\\label{eq:ir-t2}
& & u(t_2) \geq v(t_2), \, \, \, u(t_1) \geq 0 \\ \label{eq:non-negativity}
& & p(t) \geq 0,  \, \, \forall t \in [T]. 
 \end{eqnarray}
\end{lemma}



\begin{proof}
The necessity of these constraints come from the above derivation and the IR constraint for type $t_2$. We now prove that they are sufficient.  That is, Constraint \eqref{eq:signal-monotonicity}-\eqref{eq:non-negativity} implies Obedience, IC and IR constraints \eqref{cons:obedience}, \eqref{cons:IC} and \eqref{cons:IR}. 

IC constraint \eqref{cons:IC} is equivalent to 
\begin{equation*}
     u(t) \geq u(t') + \int_{q_1}^{q_2} \pi(q, t') \cdot g(q) [v(q,t) - v(q,t')] dq = u(t') + (t-t') Q(t'). 
\end{equation*}
Therefore Constraint \eqref{eq:signal-monotonicity} and \eqref{eq:buyer-utility-identify2} implies IC constraint \eqref{cons:IC} because if $t' < t$ we have 
\begin{equation*}
     u(t) - u(t') = \int_{t'}^{t} Q(x)  dx \geq \int_{t'}^{t} Q(t')  dx = (t-t')Q(t'). 
\end{equation*}
Similarly, when $t' > t$, we also have $    u(t) - u(t') \geq  (t-t')Q(t'). $ 

The IR constraint \eqref{cons:IR} is equivalent to $u(t) \geq 0$ and $u(t) \geq v(t)$. Since $Q(x)\geq 0$, Constraint \eqref{eq:buyer-utility-identify2}, together with $u(t_1) \geq 0$, implies $u(t) \geq 0$ for any $t$. We now leverage $u(t_2) \geq v(t_2)$ to prove that  $u(t) \geq v(t)$ also holds, as follows:
\begin{eqnarray*}
u(t) &=&  u(t_1) + \int_{t_1}^{t} Q(x)  dx  \\
& = &  u(t_2) - \int_{t}^{t_2} Q(x)  dx  \\
& \geq  &  v(t_2)  - \int_{t}^{t_2} Q(x)  dx  \\
& =   &   \int_{q_1}^{q_2} g(q) [v_1(q)t_2 + v_0(q)]dq  - \int_{t}^{t_2}   \int_{q_1}^{q_2}  \pi(q, x) \cdot g(q) v_1(q)dq  dx  \\
& \geq  &   \int_{q_1}^{q_2} g(q) [v_1(q)t_2 + v_0(q)]dq  - \int_{t}^{t_2}   \int_{q_1}^{q_2}   g(q) v_1(q)dq  dx  \\
& =  &   \int_{q_1}^{q_2} g(q) [v_1(q)t + v_0(q)]dq  = v(t) \\
\end{eqnarray*}

Finally, the Obedience constraint \eqref{cons:obedience} follows from IR constraint \eqref{cons:IR} and $p(t) \geq 0$. 

\end{proof}


\hf{
For general $v(q,t)$, the lemma is the following, which I do not know how to prove 

\begin{lemma}\label{lem:feasible-M}
A mechanism $(\pi, p)$ is feasible if and only if it satisfies the following constraints:
\begin{eqnarray}\label{eq:signal-monotonicity}
&& \int_{q_1}^{q_2} g(q) [\pi(q,t) - \pi(q,t')][v(q,t) - v(q,t')] \geq 0 \\\label{eq:buyer-utility-identify2}
&& u(t) = u(t_1) + \int_{q_1}^{q_2}\int_{t_1}^{t}  g(q) \pi(q,x) \frac{\partial v(q,x)}{\partial x}  dx, \, \, \, \forall t \in [T] \\\label{eq:ir-t2}
& & u(t_2) \geq v(t_2) \\ \label{eq:non-negativity}
& & p(t) \geq 0, \, u(t) \geq 0 \, \, \, \forall t \in [T]
 \end{eqnarray}
\end{lemma}
\begin{proof}

An equivalence to Condition (20) is the 
\begin{equation}
p'(t) =  \int_{q_1}^{q_2}  g(q) \frac{\partial \pi(q,t)}{\partial t}  v(q,t)    dq, \, \, \, \forall t \in [T] 
\end{equation}
This comes from the definition of $u(t):$
\begin{equation}
u(t) =  \int_{q_1}^{q_2}  g(q)  \pi(q,t)  v(q,t)    dq - p(t), \, \, \, \forall t \in [T] 
\end{equation}





Therefore, the IC constraint is equivalent to 
\begin{eqnarray}
&& \int_{t'}^t \int_{q_1}^{q_2} \left[ g(q) \pi(q,s) \frac{\partial v(q,s)}{\partial s}   \right] dq  ds \geq \int_{q_1}^{q_2} \pi(q, t') \cdot g(q) [v(q,t) - v(q,t')] dq \\
&\Longleftrightarrow&  \int_{q_1}^{q_2} g(q) \Bigg[ \int_{t'}^t  \left[ \pi(q,s) \frac{\partial v(q,s)}{\partial s}   \right] ds - \pi(q, t')  [v(q,t) - v(q,t')]  \Bigg]  dq  \geq 0 \\ 
&\Longleftrightarrow&  \int_{q_1}^{q_2} g(q) \Bigg[ \int_{t'}^t  \left[ \pi(q,s) \frac{\partial v(q,s)}{\partial s}   \right] ds - \int_{t'}^t \pi(q, t') \frac{\partial v(q,s)}{ \partial s} ds  \Bigg]  dq  \geq 0 \\  
&\Longleftrightarrow&  \int_{q_1}^{q_2} g(q) \Bigg[ \int_{t'}^t  \left[ [\pi(q,s) - \pi(q, t')] \frac{\partial v(q,s)}{\partial s}   \right] ds \Bigg]  dq  \geq 0 \\   
&\Longleftrightarrow&  \int_{q_1}^{q_2} g(q) \Bigg[   [\pi(q,s) - \pi(q, t')]v(q,s)|_{t'}^t -    \int_{t'}^t  \left[ \frac{\partial \pi(q,s)}{\partial s} v(q,s)  \right] ds     \Bigg]  dq  \geq 0 \\    
&\Longleftrightarrow&  \int_{q_1}^{q_2} g(q) \Bigg[   [ \pi(q,t) - \pi(q, t')]v(q,t) -    \int_{t'}^t  \left[ \frac{\partial \pi(q,s)}{\partial s} v(q,s)  \right] ds     \Bigg]  dq  \geq 0 \\     
&\Longleftrightarrow& \int_{q_1}^{q_2} g(q) \Bigg[  \int_{t'}^t  \left[ \frac{\partial \pi(q,s)}{\partial s} [v(q,t) - v(q,s)]  \right] ds     \Bigg]  dq  \geq 0 
\end{eqnarray} 
\end{proof}

}



\subsection{Optimizing Revenue }

Additionally, the definition of $u(t)$ gives us the following identify:
\begin{gather*}
\frac{ \partial u(t) }{\partial t}= \int_{q \in Q} g(q) \left[  \frac{\partial \pi(q,t) }{\partial t} v(q,t) + \pi(q,t) \frac{\partial v(q,t)}{\partial t} \right] dq -p'(t)
\end{gather*}
where $p'(t)$ is the derivative of the payment function $p(t)$. Plugging Identify \eqref{eq:buyer-utility-identify} into the above equality gives us the relation between the payment function $t$ and the signaling scheme $\pi$:
\begin{equation}
\text{Payment Identify: } \quad p'(t) = \int_{q \in Q} g(q)  \frac{\partial \pi(q,t) }{\partial t} v(q,t)  dq, \, \, \, \forall t \in T
\end{equation}

Revenue derivation with $t_2$ as the reference point can be expressed as follows: 
\begin{align*}
REV (\pi, p)&=\int_{t_1}^{t_2} f(t)p(t)\,\mathrm{d}t\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \left[ \pi(q,t)v(q,t)\right]  dq -u(t) \right)\,\mathrm{d}t\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q)\pi(q,t)v(q,t) dq  -u(t_2) + \int_{t}^{t_2} Q(x) \mathrm{d}x \right)\,\mathrm{d}t\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \pi(q,t)v(q,t)  dq \right)\,\mathrm{d}t + \int_{t_1}^{t_2} \int_{t}^{t_2}f(t) Q(x)\,\mathrm{d}x\,\mathrm{d}t -u(t_2)\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \pi(q,t)v(q,t)  dq \right)\,\mathrm{d}t + \int_{t_1}^{t_2} \int_{t_1}^{x}f(t) Q(x)\,\mathrm{d}t\,\mathrm{d}x -u(t_2)\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q)  \pi(q,t)v(q,t) dq \right)\,\mathrm{d}t + \int_{t_1}^{t_2} F(x)Q(x)\,\mathrm{d}x-u(t_2)\\
&=\int_{q_1}^{q_2} g(q)\left[\int_{t_1}^{t_2} f(t) \pi(q,t)v(q,t) dq \right]\,\mathrm{d}t + \int_{t_1}^{t_2} F(t)\int_{q_1}^{q_2} g(q)\left[ \pi (q,t)v_1(q) \right] \mathrm{d}q\,\mathrm{d}t-u(t_2)\\
&=\int_{q_1}^{q_2} g(q)\left[ \int_{t_1}^{t_2} f(t)\pi(q,t) \left(v(q,t)+ v_1(q)\frac{F(t)}{f(t)}\right)\,\mathrm{d}t \right] \mathrm{d}q -u(t_2)\\
&=\int_{q_1}^{q_2} g(q)\left[ \int_{t_1}^{t_2} f(t)\pi(q,t) [v_1(q) \varphi(t) + v_0(q)]\,\mathrm{d}t \right] \mathrm{d}q -u(t_2) 
\end{align*}


Revenue derivation with $\bar{t}$ as the reference point where $\bar{t}$ satisfies $\var{v}(\bar{t}) = \int_{q_1}^{q_2} v(q, \bar{t}) g(q) dq = 0$. 
\begin{align*}
REV (\pi, p)&=\int_{t_1}^{t_2} f(t)p(t)\,\mathrm{d}t\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \left[ \pi(q,t)v(q,t)\right]  dq -u(t) \right)\,\mathrm{d}t\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q)\pi(q,t)v(q,t) dq -\int_{\bar{t}}^{t} Q(x) \mathrm{d}x -u(\bar{t}) \right)\,\mathrm{d}t\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \pi(q,t)v(q,t)  dq \right)\,\mathrm{d}t-\int_{t_1}^{t_2} \int_{\bar{t}}^{t}f(t) Q(x)\,\mathrm{d}x\,\mathrm{d}t -u(\bar{t})\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q)  \pi(q,t)v(q,t) dq \right)\,\mathrm{d}t+ \int_{t_1}^{\bar{t}} F(x)Q(x)dx - \int_{\bar{t}}^{t_2} (1-F(x))Q(x)\,\mathrm{d}x-u(\bar{t})
\end{align*}


{\color{red}
\begin{align*}
\int_{\bar{t}}^{t_2} f(t)p(t)\,\mathrm{d}t&=\int_{\bar{t}}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \left[ \pi(q,t)v(q,t)\right]  dq -u(t) \right)\,\mathrm{d}t\\
&=\int_{\bar{t}}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q)\pi(q,t)v(q,t) dq -\int_{\bar{t}}^{t} Q(x) \mathrm{d}x -u(\bar{t}) \right)\,\mathrm{d}t\\
&=\int_{\bar{t}}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \pi(q,t)v(q,t)  dq \right)\,\mathrm{d}t-\int_{\bar{t}}^{t_2} \int_{\bar{t}}^{t}f(t) Q(x)\,\mathrm{d}x\,\mathrm{d}t -u(\bar{t})\\
&=\int_{\bar{t}}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \pi(q,t)v(q,t)  dq \right)\,\mathrm{d}t-\int_{\bar{t}}^{t_2} \int_{x}^{t_2}f(t) Q(x)\,\mathrm{d}t\,\mathrm{d}x -u(\bar{t})\\
&=\int_{\bar{t}}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q)  \pi(q,t)v(q,t) dq \right)\,\mathrm{d}t-\int_{\bar{t}}^{t_2} (1-F(x))Q(x)\,\mathrm{d}x-u(\bar{t})\\
&=\int_{q_1}^{q_2} g(q)\left[\int_{\bar{t}}^{t_2} f(t) \pi(q,t)v(q,t) dq \right]\,\mathrm{d}t-\int_{\bar{t}}^{t_2} (1-F(t))\int_{q_1}^{q_2} g(q)\left[ \pi (q,t)v_1(q) \right] \mathrm{d}q\,\mathrm{d}t-u(\bar{t})\\
&=\int_{q_1}^{q_2} g(q)\left[ \int_{\bar{t}}^{t_2} f(t)\pi(q,t) \left(v(q,t)-v_1(q)\frac{1-F(t)}{f(t)}\right)\,\mathrm{d}t \right] \mathrm{d}q -u(\bar{t})\\
&=\int_{q_1}^{q_2} g(q)\left[ \int_{\bar{t}}^{t_2} f(t)\pi(q,t) [v_1(q) \varphi(t) + v_0(q)]\,\mathrm{d}t \right] \mathrm{d}q -u(\bar{t}) 
\end{align*}
}
where $\varphi(t) = t + \frac{F(t)}{f(t)}$ is the called the \emph{virtual value} for type $t$.  


Revenue derivation with $t_1$ as the reference point: 
\begin{align*}
REV (\pi, p)&=\int_{t_1}^{t_2} f(t)p(t)\,\mathrm{d}t\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \left[ \pi(q,t)v(q,t)\right]  dq -u(t) \right)\,\mathrm{d}t\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q)\pi(q,t)v(q,t) dq -\int_{t_1}^{t} Q(x) \mathrm{d}x -u(t_1) \right)\,\mathrm{d}t\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \pi(q,t)v(q,t)  dq \right)\,\mathrm{d}t-\int_{t_1}^{t_2} \int_{t_1}^{t}f(t) Q(x)\,\mathrm{d}x\,\mathrm{d}t -u(t_1)\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q) \pi(q,t)v(q,t)  dq \right)\,\mathrm{d}t-\int_{t_1}^{t_2} \int_{x}^{t_2}f(t) Q(x)\,\mathrm{d}t\,\mathrm{d}x -u(t_1)\\
&=\int_{t_1}^{t_2} f(t)\left(\int_{q_1}^{q_2} g(q)  \pi(q,t)v(q,t) dq \right)\,\mathrm{d}t-\int_{t_1}^{t_2} (1-F(x))Q(x)\,\mathrm{d}x-u(t_1)\\
&=\int_{q_1}^{q_2} g(q)\left[\int_{t_1}^{t_2} f(t) \pi(q,t)v(q,t) dq \right]\,\mathrm{d}t-\int_{t_1}^{t_2} (1-F(t))\int_{q_1}^{q_2} g(q)\left[ \pi (q,t)v_1(q) \right] \mathrm{d}q\,\mathrm{d}t-u(t_1)\\
&=\int_{q_1}^{q_2} g(q)\left[ \int_{t_1}^{t_2} f(t)\pi(q,t) \left(v(q,t)-v_1(q)\frac{1-F(t)}{f(t)}\right)\,\mathrm{d}t \right] \mathrm{d}q -u(t_1)\\
&=\int_{q_1}^{q_2} g(q)\left[ \int_{t_1}^{t_2} f(t)\pi(q,t) [v_1(q) \varphi(t) + v_0(q)]\,\mathrm{d}t \right] \mathrm{d}q -u(t_1) 
\end{align*}

\begin{align*} 
\max_{\pi} & \int_{t_1}^{t_2}  \int_{q_1}^{q_2} \left[ g(q) \pi(q,t) f(t)[v_1(q) \varphi(t) + v_0(q)]\,\mathrm{d}t \right] \mathrm{d}q \\
\text{subject to} & \int_{t_1}^{t_2} \int_{q_1}^{q_2} g(q) \pi(q,t) v_1(q) dq dt \geq \int_{q_1}^{q_2} g(q) v(q,t_2) dq\\
& Q(t) \text{ monotonoe in }t
\end{align*}
\begin{lemma}
There exists a threshold mechanism that solves the above mathematical program optimally if $\frac{v_0(q)}{v_1(q)}$ is increasing in $q$.
\end{lemma}
\begin{proof}
    To prove the lemma, we show that for any feasible solution to the above program, there exists a feasible threshold mechanism that weakly increases the objective function.
    
    Given a feasible mechanism $\pi(q, t)$, let $q^*(t)$ be
    \begin{gather*}
    q^*(t)=\argmin_{q^*}\left\{q^*\,\left|\, \int_{q^*}^{q_2}g(q)v_1(q)\,\mathrm{d}q=Q(t)=\int_{q_1}^{q_2}g(q)\pi(q,t)v_1(q)\,\mathrm{d}q\right.\right\}.
    \end{gather*}
    $q^*(t)$ always exists, since the function $\int_{q^*}^{q_2}g(q)v_1(q)\,\mathrm{d}q$ is continuous and decreasing in $q^*$, and
    \begin{gather*}
    \int_{q_2}^{q_2}g(q)v_1(q)\,\mathrm{d}q=0\le Q(t)\le \int_{q_1}^{q_2}g(q)v_1(q)\,\mathrm{d}q.
    \end{gather*}
    
    Define a new allocation function as follows:
    \begin{gather*}
    \pi'(q,t)=
    \begin{cases}
    1 & \text{ if } q\ge q^*(t)\\
    0 & \text{ otherwise}
    \end{cases}.
    \end{gather*}
    It is clear that the corresponding $Q(t)$ function is the same as the original $\pi(q,t)$:
    \begin{gather}
    Q'(t)=\int_{q_1}^{q_2}g(q)\pi'(q,t)v_1(q)\,\mathrm{d}q=\int_{q^*(t)}^{q_2}g(q)v_1(q)\,\mathrm{d}q=Q(t).
    \label{eq:Q_equal}
    \end{gather}
    Moreover, the left-hand-side of the first constraint
    \begin{gather*}
    \int_{t_1}^{t_2} \int_{q_1}^{q_2} g(q) \pi(q,t) v_1(q)\, \mathrm{d}q \mathrm{d}t=\int_{t_1}^{t_2}Q(t)\,\mathrm{d}t
    \end{gather*}
    also remains the same. The above two equations imply that $\pi'(q,t)$ is also feasible. Now it suffices to show that $\pi'(q,t)$ leads to a higher revenue. The proof is immediate if we notice that the original program is very similar to the fractional knapsack problem. However, we still include a proof here to make it self-contained.
    
    Define
    \begin{gather*}
    \Phi(q, t) = f(t)\left[ \varphi(t)+\frac{v_0(q)}{v_1(q)} \right].
    \end{gather*}
    $\Phi(q,t)$ is monotone increasing in $q$ since $\frac{v_0(q)}{v_1(q)}$ is increasing and $f(t)$ is always non-negative. Thus if $q\ge q^*(t)$, $\pi'(q,t)=1\ge \pi(q,t)$, and $\Phi(q,t)\ge \Phi(q^*(t),t)$, and if $q< q^*(t)$, $\pi'(q,t)=0\le \pi(q,t)$, and $\Phi(q,t)\le \Phi(q^*(t),t)$. Therefore,
    \begin{gather}
    \left[ \pi'(q,t)-\pi(q,t) \right]\left[ \Phi(q,t)-\Phi(q^*(t),t) \right]\ge 0, \forall q, t. \label{eq:monotone}
    \end{gather}
    The revenue difference of the two mechanisms $\pi(q,t)$ and $\pi'(q,t)$ is:
    \begin{align*}
    &\int_{t_1}^{t_2}  \int_{q_1}^{q_2} g(q) \left[\pi'(q,t)-\pi(q,t)\right] f(t)[v_1(q) \varphi(t) + v_0(q)]\,\mathrm{d}q \mathrm{d}t\\
    =&\int_{t_1}^{t_2}  \int_{q_1}^{q_2} g(q) \left[\pi'(q,t)-\pi(q,t)\right] v_1(q)\Phi(q,t)\,\mathrm{d}q \mathrm{d}t\\
    \ge&\int_{t_1}^{t_2}  \int_{q_1}^{q_2} g(q) \left[\pi'(q,t)-\pi(q,t)\right] v_1(q)\Phi(q^*(t),t)\,\mathrm{d}q \mathrm{d}t\\
    =&\int_{t_1}^{t_2} \Phi(q^*(t),t) \int_{q_1}^{q_2} g(q) \left[\pi'(q,t)-\pi(q,t)\right] v_1(q)\,\mathrm{d}q \mathrm{d}t\\
    =&\int_{t_1}^{t_2} \Phi(q^*(t),t) \left[Q'(t)-Q(t)\right]\, \mathrm{d}t\\
    =&0,
    \end{align*}
    where the inequality is because of Equation \eqref{eq:monotone} and the last equation is due to Equation \eqref{eq:Q_equal}.
\end{proof}
% \begin{lemma}
% The solution to the above mathematical program is a threshold mechanism if the following function is monotone increasing in both $t$ and $q$:
% \begin{gather*}
%     \Phi(q, t) = f(t)\left[ \varphi(t)+\frac{v_0(q)}{v_1(q)} \right].
% \end{gather*}
% \end{lemma}
% \begin{remark}
% The above condition is also equivalent to the following two conditions:
% \begin{itemize}
%     \item $\frac{v_1(q)}{v_0(q)}$ is increasing in $q$;
%     \item $\frac{f'(t)}{f(t)}\frac{v(q,t)}{v_1(q)}\ge -2$.
% \end{itemize}
% \end{remark}
% To prove this result, we first relax the second constraint and show that the solution to the relaxed program is a special class of allocation rules. Then we prove that the this special class of rules automatically satisfies the second constraint.
% \begin{proof}
% % Let
% % \begin{gather*}
% %     D_+=\{(t, q)\mid v_1(q)\varphi(t)+v_0(q)\ge 0\},\\
% %     D_-=\{(t, q)\mid v_1(q)\varphi(t)+v_0(q)< 0\}.
% % \end{gather*}
% % Thus the objective function can be written as:
% % \begin{gather*}
% %     \left(\int_{D_+}-\int_{D_-}\right)g(q)\pi(q,t)f(t)|v_1(q)\varphi(t)+v_0(q)|\,\mathrm{d}t\mathrm{d}q.
% % \end{gather*}

% Let's relax the second constraint first. Similar to the fractional knapsack problem, the optimal solution to the relaxed program is to ``sort'' the ratio
% \begin{gather*}
%     \frac{g(q) \pi(q,t) f(t)[v_1(q) \varphi(t) + v_0(q)]}{g(q) \pi(q,t) v_1(q)}=\Phi(q, t)
% \end{gather*}
% in descending order and set $\pi(q, t)=1$ greedily until the first constraint is satisfied. Therefore, the solution to the relaxed program must have the following format: 
% \begin{gather}
%     \pi_h(q, t)=
%     \begin{cases}
%     1 & \text{~if~} \Phi(q, t) \ge h\\
%     0 & \text{~otherwise}
%     \end{cases},
% \end{gather}
% where $h$ is a parameter.

% Now we show that the above class of allocation rules also satisfies the second constraint. Consider the function $\underline{q}(t|h)=\inf\{q\mid \Phi(q, t)\ge h\}$. It is easy to see that when $\Phi(q, t)$ is increasing in both $t$ and $q$, $\underline{q}(t|h)$ is always a decreasing function for all $h$, and that $\pi_h(q, t)=1$ for all $\underline{q}(t|h)\le q\le q_2$. We claim that the corresponding $Q(t)$ is monotone in $t$. This is because for any $t<t'$,
% \begin{align*}
%     Q(t')-Q(t)&=\int_q\pi_h(q,t')g(q)v_1(q)\,\mathrm{d}q-\int_q\pi_h(q,t)g(q)v_1(q)\,\mathrm{d}q\\
%     &=\int_{\underline{q}(t'|h)}^{q_2}g(q)v_1(q)\,\mathrm{d}q-\int_{\underline{q}(t|h)}^{q_2}g(q)v_1(q)\,\mathrm{d}q\\
%     &=\int_{\underline{q}(t'|h)}^{\underline{q}(t|h)}g(q)v_1(q)\,\mathrm{d}q\\
%     &\ge 0,
% \end{align*}
% where the inequality comes from the fact that $\underline{q}(t|h)$ is a decreasing function.

% Also, $\pi_h(q, t)$ gives a threshold mechanism because $\pi_h(q, t)=1$ for all $\underline{q}(t|h)\le q\le q_2$.
% \end{proof}

\subsection{The Case with Regular $F$ and Non-negative $v_1(q) $} 
When $v_1(q) \geq 0$, we know that $Q(t) \geq 0$ for all $t$. The minimum value of $u(t_2)$ is $\max \{ 0, v(t_2) \}$. Therefore, the maximum possible value of  $REV (\pi, p)$ will be achieved by setting $u(t_2) = \max \{ 0, v(t_2) \}$ and $\pi(q,t) = 1$ whenever $v_1(q) \varphi(t) + v_0(q) \geq 0$ and $\pi(q,t) = 0$ otherwise. What remains to verify is that this mechanism does satisfy all the conditions in Lemma \ref{lem:feasible-M}. 

Since $v_1(q) \varphi(t) + v_0(q)$ is monotone increasing in $t$ when $F$ is regular and $v_1(q) \geq 0$. The $\pi$ above is a \emph{threshold signaling scheme} which signals $1$ to buyer type $t$ whenever \hf{need to assume $- \frac{ v_0(q)}{v_1(q) } $ is decreasing in $q$}   
\begin{equation}
     - \frac{ v_0(q)}{v_1(q) }   \leq \varphi(t) 
\end{equation}
Since $- \frac{ v_0(q)}{v_1(q) } $ is decreasing in $q$ and $\varphi(t)$ is increasing in $t$, there exists a threshold $\theta(t)$ such that $\pi(q,t) = 1$ for any $q \geq \theta(t)$ and $\pi(q,t)=0$ otherwise. Moreover, $\theta(t)$ is decreasing in $t$. This can equivalently be viewed as a therhsold mechanism on $t$ where $\pi(q,t) = 1$ whenever $t \geq \beta{q}$ where $\beta(q)$ is now an increasing function in $q$. In fact, $\beta(q)$ minimize function $U(t;q) = F(t)v(q,t) = F(t)[v_1(q)t + v_0(q) ] $. We have $U'(t;q) = f(t)[v_1(q)t + v_0(q) ] + F(t) v_1(q) = f(t) [v_1(q) \varphi(t) + v_0(q)]$ which is positive for $t \geq \beta(q)$ and negative otherwise. Thus, $\beta(q)$ minimizes $U(t;q)$. 


It is easy to verify such a threshold policy satisfy monotonicity. We only need to guarantee $u(t_1) \geq 0$, or equivalently $p(t_1) \leq \int_{q_1}^{q_2} g(q) \pi(q,t_1) v(q,t_1) dq = B_{t_1}$, and $u(t_2) \geq v(t_2)$, or equivalently $p(t_2) \leq \int_{q_1}^{q_2} g(q) \pi(q,t_2) v(q,t_2) dq - \int_{q_1}^{q_2} g(q) v(q,t_2) dq =B_{t_2}$.  Note that $p(t_2) - p(t_1) = \int_{t_1}^{t_2} p'(t)dt$ which only depends on the signaling scheme $\pi$. Therefore, we would like to figure which of the upper band is tight.

Note that
\begin{eqnarray}
p(t) = \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq  - \int_{t_1}^{t} Q(t) dt  - u(t_1) 
\end{eqnarray}

Therefore,
\begin{eqnarray}
p(t_2) - p(t_1) = \int_{q_1}^{q_2} g(q) \pi(q,t_2) v(q,t_2) dq - \int_{q_1}^{q_2} g(q) \pi(q,t_1) v(q,t_1) dq   - \int_{t_1}^{t_2} Q(t) dt
\end{eqnarray}
\begin{eqnarray}
B_{t_2} - B_{t_1} = \int_{q_1}^{q_2} g(q) \pi(q,t_2) v(q,t_2) dq - \int_{q_1}^{q_2} g(q) \pi(q,t_1) v(q,t_1) dq  - \int_{q_1}^{q_2} g(q) v(q,t_2) dq 
\end{eqnarray}
Therefore, it remains to compare $\int_{q_1}^{q_2} g(q) v(q,t_2) dq = v(t_2)$ and $\int_{t_1}^{t_2} Q(t) dt$. 

The following claim illustrate the fundamental difficulty in this optimization. When using $t_2$ as the basis, we know $u_1 = 0$ is guaranteed, thus $u_2$ will be changed when we adjust $\pi$ to achieve obedience. How to change $\pi$ to maximize the Rev function on page 9 with $u(t_2)$, which also depend on $\pi$. Conversely, if we use $t_1$ as basis, we know $u(t_2) = v(t_2)$ and $u(t_1)$ will change and we face the same difficulty. Myerson does not have this problem since in his problem $u(t_1) = 0$ for sure and he does not need to adjust the $\pi$. 
\begin{claim}
$p(t_2) - p(t_1) \leq B_{t_2} - B_{t_1} $ when using $t_1$ as basis and $p(t_2) - p(t_1) \geq B_{t_2} - B_{t_1} $ when using $t_2$ as basis. 
\end{claim}
\begin{proof}
Let $\beta(q)$ denote the threshold for $t$. We have 
\begin{eqnarray}
& & p(t_2) - p(t_1)  - [B_{t_2} - B_{t_1}] \\
& = & \int_{q_1}^{q_2} g(q) v(q,t_2) dq  - \int_{t_1}^{t_2} Q(t) dt \\
&=& \int_{q_1}^{q_2} g(q) v(q,t_2) dq - \int_{t_1}^{t_2} \int_{q_1}^{q_2} g(q) \pi(q,t) v_1(q) dq dt \\ 
&=& \int_{q_1}^{q_2} g(q) v(q,t_2) dq - \int_{q_1}^{q_2} g(q) (t_2 - \beta(q)) v_1(q) dq \\
&=& \int_{q_1}^{q_2} g(q) [v_1(q)t_2 + v_0(q)] dq - \int_{q_1}^{q_2} g(q) (t_2 - \beta(q)) v_1(q) dq \\
&=& \int_{q_1}^{q_2} g(q) [v_1(q)\beta(q) + v_0(q)] dq 
\end{eqnarray}
because $v_1(q)\beta(q) + v_0(q) \leq 0$ for any $q$ when using $u_2$ as basis on Page 9 and $v_1(q)\beta(q) + v_0(q) \geq 0$ for any $q$ when using $u_1$ as basis on Page 9.  
\end{proof}


\begin{eqnarray}
p(t) &=& p(t_2) - \int_{t}^{t_2} p'(x)dx   \\
&=& p(t_2) - \int_{t}^{t_2}  \int_{q_1}^{q_2}  g(q) \frac{\partial \pi(q,x)}{\partial x}  v(q,x)    dq  dx   \\
&=& p(t_2)  - \int_{q_1}^{q_2} g(q) \pi(q,t2) v(q,t_2) dq + \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq   + \int_{t}^{t_2} Q(x) dx  \\
&=&  \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} Q(x) dx - u(t_2) \\
&=&  \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} Q(x) dx  - \max\{0, v(t_2 \}) \\ 
&=&  \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} \int_{q_1}^{q_2} g(q) \pi(q,x) v_1(q) dq   dx  - \max\{0, v(t_2 \}) \end{eqnarray}

If $p(t_1) = \int_{q_1}^{q_2} g(q) \pi(q,t_1) v(q,t_1)$, then $u(t_1) = 0 $. We claim $u(t_2) \geq v(t_2)$ is also satisfied, because 
\begin{eqnarray}
p(t) &=& p(t_2) - \int_{t}^{t_2} p'(x)dx   \\
&=& p(t_2) - \int_{t}^{t_2}  \int_{q_1}^{q_2}  g(q) \frac{\partial \pi(q,x)}{\partial x}  v(q,x)    dq  dx   \\
&=& p(t_2)  - \int_{q_1}^{q_2} g(q) \pi(q,t2) v(q,t_2) dq + \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq   + \int_{t}^{t_2} Q(x) dx  \\
&=&  \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} Q(x) dx - u(t_2) \\
&=&  \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} Q(x) dx  - \max\{0, v(t_2 \}) \\ 
&=&  \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq + \int_{t}^{t_2} \int_{q_1}^{q_2} g(q) \pi(q,x) v_1(q) dq   dx  - \max\{0, v(t_2 \}) \end{eqnarray}


Remains to verify $p(t) \geq 0, u(t_1) \geq 0$?

\begin{eqnarray}
p(t_2) &=&  \int_{q_1}^{q_2} g(q) \pi(q,t_2) v(q,t_2) dq   - \max\{0, v(t_2 \}) \\ 
\end{eqnarray}
$\pi(q,t_2) = 1$ whenever $q \geq \theta(t_2) $ or equivalently $ v(q,t_2) + v_1(q) \frac{F(t_2)}{f(t_2)} \geq 0 $. 



What remains to verify is $p(t) \geq 0$, as follows:
\begin{eqnarray}
p(t)  &=&  \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq + \int_{t_1}^t Q(x) dx   \\ 
 &=&  \int_{q_1}^{q_2} g(q) \pi(q,t) v(q,t) dq + \int_{t_1}^t \int_{q_1}^{q_2} g(q) \pi(q,x)  v_1(q)  dq  dx   \\  
\end{eqnarray}


As $\odv{u(t)}{t}\ge0$, we can set $u(0)=0$. Let
\begin{gather*}
\varphi(t|q)=v(q,t)-\pdv{v(q,t)}{t}\frac{1-F(t)}{f(t)}.
\end{gather*}
We have
\begin{gather*}
REV=\int_{q_1}^{q_2} g(q)\left[ \int_{t_1}^{t_2} f(t)\pi_t(q,1)\varphi(t|q)\,\mathrm{d}t \right].
\end{gather*}
Similar to the Myerson auction, there is a threshold $\theta_q$ for each $q$. We may need the ``ironing'' trick and define
\begin{gather*}
R(\eta|q)=v\cdot \eta,
\end{gather*}
where $\eta=1-F(t)$. And we also have $\pdv{R(\eta|q)}{\eta}=\varphi(t|q)$.

With Equation \eqref{eq:allocation_monotonicity}, any threshold testing mechanism must satisfy that $\theta_t$ is decreasing in $t$. If the optimal mechanism is a threshold testing mechanism, then $\theta_q$ must also be a decreasing function of $q$. With the regularity assumption, we have
\begin{gather*}
v(q,\theta_q)-\pdv{v(q,\theta_q)}{\theta_q}\frac{1-F(\theta_q)}{f(\theta_q)}=0.
\end{gather*}
Therefore, the optimal mechanism is a threshold testing mechanism if and only if
\begin{gather*}
\odv{\theta_q}{q}\le 0,
\end{gather*}
where
\begin{gather*}
\odv{\theta_q}{q}=-\frac{\pdv{v(q,\theta_q)}{q}-\pdv{v(q,\theta_q)}{q,\theta_q}\frac{1-F(\theta_q)}{f(\theta_q)}}{\pdv{v(q,\theta_q)}{\theta_q}-\pdv[2]{v(q,\theta_q)}{\theta_q}\frac{-f^2(\theta_q)-(1-F(\theta_q))f'(\theta_q)}{f^2(\theta_q)}}
\end{gather*}


==> optimal.tex <==
\section{The Optimal Mechanism}
%We consider the case where both $t\in T = [t_1, t_2]$ and $q\in Q = [q_1, q_2]$ are continuous. Assume $q\sim G(q)$ and $t\sim F(t)$ are independent.  As a useful notation, let $v(t) = \Ex_{q \sim G} v(q,t) = \int_{q \in Q} g(q) v(q,t) dq $ denote the expected utility of buyer type $t$ for taking action $1$ without any additional information. Note that, the utility for action $0$ is always $0$, regardless of $q,t$. 
%
%\begin{definition}[Threshold Mechanism]
%Define $v(q,t) = v_1(q)t+ v_0(q) = v_1(q)[t + \rho(q)]$ where $\rho(q) = \frac{v_0(q)}{v_1(q)}$. A  threshold mechanism is described by two functions $\theta_t, p(t)$ over   buyer type $t$, such that buyer type $t$ will be charged $p(t)$ and afterwards be recommended action $1$ at state $q$ if and only if $\rho(q) \geq \theta_t$.  
%\end{definition} 
%
%% \begin{definition}[Upper/Lower-Boundary Virtual Value Function]
%% We call  $\underline{\phi}(t) = t - \frac{1-F(t)}{f(t)}$   the \emph{lower-boundary} virtual value function and call  $\bar{\phi}(t) = t + \frac{F(t)}{f(t)} $  the \emph{upper-boundary} virtual value function.  We say a virtual value function, upper-boundary or lower-boundary, is regular if it is monotone non-decreasing in $t$. 
%% \end{definition}
%
%
%\begin{definition}[Upper/Lower  Virtual Value Function]
%We call  $\underline{\phi}(t) = t - \frac{1-F(t)}{f(t)}$   the \emph{lower} virtual value function and call  $\bar{\phi}(t) = t + \frac{F(t)}{f(t)} $  the \emph{upper} virtual value function.  We say a lower or upper virtual value function  is \emph{regular} if it is monotone non-decreasing in $t$. 
%\end{definition} 
%
%\begin{definition}[Ironed Upper/Lower  Virtual Value Function]
%We call  $\underline{\phi}(t) = t - \frac{1-F(t)}{f(t)}$   the \emph{ ironed lower} virtual value function and call  $\bar{\phi}(t) = t + \frac{F(t)}{f(t)} $  the \emph{ironed upper} virtual value function.  We say a lower or upper virtual value function  is \emph{regular} if it is monotone non-decreasing in $t$. 
%\end{definition}
%
%
%Our main result is the following theorem.
%
%
%\begin{theorem}%\label{thm:opt-scheme}
%Given $v(q,t) = v_1(q)[t + \rho(q)]$,
%\begin{enumerate}
%\item If $v(t_2) \leq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) dq  dx $ and $\underline{\phi}(t)$ is monotone non-decreasing, the optimal information selling mechanism is a threshold mechanism on $\rho(q)$ with threshold $\underline{\theta}_t =  -\underline{\phi}(t) $ for each type $t$.  The payment is determined by the following identity and is monotone non-decreasing in $t$: $$p(t) = \int_{q\in Q} [g(q) \pi(q,t)v(q,t)] dq -  \int_{t_1}^{t} P(x)  dx.$$ 
%\item If $v(t_2) \geq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx $ and $\bar{\phi}(t)$ is monotone non-decreasing, the optimal information selling mechanism is a threshold mechanism on $\rho(q)$ with threshold $\bar{\theta}_t =  -\bar{\phi}(t) $ for each type $t$. The payment is determined by the following identity and is monotone non-increasing in $t$:
%$$p(t) = \int_{q\in Q} [g(q) \pi(q,t)v(q,t)] dq - v(t_2) + \int_{t}^{t_2} P(x)  dx.$$   
%\item If $\max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) dq  dx  \leq v(t_2) \leq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) \\ dq  dx $, with new virtual value $\widetilde{\phi}_q(t) = f(t)t + F(t) + f(t)\rho(q)$ is non-decreasing in t for any q, the optimal mechanism is a threshold mechanism on $\rho(q)$ with threshold $\theta(t) =\frac{C - f(t)t - F(t)}{f(t)} $, where $C \in [0,1) $ is a constant and satisfies  $\int_{(t,q):  \widetilde{\phi}_q(t)>= C } g(q)  v_1(q) dq dt = v(t_2)$. 
%
%The payment is determined by the following identity and is monotone non-decreasing in $t\leq F(t)$ and monotone non-increasing in $t>F(t)$:
%$$
%p(t) = \int_{q \in Q} g(q) \pi(q,t)v(q,t) dq -  \int_{t_1}^{t} P(x)  dx
%$$
% 
%\end{enumerate}
%
%
%\end{theorem}
% 




\textbf{An Instance in Case 1:}

Define an instance where both the type $t$ of the buyer and the quality $q$ are uniformed distributed over 0 to 2. \\
$t_1  = 0$, $t_2 = 2$, $\forall t \; f(t) = \frac{1}{2}$ \\
$q_1  = 0$, $q_2 = 2$, $\forall q \; g(q) = \frac{1}{2}$ \\
$v_1(q) = q $, $\rho(q) = - \frac{3}{q}$. Thus, $v(q,t) = qt - 3$\\


Now, we can do the computations to decide which case this instance belongs to. The value the Buyer with type $t$ can get with $Purchase$ for all the items are: \\
$v(t_1) = \int_{q \in Q}g(q)v(q,t_1) dq = \int_{q \in Q} \frac{1}{2} (0 -3 ) dq = -3$ \\
$v(t_2) = \int_{q \in Q}g(q)v(q,t_2) dq = \int_{q \in Q} \frac{1}{2} (2q - 3) dq = -1$ \\


$\underline{\phi}(t) = t - \frac{1 - F(t)}{f(t)} = 2t - 2$  \\
$\int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) dq  dx =  \int_{0}^{2} \int_{q: -\frac{3}{q} \geq - (2t-2)} (\frac{1}{2} q) dq  dx = \frac{1}{16} $ 


Thus, this instance is  in case 1 because of
$v(t_2) \leq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) dq  dx $.





Thus, the optimal policy is to recommend $purchase$ whenever $\rho(q) \geq -\underline{\phi}(t) $ and $not \; purchase$ otherwise. And for each type $t$, the information price in close form is 
\begin{align*}
 p(t) &= \int_{q\in Q} [g(q) \pi(q,t)v(q,t)] dq -  \int_{t_1}^{t} P(x)  dx \\
 &= \int_{q\in Q} [ \mathbb{I}(\rho(q) \geq -\underline{\phi}(t))  \frac{1}{2} (qt - 3)] dq -  \int_{0}^{t} \int_{q\in Q} [\mathbb{I}(\rho(q) \geq -\underline{\phi}(x)) \frac{1}{2}  q] dq  dx 
\end{align*}



\textbf{An Instance in Case 2:}

Define an instance where\\
$t_1  = 3$, $t_2 = 6$, $\forall t \; f(t) = \frac{1}{3}$ \\
$q_1  = 1$, $q_2 = 4$, $\forall q \; g(q) = \frac{1}{3}$ \\
$v_1(q) = q $, $v_0(q) = -6$. Thus, $v(q,t) = qt - 6$ and $\rho(q) = - \frac{6}{q}$. \\

\hf{ refer to my comments at the beginning, we will not use $t_0$ any more.  }

Now, we can do the computations to decide which cases this instance belongs to. \\
$v(t_1) = \int_{q \in Q}g(q)v(q,t_1) dq = \int_{q \in Q} \frac{1}{3} (3q -6 ) dq = 1.5$ \\
$v(t_2) = \int_{q \in Q}g(q)v(q,t_2) dq = \int_{q \in Q} \frac{1}{3} (6q - 6) dq = 9$ \\


$\bar{\phi}(t) = t + \frac{F(t)}{f(t)} = 2t - 3$  \\
$\int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx =  \int_{3}^{6} \int_{q: -\frac{6}{q} \geq - (2t-3)} (\frac{1}{3} q) dq  dx = 7.25 $ 

Thus, this instance is  in case 2 because of
$v(t_2) \geq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx $


Thus, the optimal policy is to recommend $purchase$ whenever $\rho(q) \geq -\bar{\phi}(t) $ and $not \; purchase$ otherwise. And for each type $t$, the information price in close form is 
\begin{align*}
p(t) &= \int_{q\in Q} [g(q) \pi(q,t)v(q,t)] dq - v(t_2) + \int_{t}^{t_2} P(x)  dx \\
 &= \int_{q\in Q} [ \mathbb{I}(\rho(q) \geq -\bar{\phi}(t))  \frac{1}{3} (qt - 6)] dq - 9 + \int_{3}^{t} \int_{q\in Q} [\mathbb{I}(\rho(q) \geq -\bar{\phi}(x)) \frac{1}{3}  q] dq  dx 
\end{align*}


 
\textbf{An Instance in Case 3:}

Define an instance where\\
$t_0  = 0$, $t_1 = 10$, $\forall t \; f(t) = \frac{1}{10}$ \\
$q_0  = 0$, $q_1 = 10$, $\forall q \; g(q) = \frac{1}{10}$ \\
$v_1(q) = q $, $v_0(q) = -30$. Thus, $v(q,t) = qt - 30$ \\

Now, we can do the computations to decide which cases this instance belongs to. \\
$v(t_1) = \int_{q \in Q}g(q)v(q,t_1) dq = \int_{q \in Q} \frac{1}{10} -30 dq = -30$ \\
$v(t_2) = \int_{q \in Q}g(q)v(q,t_2) dq = \int_{q \in Q} \frac{1}{10} (10q - 30) dq = 20$ 

$\underline{\phi}(t) = t - \frac{1-F(t)}{f(t)} = 2t - 10$  \\
$\int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) dq  dx = \int_{0}^{10} \int_{q: -\frac{30}{q} \geq - (2t -10)} (\frac{1}{10} q) dq  dx \approx 12.25 $ 


$\bar{\phi}(t) = t + \frac{F(t)}{f(t)} = 2t$  \\
$\int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx =  \int_{0}^{10} \int_{q: -\frac{30}{q} \geq - 2t} (\frac{1}{10} q) dq  dx \approx 36.13 $ 

Thus, this is an instance of case 3 because of $\max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \underline{\theta}_x} g(q) v_1(q) dq  dx  \leq v(t_2) \leq \max \{v(t_1), 0 \} + \int_{t_1}^{t_2} \int_{q: \rho(q) \geq \bar{\theta}_x} g(q) v_1(q) dq  dx $.
So, we can use binary search to find a C where $C \in [0,1) $ is a constant and satisfies  $\int_{(t,q):  \widetilde{\phi}_q(t)>= C } g(q)  v_1(q) dq dt = v(t_2)$.


Thus, the optimal policy is to recommend $purchase$ whenever $\rho(q) \geq \theta(t) =\frac{C - f(t)t - F(t)}{f(t)}$ and $not \; purchase$ otherwise. And for each type $t$, the information price in close form is 
\begin{align*}
 p(t) &= \int_{q\in Q} [g(q) \pi(q,t)v(q,t)] dq -  \int_{t_1}^{t} P(x)  dx \\
 &= \int_{q\in Q} [ \mathbb{I}(\rho(q) \geq \theta(t))  \frac{1}{10} (qt - 30)] dq -  \int_{0}^{t} \int_{q\in Q} [\mathbb{I}(\rho(q) \geq \theta(x)) \frac{1}{10}  q] dq  dx 
\end{align*}

% \noincident{Interpretations of the Conditions. } 
 
 
 
% \textbf{Explanation of the theorem:}

% This theorem covers all the possible cases of $v(q,t)$. Because $v(q,t)$ is assumed to be non-decreasing in both $q$ and $t$, $v(t_2) \leq 0 \Rightarrow \forall t \; v(t) \leq 0$ and $v(t_1) \geq 0 \Rightarrow \forall t \; v(t) \geq 0$. Since $\forall q \; v_1(q) > 0$, we have $\int_{\rho(q) \geq \underline{\theta}_(x)} g(q) v_1(q) dq  dx \geq 0$ and $\int_{\rho(q) \geq \bar{\theta}_(x)} g(q) v_1(q) dq  dx \geq 0$.

% So, the first augment covers the cases $\forall t \; v(t) \leq 0$ and part of cases where $v(t_1) \leq 0$ and $0 \leq v(t_2) \leq \int_{t_1}^{t_2} \int_{\rho(q) \geq \underline{\theta}_(x)} g(q) v_1(q) dq  dx$. The second augment covers the cases $\forall t \; v(t) \geq 0$ and part of cases where $v(t_1) \leq 0$ and $v(t_2) \geq  \int_{t_1}^{t_2} \int_{\rho(q) \geq \bar{\theta}_(x)} g(q) v_1(q) dq dx  \geq 0$. 

% The third augment covers the remain cases where $v(t_1) \leq 0$ and $\int_{t_1}^{t_2} \int_{\rho(q) \geq \underline{\theta}_(x)} g(q) v_1(q) dq  dx \leq v(t_2) \leq \int_{t_1}^{t_2} \int_{\rho(q) \geq \bar{\theta}_(x)} g(q) v_1(q) dq  dx$.


%\section{Proof of Theorem \ref{thm:opt-scheme}}
%\subsection{Problem Formulation}
%Our starting point is the revelation principle  proved in previous works \cite{Babaioff12,chen2020selling} for selling information. Specifically, when $q,t$ are independent, there always exists an optimal mechanism that consists of a pair $\pi(  t), p(t)$ for each type $t \in T$ where $\pi(  t)$ is an \emph{obedient} signaling scheme and $p(t)$ is the payment of type $t$. Since both $\pi(t), p(t)$ depend on the continuous variable $t$, we shall refer to them as signaling function and payment function, respectively. The mechanism proceeds as follows: 
%\begin{enumerate}
%   \item Seller posts  a mechanism consists of the signaling function $\pi(t)$ and payment function $p(t)$;
%    \item The true state of nature $q$ and buyer type $t$ are realized;  
%    \item Seller asks the buyer to report his type $t$ and  charges the buyer  $p(t)$;\footnote{An alternative way is to post a menu $\{\pi(t), p(t) \}_{t \in T}$ and then ask the buyer to select a menu. This is mathematically equivalent to imposing incentive compatibility constraints and then asking the buyer to report his type. However, since there is a continum amount of buyer types, buyer type reporting could be an easier way to implement in practice. }  
%    \item Seller signals information to the buyer according to the signaling scheme $\pi(t)$ and realized $q$. 
%\end{enumerate} 
%Moreover, the mechanism can without of generality to be incentive compatible --- i.e., revealing true type $t$ is a best response for the buyer. Note that the above mechanism only has a single-round interaction. Nevertheless, there always exists an optimal mechanism of this format, even when multi-round interactions are allowed. This is due to the independence   between buyer type $t$ and state $q$ \cite{Babaioff12}. 
%
%Similar to classic mechanism design for  goods, the revelation principle here does not  tell us what the signaling function and payment function are like. The remainder  of this section will derive an optimal solution for $\pi(t), p(t)$ in our information selling setup.  
%%Different from the above results from \cite{chen2020selling}, Theorem \ref{thm:opt-scheme} provides a   characterization of the optimal information selling mechanism, which terms out to have a natural format that is observed widely in practice. To prove Theorem \ref{thm:opt-scheme}, we  first utilize the results of \cite{chen2020selling} to formulate the problem of optimal mechanism design for selling information in our setup. Formally,   
%We start with some necessary definitions. A signaling scheme in our setup can be viewed as a function $\pi: Q \times T \to [0,1] $ over \emph{continuous} variables, where $\pi(q, t) \in [0,1]$ is the probability of recommending action $1$ at quality $q$ conditioning on buyer type $t$ (thus action $0$ is recommended with probability $1 -\pi(q, t)$). A payment function $p(t)$ is also defined on the continuous domain. The information seller's objective is thus to maximize the following objective of revenue:
%\begin{equation}\label{cons:obj}
%\text{ Seller's Objective: } \quad \max_{\pi, p} \int_{t\in T} f(t) p(t) dt  
%\end{equation}
%
%The mechanism $(\pi, p)$ needs to satisfy the following sets of conditions. 
%
%The first set of constraints is the \emph{obedience} constraint for the signaling scheme. That is, when action $1$ is recommended to a buyer type $t$, the expected conditional buyer utility of taking action $1$ is $ \frac{ \Ex_{q\sim G}\left[ \pi(q,t)v(q,t) \right] }{ \Ex_{q\sim G} [\pi(q,t)] }$, which should indeed be at least $0$, i.e., the utility of action $0$. This is equivalent to $\Ex_{q\sim G}\left[ \pi(q,t)v(q,t) \right] \geq 0$. Conversely,  when action $0$ is recommended to a buyer type $t$, the expected conditional buyer utility of taking action $1$ is $ \frac{ \Ex_{q\sim G}\left[ (1 - \pi(q,t)) \cdot v(q,t) \right] }{ \Ex_{q\sim G} [1 - \pi(q,t)] }$, which should be at most $0$. This is equivalent to $\Ex_{q\sim G}\left[ (1 - \pi(q,t)) \cdot v(q,t) \right] \leq 0$ or $\Ex_{q\sim G}\left[   \pi(q,t) \cdot v(q,t) \right] \geq \Ex_{q\sim G}\left[  v(q,t) \right] = v(t) $. 
%% These two constraints can be mathematically expressed as the following linear constraints over the signaling scheme $\pi$:  
%% \begin{eqnarray}
%% \text{Obedience Constraints: } & \quad &  \int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t) dq  \geq  0\\
%% & \quad &  \int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t) dq  \geq   v(t). 
%% \end{eqnarray}
%As a consequence, the obedience constraint can be summarized into the following  linear constraint over the signaling scheme $\pi$:  
%\begin{eqnarray}\label{cons:obedience}
%\text{Obedience: } \quad & & \int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t) dq \geq   \max \{ 0, v(t) \}, \, \, \, \forall t \in [T]
%\end{eqnarray}
%
%The second set of constraint is the incentive compatibility (IC) constraint. That is, each buyer type $t$ has no incentive to misreport any other type $t'$. Note that, given any obedient signaling scheme, the expected utility of buyer type $t$ from the scheme, under truthful reporting,  is $\int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t)$. Therefore, the IC  constraint can be expressed as follows:
%\begin{equation}\label{cons:IC}
%\text{IC: } \quad \int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t) dq - p(t) \geq \int_{q \in Q} \pi(q, t') \cdot g(q) v(q,t) dq  - p(t'), \, \, \, \forall, t, t' \in [T] 
%\end{equation}
%
%The last set of constraints is the individual rationality (IR) constraint. That is, participating the mechanism is at least as good as no participation, in which case the buyer utility is $\max \{ 0, v(t) \}$, i.e., the larger of the utilities of action $0$ and $1$ without any additional information from the seller.  The IR constraint can be expressed as follows.
%\begin{equation}\label{cons:IR}
%    \text{IR Constraint: } \quad \int_{q \in Q} \pi(q, t) \cdot g(q) v(q,t) dq - p(t) \geq  \max \{ 0, v(t) \}, \, \, \, \forall, t  \in [T]  
%\end{equation} 
%
%The seller's optimization problem is to find feasible mechanism $(\pi, p)$ to maximize Objective \eqref{cons:obj} subject to Constraints \eqref{cons:obedience}, \eqref{cons:IC} and \eqref{cons:IR}. 

% Now, because the buyer will have a imperfect prior (the distribution of the quality) of the information target, the buyer can make a rough decision whether to $purchase$ the product or not. So, compared with classic physical goods with benchmark $0$, we need to increase the benchmark to $\max(0,v(t)$.
%  As we shall see, this  difference makes the classic Myerson approach does not directly apply to our setup and raises crucial challenges to the design of information selling mechanism.        %the buyer utility is the expected utility over the item quality whereas the buyer's utility in single-item auction is the expected utility over other bidders' values. Moreover, we have an additional constraint, i.e.,


\hf{add a discussion about correlated $t,q$. I think this correlated setting is not that well-motivated in our model since there are not many cases where buyer's value $t$ is correlated with some uncertainty $q$.   Also discuss
about non-linear buyer utility function, about when $v_1(q)$ is not always positive.  }

